Stability Guarantees for Feature Attributions with Multiplicative Smoothing

Explanation methods for machine learning models tend not to provide any formal guarantees and may not reflect the underlying decision-making process. In this work, we analyze stability as a property for reliable feature attribution methods. We prove that relaxed variants of stability are guaranteed if the model is sufficiently Lipschitz with respect to the masking of features. We develop a smoothing method called Multiplicative Smoothing (MuS) to achieve such a model. We show that MuS overcomes the theoretical limitations of standard smoothing techniques and can be integrated with any classifier and feature attribution method. We evaluate MuS on vision and language models with various feature attribution methods, such as LIME and SHAP, and demonstrate that MuS endows feature attributions with non-trivial stability guarantees.

==> old/alternative_formulations_1.tex <==
\section{Alternative Formulations of Smoothing Results}

We now present some alternative formulations of our smoothing results.
Many of these results have a similar flavor, except rather than specifying the smoothing parameter \(\lambda\), we instead draw the feature attribution \(\alpha \in [0,1]_{(q)} ^n\), where \([0,1]_{(q)} = \{0, 1/q, \ldots, q/q\}\) is a uniform \((q+1)\)-valued discretization of the unit interval.


\begin{theorem}[Alt. Simple \dname{}] \label{thm:alt-simple-smoothing}
    Consider any \(h : \mcal{X} \to [0,1]\) and define \(g : \mcal{X} \times \mbb{R}^n \to [0,1]\) as
    \begin{align} \label{eq:thm:alt-simple-smoothing}
        g(x, \alpha) = \expval{s \sim \mcal{U}^{n} (0,1)} h(x \odot \tilde{\alpha}),
        \quad \tilde{\alpha} = \mbb{I}[\alpha \geq s]
    \end{align}
    Then \(g(x, \cdot) : \mbb{R}^n \to [0,1]\) is \(1\)-Lipschitz in the \(\ell^1\) norm for all \(x \in \mcal{X}\).
\end{theorem}
\begin{proof}
Consider any \(x \in \mcal{X}\) and let \(\mbb{I}_{\geq 0} : \mbb{R}^{n} \to \{0,1\}^n\) be the coordinate-wise indicator function of non-negativity.
Then we may rewrite \(g(x, \alpha)\) as
\begin{align*}
    g(x, \alpha)
    &= \expval{s \sim \mcal{U}^{n} (0,1)}
        \bracks{(h \circ (x \odot \cdot) \circ \mbb{I}_{\geq 0})(\alpha - s)} \\
    &= \expval{s \sim \mcal{U}^n (0,1)}
        \bracks{\omega (\alpha - s)} \\
    &= \expval{t \sim \mcal{U}^n (-1/2, 1/2)}
        \bracks{\omega(\alpha - 
        (- t + \mbf{1}/2))} \\
    &= \expval{t \sim \mcal{U}^n (-1/2, 1/2)}
        \bracks{h (\alpha + t - \mbf{1}/2)},
\end{align*}
where \(\omega : \mbb{R}^n \to [0,1]\) is implicitly defined, and use
\begin{align*}
    \mcal{U}^n (0,1) = - \underbrace{\mcal{U}^n (-1/2, 1/2)}_{\sim t} + \mbf{1}/2.
\end{align*}
It follows from Theorem 1~\cite{levine2021improved} that \(g(x, \cdot)\) is \(1\)-Lipschitz in the \(\ell^1\) norm.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Alt. Derandomized \dname{}] \label{thm:alt-derand-smoothing}
    Fix an integer \(q > 0\) and let \(s \sim \mcal{D}\) be a \(n\)-dimensional random vector with each coordinate uniformly distributed as
    \begin{align} \label{eq:thm:alt-derand-smoothing-1}
        s_i \sim \mcal{U}(\{1/q, \ldots, q/q\}) - 1/(2q),
        \enskip i = 1, \ldots, n,
    \end{align}
    where \(\mcal{D}\) is any finite discrete distribution on \([0,1]^n\) such that \(s_i\) need not be independent.
    Consider any \(h : \mcal{X} \to [0,1]\) and define \(g : \mcal{X} \times [0,1]_{(q)} ^{n} \to [0,1]\) as
    \begin{align} \label{eq:thm:alt-derand-smoothing-2}
        g(x, \alpha) = \expval{s \sim \mcal{D}} h(x \odot \tilde{\alpha}),
        \quad \tilde{\alpha} = \mbb{I}[\alpha \geq s],
    \end{align}
    Then \(g(x, \cdot) : [0,1]_{(q)} ^n \to [0,1]\) is \(1\)-Lipschitz in the \(\ell^1\) norm for all \(x \in \mcal{X}\).
\end{theorem}
\begin{proof}
Fix any \(s \sim \mcal{D}\) and \(x \in \mcal{X}\).
Let \(\alpha, \alpha' \in [0,1]_{(q)} ^n\) and define \(\delta = \alpha - \alpha'\).
Observe that \(\tilde{\alpha}_i \neq \tilde{\alpha}_i '\) exactly when: either \(\alpha_i < s_i < \alpha_i '\) or \(\alpha_i ' < s_i < \alpha_i\).
Because \(s_i\) is uniformly distributed across \(q\) distinct values and only \(\abs{\delta_i} q\) of those values can make this condition hold, it follows that \(\mrm{Pr}[\tilde{\alpha}_i \neq \tilde{\alpha}_i '] = \abs{\delta_i}\).
Applying the union bound:
\begin{align*}
    \prob{s \sim \mcal{D}}
        \bracks{\tilde{\alpha} \neq \tilde{\alpha}'}
    = \prob{s \sim \mcal{D}}
        \bracks{\bigcup_{i=1}^{n} \tilde{\alpha}_i \neq \tilde{\alpha}_i '}
    \leq \sum_{i=1}^{n} \abs{\delta_i}
    = \norm{\delta}_1,
\end{align*}
and so:
\begin{align*}
    \abs{g(x, \alpha) - g(x, \alpha')}
    &= \abs*{\expval{s \sim \mcal{D}} h(x \odot \tilde{\alpha})
        - \expval{s \sim \mcal{D}} h(x \odot \tilde{\alpha}')} \\
    &= \abs*{\expval{s \sim \mcal{D}}
            \bracks{h(x \odot \tilde{\alpha}) - h(x \odot \tilde{\alpha}')}} \\
    &= \Big|
            \prob{s \sim \mcal{D}} \bracks{\tilde{\alpha} \neq \tilde{\alpha}'}
            \cdot \expval{s \sim \mcal{D}} \bracks{h(x \odot \tilde{\alpha}) - h(x \odot \tilde{\alpha}') \,|\, \tilde{\alpha} \neq \tilde{\alpha}'} \\
    &\quad - \prob{s \sim \mcal{D}} \bracks{\tilde{\alpha} = \tilde{\alpha}'}
            \cdot \expval{s \sim \mcal{D}} \bracks{h(x \odot \tilde{\alpha}) - h(x \odot \tilde{\alpha}') \,|\, \tilde{\alpha} = \tilde{\alpha}'}
        \Big|.
\end{align*}
Note that \(\mbb{E}\, \bracks{h(x \odot \tilde{\alpha}) - h(x \odot \tilde{\alpha}') \,|\, \tilde{\alpha} = \tilde{\alpha}'} = 0\), and so
\begin{align*}
    \abs{g(x, \alpha) - g(x, \alpha')}
    &= \prob{s \sim \mcal{D}} \bracks{\tilde{\alpha} \neq \tilde{\alpha}'}
            \cdot
            \underbrace{
                \abs*{\expval{s \sim \mcal{D}} \bracks{h(\angles{x, \tilde{\alpha}}) - h(\angles{x, \tilde{\alpha}'}) \,|\, \tilde{\alpha} \neq \tilde{\alpha}'}}
            }_{\leq 1 \enskip \text{because \(h(\cdot) \in [0,1]\)}}
    \\
    & \leq \prob{s \sim \mcal{D}} \bracks{\tilde{\alpha} \neq \tilde{\alpha}'}
    \leq \norm{\delta}_1 .
\end{align*}
Thus, \(g(x, \cdot)\) is \(1\)-Lipschitz in the \(\ell^1\) norm.
\end{proof}




==> old/attribution_study.tex <==
% \input{figures/feature-attributions-eval}

\section{A Study of Feature Attribution Methods}
\label{sec:attribution-study}


We additionally study the quality of existing feature attribution methods, namely vanilla gradient saliency, Integrated Gradients, LIME, and SHAP.
All of these methods provide continuous-valued attribution scores, and we convert these to binary feature attributions by taking the top-k fraction of scores for \(k \in \{1/8, 2/8, 3/8, 4/8\}\).
Our results are shown in Figure~\ref{fig:feature-attributions-eval-1}.
Each plot shows the clean accuracy vs the \(\lambda\).
We see that in general SHAP generates the attributions that best explain the input.

We also use these four feature attribution methods as a starting point \(\varphi\).
We measure the \emph{density} of a binary feature attribution as \(\norm{\alpha}_1 / n\), which is the fraction features that are hot.
Our results are shown in Figure~\ref{fig:feature-attributions-eval-2}.
On the horizontal axis we enumerate through the top-k\% of the scores.
We see that on average SHAP provides the sparsest binary feature attributios, followed by Integrated Gradients.



==> old/experiments_1.tex <==
\section{Empirical Evaluations}
\label{sec:experiments}



In our numerical experiments we aim to evaluate answer the following questions:

\paragraph{(Q1)} \textbf{Does smoothing yield robust explanations?}
We investigate whether \dname{} yields non-vacuous robustness on guarantees on feature attributions.


\paragraph{(Q2)} \textbf{What is the cost of smoothing?}
We investigate how varying the Lipschitz constant \(\lambda\) affects the accuracy and robustness of the smoothed classifier.


\paragraph{(Q3)} \textbf{What is the empirical-theoretical gap?}
We investigate to what extent is the certified radii of Section~\ref{sec:certifying-stability} conservative, compared to empirically sampled ones?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \paragraph{(Q1)} \textbf{Does smoothing help?}
% Is \dname{} smoothing able to yield strong robustness guarantees without significantly sacrificing accuracy?
% We investigate the impact of decreasing \(\lambda\) (more noise and smaller Lipschitz constant) affects the overall smoothed classifier accuracy.


% \paragraph{(Q2)} \textbf{Which existing methods are good?}
% We study binary feature attributions extracted from three different feature attribution methods: vanilla gradient
% saliency~\cite{simonyan2013deep}, Integrated Gradients~\cite{sundararajan2017axiomatic}, LIME~\cite{ribeiro2016should}, and SHAP~\cite{lundberg2017unified}.
% In particular, we see how well the top-k fraction of the attributions serve as explanations, and which method generates the most efficient ordering by the criteria of Section~\ref{sec:constructing-robust}.


% \paragraph{(Q3)} \textbf{What is the gap between empirical and theoretical robustness guarantees?}
% It is well known that certified guarantees tend to be conservative, but to what extent are the certified radii in Section~\ref{sec:robustness-analysis} conservative, compared to empirically sampled ones?


\paragraph{Experimental Setup}
We consider three models in total: two vision models in Vision Transformer~\cite{dosovitskiy2020image} and ResNet50~\cite{he2016deep}; and one language model in RoBERTa~\cite{liu2019roberta}.
For the vision dataset we use ImageNet~\cite{russakovsky2015imagenet} and for the language dataset we use TweetEval~\cite{barbieri2020tweeteval}.
We apply some extensions from Appendix~\ref{sec:basic-extensions} to boost performance.
Namely, we use feature grouping on ImageNet1K to reduce the \(3 \times 224 \times 224\) sized-image into patches of size \(3 \times 16 \times 16\), such that the there are a total of \((224/16)^2 = 196\) feature groups.
This means that explanations have size \(\alpha \in \{0,1\}^{196}\).
We also apply selective masking for decremental stability in order to slightly boost performance.


For each \(\lambda \in \{1/8, 2/8, \ldots, 8/8\}\), we fine-tuned each classifier with ADAM~\cite{kingma2014adam} for \(1\) epoch on their respective dataset with learing rates of: Vision Transformer (\(5 \times 10^{-6}\)), ResNet50 (\(10^{-5}\)), RoBERTa (\(10^{-6}\)).
For each \(x\) in the training dataset we generate two copies: one ablated so that only \(\lambda\) fraction of the features are retained, and the other so that \(\lambda/2\) fraction of the features are retained.
For instance if \(\lambda = 5/8\) we generate two copies of \(x\) for training: one where \(5/8\) of the features are kept, and one where \(5/16\) of the features are kept.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{figures/robust-explanation-accuracy}
\subsection{(Q1) Robust Explanations and Smoothing}
We first investigate whether smoothing is able to yield robustness guarantees on accuracy.
For \(\varphi\) we use a simple method of SHAP top-25\%, i.e. the top 25\% of the features are selected for \(\varphi(x)\).
While this means that the \(\angles{f, \varphi}\) is not guaranteed to be consistent nor non-trivially stable, our goal for this experiment is to study how changing \(\lambda\) affects the fraction of inputs that can be certified --- and up to what radius of stability.


We show these numbers in Figure~\ref{fig:robust-explanation-accuracy}, where we show the fraction of inputs that are certifiable up to a particular radius.
We see that more smoothing (i.e. smaller \(\lambda\)) does indeed allow for more samples to be certified at a greater radius --- though at a cost to accuracy.
In particular, decremental stability is better preserved at lower \(\lambda\).



\input{figures/certified-accuracy}
\subsection{(Q2) Cost of Smoothing}
We next investigate how smoothing impacts the classifier accuracy.
We show in Figure~\ref{fig:certified-accuracy} the certified accuracy of our smoothed classifiers, with \(N = 2000\) samples drawn from their respective datasets.
The smoothed classifier is shown the full input, and the certified accuracy depicts the fraction of images that can be classified correctly vs up to how many feature (groups) of perturbation can we certify this classification.
The clean accuracy is the value at radius zero, and corresponds to the accuracy of the smoothed classifier on their respective datasets.
The value of \(\lambda = 1\) is equivalent to the original classifier with no smoothing applied.






\input{figures/empirical-robustness}
\subsection{(Q3) Empirical Robustness}

It is known that provable guarantees are often conservative compared to what is empirically observed.
We test the empirical radii that can be obtained for \(P_{\mrm{suff}}\) and \(P_{\mrm{necc}}\).
We sample \(N = 250\) elements from each respective dataset, and take \(\alpha\) generated by SHAP-top-25\%.
Note this means that \(\alpha\) may not explain each \(x\), and may not be certifiably robust --- but this ensures a consistent format of \(\alpha\) for each experiment.
We then apply a box attack strategy like~\cite{chen2017zoo} to find the smallest radii at which a counter-example is found.
In general we find that as \(\lambda\) decreases, so does the corresponding curve --- meaning that it becomes harder to find counter-examples.



\subsection{Discussion}
\label{sec:experments-discussion}
A possible limitation of using derandomized \dname{} (Theorem~\ref{thm:derand-smoothing}) is in the amount of \(q\) needed.
We found in experiments with ImageNet1K that values of \(q = 64\) are sufficient for high accuracy, with even \(q = 16\) achieving strong performance.
For hex-valued RGB images in particular, the practical limit is \(q = 256\) due to the inherent discrete nature of such encodings.
In addition, another limitation the possibility of an unlucky seed \(v\).

Moreover, we found feature grouping to be very helpful, as it reduces the effective dimensionality of the input, and therefore allows us to establish non-trivial stability radii.
For instance, an image from ImageNet1K has \(n = 3 \times 224 \times 224 = 150528\) features, which would require a prohibitively small \(\lambda\) to achieve any coverage on the image.
By taking patches of size \(3 \times 16 \times 16\) this reduces the effective dimension of an explanation to \(\alpha \in \{0,1\}^{196}\).



==> old/explanations_1.tex <==
\section{Problem Formulation}
\label{sec:explanations}

In this section we formally define our explanation properties of interest.
We are particularly interested in the power (\emph{sufficiency}) and compactness (\emph{necessity}) of an explanation
\footnote{
    For more properties, see~\cite{nauta2022anecdotal}.
},
which we choose to study in the framework of \emph{robustness}.
We first present some background on binary feature attribution methods, before formally defining robust formulations of sufficiency (\propA{}) and necessity (\propB{}).
These in turn then allows us to formally state the two central problems of this paper of \emph{analysis} and \emph{search}:


\begin{itemize}
    \item (\emph{Analysis}): to what extent does \(\alpha\) satisfy \propA{} and/or \propB{} with respect to model \(f\) and input \(x\)?
    
    \item (\emph{Search}): find \(\alpha\) that satisfies \propA{} and/or \propB{} given model \(f\) and input \(x\).
    
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Binary Feature Attribution}

We refer to measurable \(f : \mcal{X} \to [0,1]^K\) as \emph{classifiers}, where \(\mcal{X} \subseteq \mbb{R}^{n}\) and \(K\) are given, and let \(\mcal{F}\) be the space of all such \(f\).
For some \(x \in \mcal{X}\) we define its \emph{classification} by \(f\) to be the index of the largest logit:
\begin{align*}
    \mcal{C}(f, x) = \underset{1 \leq i \leq K}{\msf{argmax}} \enskip f_i (x).
\end{align*}
We call functionals of form \(\mcal{M} : \mcal{F} \times \mcal{X} \to \{0,1\}^n\) \emph{binary feature attribution methods}.
Given a classifier \(f \in \mcal{F}\) and input \(x \in \mcal{X}\), we call the binary vector \(\alpha = \mcal{M}(f, x)\) an \emph{explanation} of \(x\) with respect to \(f\), and we will sometimes use \emph{(binary) feature attribution} to mean the same thing.
Moreover, we say that \(\alpha\) is \emph{reproducing}
\footnote{
Sometimes also called \emph{preservation}~\cite{nauta2022anecdotal}.
}
for \(f, x\) if \(\mcal{C}(f, x \odot \alpha) = \mcal{C}(f, x)\).
% \begin{align*}
%     \mcal{C}(f, x \odot \alpha) = \mcal{C}(f, x),
% \end{align*}
That is, the ablated vector \(x \odot \alpha\) contains enough information to recover the classification of \(x\).
Crucially, this means that an output of \(\mcal{M}(f, x)\) might not be reproducing (although it is desirable), and this point of distinction allows us to more finely quantify the performance of \(\mcal{M}\).

It is also useful to establish a partial ordering (\(\preceq\)) over binary vectors.
We say that \(\alpha \preceq \beta\) if \(\alpha_i = 1\) implies \(\beta_i = 1\).
Moreover, recall that the \(\ell^1\) norm on binary vectors is simply the number of entries where they differ:
\begin{align*}
    \norm{\alpha - \beta}_1 = \abs{\{i \in [n] : \alpha_i \neq \beta_i\}},
    \quad [n] = \{1, \ldots, n\}.
\end{align*}
If \(\alpha_i = 1\), then we say that \(x_i\) is an \emph{explanatory} feature, and otherwise for \(\alpha_i = 0\) we say that \(x_i\) is a \emph{non-explanatory} feature.
These establish the background context for presenting our aforementioned properties, and below we present our formulations for sufficiency (\propA{}) and necessity (\propB{}) as robustness conditions with respect to non-explanatory features.



\subsection{Sufficiency}
When analyzing the quality of an explanation, it is common to think of an explanation as \emph{sufficient} if (1) contains enough information to reproduce the original classification, and that (2) the presented information is sufficiently information-rich, such that any superset of information would not affect the provided rationale.
We therefore say that \(\alpha\) is \emph{sufficient} with respect to \(f\) and \(x\) if: \(\alpha\) is reproducing, and any \(\alpha' \succeq \alpha\) is also reproducing, i.e. \(\mcal{C}(f, x \odot \alpha') = \mcal{C}(f, x)\).
The non-explanatory features of \(\alpha\) should therefore \emph{lack} so much coherent information that introducing any combination of them in \(\alpha'\) will not sufficiently hinder the predictive power of the already-present explanatory features.
This is formalized in the following definition.

\begin{definition}[Sufficiency]
Given a classifier \(f \in \mcal{F}\) and input \(x \in \mcal{X}\), we say that \(\alpha \in \{0,1\}^n\) is \emph{locally sufficient with radius \(r\)} if: \(\alpha\) is reproducing, and for any \(\delta \preceq 1 - \alpha\) such that \(\norm{\delta}_1 \leq r\), the binary vector \(\alpha + \delta\) is also reproducing.
We define the equivalent predicate as follows:
\begin{align*}
    &P_{\mrm{suff}}(f, x, \alpha, r) \equiv
    \mcal{C}(f, x) = \mcal{C}(f, x \odot \alpha)
    \enskip \text{and} \\
    &\quad \forall \delta :
        \norm{\delta}_1 \leq r, \,
        \delta \preceq 1 - \alpha \\
    &\quad \implies \mcal{C}(f, x) = \mcal{C}(f, x \odot (\alpha + \delta))
\end{align*}
\end{definition}

Notably, we have opted to present our formulation of sufficiency as a local property (i.e. for \(\norm{\alpha - \alpha'}_1 \leq r\) where \(\alpha' \succeq \alpha\)), rather than global one (for all \(\alpha' \succeq \alpha\)).
This is because checking for the global property is currently not computationally tractable on modern machine learning architectures, namely very large neural networks.
Unless special properties are known, a global check would involve enumerating through a prohibitively large search space.

We are also motivated to examine the local case because powerful classifiers also tend to be sensitive to small changes.
Highly similar explanations may in fact yield different predictions, and thus it makes sense to at least ensure the local quality of an explanation.

\red{IMAGE HERE}

\red{AAA}

\red{AAA}


\subsection{Necessity}
It is common to consider an explanation \emph{necessary} if it contains just enough information, such that any omission would lack explanatory power.
In other words, we may say that \(\alpha\) is \emph{necessary} if (1) it contains just enough information to recover the original classification, and (2) deleting non-explanatory features from the full image should not alter the prediction.
That is, \(\alpha\) is reproducing, and any \(\alpha'\) such that \(\alpha \preceq \alpha' \preceq \mbf{1}\) satisfies \(\mcal{C}(f, x\odot \alpha') = \mcal{C}(f, \mbf{1})\).
As with the sufficiency property of \propA{}, we can dually define the necessary condition as follows.


\begin{definition}[Necessity]
Given a classifier \(f \in \mcal{F}\) and input \(x \in \mcal{X}\), we say that \(\alpha\) is \emph{locally necessary with radius \(r\)} if: \(\alpha\) is reproducing, and for any \(\delta \preceq 1 - \alpha\) such that \(\norm{\delta}_1 \leq r\), the binary vector \(\mbf{1} - \delta\) is also reproducing.
We define the equivalent predicate as follows:
\begin{align*}
    &P_{\mrm{necc}}(f, x, \alpha, r) \equiv
        \mcal{C}(f, x) = \mcal{C}(f, x \odot \alpha) \enskip \text{and} \\
    &\quad \forall \delta :
        \norm{\delta}_1 \leq r, \,
        \delta \preceq 1 - \alpha \\
    &\quad \implies \mcal{C}(f, x) = \mcal{C}(f, x \odot (\mbf{1} - \delta))
\end{align*}
\end{definition}


Similar to sufficiency, we study a local variant of necessity.
Notably, we defined \propB{} as a ``dual'' to \propA{}: both are concerned with perturbations at the non-explanatory features, and coincide with sufficiently large \(r = n - \norm{\alpha}_1\).
In practice, we are rarely able to certify up to such a large \(r\), and the important point of distinction is that we treat \propA{} as \emph{additive}, and \propB{} as \emph{subtractive}.

\red{IMAGE HERE}

\red{AAA}

\red{AAA}


\subsection{Problem Statements}
We are now ready to formally present the problem statements.
We first formalize how to quantify the radii to which the properties \propA{} and \propB{} are satisfied, which gives us a sense of the quality of some \(\alpha\).
We assume that model \(f\), input \(x\), and explanation \(\alpha\) are given, and formulate the following problem:
\begin{align}\label{prob:analysis}
\begin{split}
    \underset{r \in \mbb{N}}{\text{maximize}}
        &\quad r \\
    \text{subject to}
        &\quad \forall \delta \in \{\delta : \norm{\delta}_1 \leq r, \enskip \delta \preceq 1 - \alpha\} \\
        &
            \begin{dcases}
            \mcal{C}(f, x) = \mcal{C}(x, \alpha + \delta) &\, (\propA{}) \\
            \mcal{C}(f, x) = \mcal{C}(x, \mbf{1} - \delta) &\, (\propB{})
            \end{dcases}
\end{split}
\end{align}
This gives us a way to quantify the extent (radii) to which \(\alpha\) satisfies \(P_{\mrm{suff}}\) or \(P_{\mrm{necc}}\) with respect to \(f\) and \(x\), which is useful for analyzing the quality of solutions proposed by different feature attribution methods \(\mcal{M}\).
We next consider the search problem.
Given some model \(f\), input \(x\), and radius \(r\), the search for some explanation \(\alpha\) can be formulated as the following problem:
\begin{align}\label{prob:search}
\begin{split}
    \text{find} &\quad \alpha \\
    \text{subject to}
        &\quad \forall \delta \in \{\delta : \norm{\delta}_1 \leq r, \enskip \delta \preceq 1 - \alpha\} \\
        &
        \begin{dcases}
        \mcal{C}(f,x) = \mcal{C}(x, \alpha + \delta) &\, (\propA{}) \\
        \mcal{C}(f,x) = \mcal{C}(x, \mbf{1} - \delta) &\, (\propB{})
        \end{dcases}
\end{split}
\end{align}
We have formulated the analysis problem~\eqref{prob:analysis} as an optimization problem, and the search problem~\eqref{prob:search} as a feasibility problem.
These are done so for convenience of presentation, and other related formulations are also valid.




==> old/introduction_1.tex <==
\section{Introduction}
\label{sec:introduction}

Modern machine learning models achieve remarkable performance in tasks ranging from image classification and natural language processing, but are notoriously black-box in their decision-making.
The primary reasons for opacity are complexity and size, which push them beyond the reach of contemporary automated verification and analysis techniques~\cite{liu2021algorithms,albarghouthi2021introduction,brix2023first}.
Any analysis method must contend with fundamental hardness~\cite{blum1993training,katz2017reluplex}, and often trade-off precision to achieve scalability~\cite{gehr2018ai2,wang2021beta}.
For modern models, \emph{explanations} are therefore integral to understanding their behavior at a human-comprehensible abstraction.
At its core, explanations aim to accurately and succinctly describe \emph{why} a decision was made, often with human comprehension as the objective~\cite{adadi2018peeking}.
However, what constitutes the form and content of a \emph{good} explanation is highly context-dependent~\cite{nauta2022anecdotal}, as it varies by the problem domain (e.g. vision vs language), the objective function (e.g. classification vs regression), and the intended audience (e.g. beginners vs experts).
In this work we study a class of explanation methods that are popular due to their simplicity and applicability, called \emph{feature attributions}~\cite{smilkov2017smoothgrad,ribeiro2016should,lundberg2017unified,sundararajan2017axiomatic}.


The goal of feature attribution is to identify the explanatory features of an input.
Let \(f : \mcal{X} \to [0,1]^K\) be a model that maps inputs in \(\mcal{X} = \mbb{R}^{n}\) to \(K\) logits, where the class of an input \(x \in \mcal{X}\) is taken to be the largest coordinate of \(y = f(x)\).
We take feature attributions of \(x\) with respect to \(f\) to be binary
\footnote{
    Binary feature attribution is also known as \emph{feature selection}~\cite{li2017feature}.
    In general one may take \(\alpha \in \mbb{R}^{n}\).
    % and remark that in general feature attributions may take on continuous values in \(\mbb{R}^{n}\).
}
vectors \(\alpha \in \{0,1\}^n\), and we say that \(\alpha\) \emph{explains} \(x\) if \(f(x)\) and \(f(x \odot \alpha)\) have the same class, where \(\odot : \mbb{R}^n \times \mbb{R}^n \to \mbb{R}^n\) is the element-wise vector product.
This format lends itself to a simple interpretation:
if \(\alpha_i = 1\), we say that \(x_i\) is \emph{explanatory} of the prediction; if \(\alpha_i = 0\), we say that \(x_i\) is \emph{non-explanatory}.
Directly evaluating \(\alpha\) on \(f\) avoids the challenge of constructing faithful surrogate explanation models and is particularly appealing in domains like image classification, since one intuitively expects that a modified image with only the important (explanatory) portions shown and everything else black (zero) should cause the classifier to confidently yield the intended prediction.
Indeed, modern architectures like Vision Transformer~\cite{dosovitskiy2020image} can perform accurate image classification with only a fraction of the original image present.



A rich family of explanation properties is naturally expressible over binary \(\alpha\).
Of these, our primary focus is on \emph{robustness}, and we show that this can encode certain notions of \emph{sufficiency} and \emph{necessity}: are the explanatory \(x_i\) enough to explain the prediction (sufficient), and is this collection in some sense minimal (necessary).
However, \textbf{existing feature attribution methods are not robust}, which in turn makes it challenging to certify other explanation properties.
To motivate the importance of robustness, consider Figure~\ref{fig:non-robust}, in which we use \(\alpha\) generated by SHAP~\cite{lundberg2017unified} and take \(f\) to be the Vision Transformer~\cite{dosovitskiy2020image}.
Although \(\alpha\) explains \(x\), a small perturbation of \(\alpha + \delta\) causes misclassification to a very different class.
The lack of robust explanations is a problem for interpretability because it means that such \(\alpha\) are only a small perturbation away from explaining some other class, thereby making it harder for users to trust the results.


\input{figures/non-robust}


The main difficulty is that remarkably little can be guaranteed of \(f\), which often need to be highly expressive and complicated in order to attain high accuracies on tasks in vision and language.
In recent years, \emph{randomized smoothing}~\cite{cohen2019certified,yang2020randomized} has emerged as a promising suite of techniques for robustifying classifiers while preserving competitive accuracies.
Concretely, the smoothed classifier \(\tilde{f} : \mcal{X} \to [0,1]^K\) is endowed with a non-vacuous Lipschitz constant, which we adapt to certify the robustness properties of \(\alpha \mapsto \tilde{f}(x \odot \alpha)\) in constant time.
Although randomized smoothing is the only known set of techniques with demonstrated scalability to very large models, many common variants have two critical drawbacks.
First, despite strong scalability, they may still require high sample complexity due to the curse of dimensionality~\cite{kumar2020curse} --- meaning that a large number of model evaluations is still needed to ensure accurate and precise Lipschitz constant guarantees.
Second, many existing techniques use \emph{additive noise}, which cannot be naively applied to our setting as it would cause \emph{information leakage}, which we illustrate in Section~\ref{sec:additive-info-leak}.
Any smoothing technique for our setting must therefore overcome these two drawbacks.


In this work we study how to provably establish non-trivial guarantees for binary feature attributions.
To do this, we present conditions of sufficiency and necessity for \(\alpha\) in the language of robustness, and employ smoothing techniques to enforce a Lipschitz constant on \(f\).
The latter presents the main technical challenge, as we must develop a smoothing method that has both low sample complexity and no information leakage.
We call our smoothing method \dname{}, and we derive it by first constructing a non-additive randomized method \sname{} that has similar smoothness properties as its additive variants and no information leakage.
We then discretize \sname{} into \dname{}, yielding similar Lipschitz guarantees at the benefit of a significantly smaller sample complexity.
Moreover, \dname{} also does not information leak, meaning that a \dname{}-smoothed \(f\) is well-suited to establishing provable guarantees on feature attributions.
In summary, our contributions are as follows:
\begin{itemize}

    \item We first introduce \sname{}, a randomized smoothing technique with non-vacuous Lipschitz constants and no information leak.
    We then derandomized \sname{} to develop our main smoothing method, \dname{}, enabling a lower sample complexity that scales proportional to a discretization parameter.

    \item We show how \dname{} can be easily combined with existing feature attribution methods to yield binary feature attributions with provable guarantees of robustness by construction.

    \item We present numerical experiments on vision and language models that demonstrate the effectiveness of \dname{} in yielding non-trivial guarantees without significantly sacrificing accuracy.
    Moreover, our experiments hint at unexplored potentials for our method, as we observe \emph{empirical} guarantees much stronger than our provable ones.

\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Related Works}

For extensive surveys on explainability methods in machine learning, see~\cite{burkart2021survey,zhou2021evaluating,nauta2022anecdotal,lyu2022towards}.
% Below we list a sample of some works relevant to us.

A number of feature attribution methods have been proposed in the past decade.
Notable among these include Vanilla Gradients~\cite{simonyan2013deep}, SmoothGrad~\cite{smilkov2017smoothgrad}, Integrated Gradients~\cite{sundararajan2017axiomatic}, Grad-CAM~\cite{selvaraju2017grad},
Occlusion~\cite{zeiler2014visualizing},
LIME~\cite{ribeiro2016should},
SHAP~\cite{lundberg2017unified},
and their variants.
Of these, SHAP and Integrated Gradients are notable because they are rooted in axiomatic principles.
An in-depth analysis and variant of SHAP is proposed in~\cite{kwon2022weightedshap}, and Integrated Gradients are studied in detail in~\cite{lundstrom2022rigorous}.
The work of \cite{slack2021reliable} uses Bayesian inference to give confidence intervals over feature attribution scores, as many current methods are sampling-based.
The work of \cite{chattopadhyay2019neural} proposes viewing neural networks as causal models.
A systematic study of many common feature attribution methods is done in~\cite{han2022explanation}, which finds that many such methods perform black-box function approximation in some way.
Perhaps most similar to our approach is~\cite{blanc2021provably}, which studies classifiers of form \(f : \{0,1\}^n \to \{0,1\}\) and presents an algorithm for feature selection with succinctness and probabilistic precision guarantees.

In the absence of formal guarantees, empirical metrics are a common way to heuristically test the quality of feature attributions.
Many such metrics are discussed in~\cite{adebayo2018sanity,hooker2019benchmark,deyoung2019eraser,bastings2021will,rong2022consistent,zhou2022solvability,nauta2022anecdotal}.
The works of~\cite{adebayo2022post,zhou2022feature} propose augmentations to the dataset for sanity-checking the quality of feature attributions.
Feature attribution methods are not without their flaws.
Whether an attribution correctly identifies the relevant features is a well-known issue~\cite{yang2019benchmarking}.
Many feature attribution methods are also susceptible to adversarial attacks~\cite{slack2021counterfactual,ivankay2022fooling}.
As a negative result, \cite{bilodeau2022impossibility} prove that for sufficiently rich model classes, many feature attribution methods can provably fail to do better than random guessing.





==> old/introduction_2.tex <==
\section{Introduction}
\label{sec:introduction}


% Modern machine learning models are incredibly powerful but notoriously black-box.
% For all their achievements in image classification, natural language processing, and other challenging tasks, the internal decision-making steps are hard to interpret and analyze at scale.
% The primary reasons for this are the mathematical complexity and sheer size that push such models beyond the reach of contemporary automated verification and analysis~\cite{liu2021algorithms,albarghouthi2021introduction,brix2023first,katz2017reluplex,gehr2018ai2,wang2021beta}.
% Without a clear understanding of behavior, even the best-performing models face serious concerns of trust and reliability for use in safety and mission-critical settings.

% Any analysis method must contend with fundamental hardness~\cite{blum1993training,katz2017reluplex} and often trade-off precision to achieve scalability~\cite{gehr2018ai2,wang2021beta}.
% ~\cite{burkart2021survey,zhou2021evaluating,nauta2022anecdotal,lyu2022towards,li2022interpretable}

Modern machine learning models are incredibly powerful but notoriously black-box.
For such complex models, \emph{explanations} have become increasingly important for understanding model behavior at a human-comprehensible abstraction.
Explanations aim to accurately and succinctly describe \emph{why} a decision was made, often with human comprehension as the objective~\cite{adadi2018peeking}.
What constitutes the form and content of a good explanation, however, is context-dependent~\cite{nauta2022anecdotal}, as it varies by the problem domain (e.g. vision vs language), the objective function (e.g. classification vs regression), and the intended audience (e.g. beginners vs experts).
In this work we study classification models with a focus on feature attributions methods~\cite{simonyan2013deep,smilkov2017smoothgrad,ribeiro2016should,lundberg2017unified,sundararajan2017axiomatic}, which are a popular class of explanation methods due to their simple form and applicability to diverse problem domains.


The goal of feature attribution is to identify the explanatory features of an input.
Many feature attribution methods, however \textbf{may not be meaningful} and \textbf{often lack formal guarantees}.
Many feature attribution methods do not soundly justify the rationale for their attribution scores (e.g. gradient saliency-based~\cite{simonyan2013deep,smilkov2017smoothgrad,selvaraju2017grad}); although some are rooted in axiomatic principles (e.g. Shapley valued-based~\cite{lundberg2017unified,sundararajan2020many,kwon2022weightedshap}), the chosen axioms may not correspond to good notions of interpretability~\cite{fryer2021shapley}.
Even so, it is rare for such explanation methods to study and guarantee what mathematical properties their attribution scores should satisfy with respect to the underlying model and input.
A lack of well-founded meaning and rigorous guarantees means that many feature attribution methods do not yield true explanations, and are at best heuristic conjectures of model behavior.

\input{figures/non-robust}

In this work we focus on ensuring formal guarantees for feature attributions.
A number of works have proposed empirical metrics for evaluating the quality of feature attributions with respect to some heuristic criteria~\cite{adebayo2018sanity,hooker2019benchmark,deyoung2019eraser,bastings2021will,rong2022consistent,zhou2022solvability,nauta2022anecdotal}.
Although these techniques may yield good performance on human-favored metrics, they cannot ensure formal guarantees with respect to model behavior.
In this work we show how to establish such guarantees.


One of the most well-studied guarantees is \textbf{robustness}~\cite{carlini2017towards,wong2018provable}, which was first investigated within the context of adversarial attacks on neural networks.
Robustness is also a desirable property for explanations, which we show in Figure~\ref{fig:non-robust}: without robustness, a minimally perturbed explanation might induce a very different class --- an undesirable quality.
Moreover, robustness over binary feature attributions naturally encodes a number of other properties (e.g. sufficiency and necessity), which we discuss in Section~\ref{sec:overview}.
To the best of our knowledge, robustness --- much less other properties --- have not been studied in the context of explainability.
Our work addresses this gap: we study how to analyze and generate provably robust feature attributions for any \emph{sufficiently smoothed} classifier.


% In recent years, \emph{randomized smoothing}~\cite{cohen2019certified,yang2020randomized} has emerged as a promising suite of techniques for robustifying classifiers while preserving competitive accuracies.
% Although randomized smoothing is the only known set of techniques with demonstrated scalability to very large models, many common variants have two critical drawbacks.
% First, they may still require high sample complexity due to the curse of dimensionality~\cite{kumar2020curse}.
% Second, many existing techniques use \emph{additive noise}, and so cannot be naively applied to our setting due to \emph{information leakage}, which we describe in Section~\ref{sec:additive-info-leak}.
% Any smoothing technique we use must therefore overcome these drawbacks.

% \red{AAAA}

% The main difficulty with formal guarantees is that remarkably little can be guaranteed of \(f\), which often need to be highly expressive and complicated in order to attain high accuracies on tasks in vision and language.
% In recent years, \emph{randomized smoothing}~\cite{cohen2019certified,yang2020randomized} has emerged as a promising suite of techniques for robustifying classifiers while preserving competitive accuracies.
% Concretely, the smoothed classifier \(\tilde{f} : \mcal{X} \to [0,1]^K\) is endowed with a non-vacuous Lipschitz constant, which we adapt to certify the robustness properties of \(\alpha \mapsto \tilde{f}(x \odot \alpha)\) in constant time.
% Although randomized smoothing is the only known set of techniques with demonstrated scalability to very large models, many common variants have two critical drawbacks.
% First, despite strong scalability, they may still require high sample complexity due to the curse of dimensionality~\cite{kumar2020curse} --- meaning that a large number of model evaluations is still needed to ensure accurate and precise Lipschitz constant guarantees.
% Second, many existing techniques use \emph{additive noise}, which cannot be naively applied to our setting as it would cause \emph{information leakage}, which we illustrate in Section~\ref{sec:additive-info-leak}.
% Any smoothing technique for our setting must therefore overcome these two drawbacks.

To do this, we use robustness to express condition like sufficiency and necessity, and employ techniques from smoothing techniques~\cite{cohen2019certified,yang2020randomized} to robustify the classifier.
Our smoothing method ensures that robustness on the feature attribution implies robustness on the original input, which we call attribution-input consistency~\ref{sec:attribution-input-consistency}.
These combined allow us to establish meaningful formal guarantees on feature attributions with respect to the smoothed model in constant time.
% Smoothing in particular presents the main technical challenge, as we need the smoothing method to be scalable to large models, have no \emph{information leakage} (Section~\ref{sec:additive-info-leak}), and achieve strong robustness without significantly degrading accuracy.
In summary, our contributions are as follows:
\begin{itemize}

    \item We present Multiplicative Smooting (\dname{}), a derandomized smoothing method with low sample complexity and strong Lipschitz constant guarantees, which also ensures that feature attribution robustness implies input robustness.

    \item We show how the robustness guarantees naturally express a number of desirable properties (e.g. sufficiency and necessity) over binary feature attributions.
    In particular, we show how such properties can be verified against a \dname{} classifier in constant time.

    \item We present numerical experiments on vision and language models that demonstrate the effectiveness of \dname{} in yielding non-trivial guarantees without significantly sacrificing accuracy.
    Moreover, our experiments hint at unexplored potentials for our method, as we observe empirical guarantees much stronger than our provable ones.

\end{itemize}

% We call our smoothing method \dname{}, and we derive it by first constructing a non-additive randomized method \sname{} that has similar smoothness properties as its additive variants and no information leakage.
% We then discretize \sname{} into \dname{}, yielding similar Lipschitz guarantees at the benefit of a significantly smaller sample complexity.
% Moreover, \dname{} also does not information leak, meaning that a \dname{}-smoothed \(f\) is well-suited to establishing provable guarantees on feature attributions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Related Works}

For extensive surveys on explainability methods in machine learning, see~\cite{burkart2021survey,zhou2021evaluating,nauta2022anecdotal,lyu2022towards,li2022interpretable}.
% Below we list a sample of some works relevant to us.

A number of feature attribution methods have been proposed in the past decade.
Notable among these include Vanilla Gradients~\cite{simonyan2013deep}, SmoothGrad~\cite{smilkov2017smoothgrad}, Integrated Gradients~\cite{sundararajan2017axiomatic}, Grad-CAM~\cite{selvaraju2017grad},
Occlusion~\cite{zeiler2014visualizing},
LIME~\cite{ribeiro2016should},
SHAP~\cite{lundberg2017unified},
and their variants.
Of these, SHAP and Integrated Gradients are notable because they are rooted in axiomatic principles.
Variants of SHAP are proposed in~\cite{sundararajan2020many,kwon2022weightedshap}, and Integrated Gradients are studied in detail in~\cite{lundstrom2022rigorous}.
The work of \cite{slack2021reliable} uses Bayesian inference to give confidence intervals over feature attribution scores, as many current methods are sampling-based.
The work of \cite{chattopadhyay2019neural} proposes viewing neural networks as causal models.
A systematic study of many common feature attribution methods is done in~\cite{han2022explanation}.
Perhaps most similar to our approach is~\cite{blanc2021provably}, which studies classifiers of form \(f : \{0,1\}^n \to \{0,1\}\) and presents an algorithm for feature selection with succinctness and probabilistic precision guarantees.

In the absence of formal guarantees, empirical metrics are a common way to heuristically test the quality of feature attributions.
Many such metrics are discussed in~\cite{adebayo2018sanity,hooker2019benchmark,deyoung2019eraser,bastings2021will,rong2022consistent,zhou2022solvability,nauta2022anecdotal}.
The works of~\cite{adebayo2022post,zhou2022feature} propose augmentations to the dataset for sanity-checking the quality of feature attributions.
Feature attribution methods are not without their flaws.
Whether an attribution correctly identifies the relevant features is a well-known issue~\cite{yang2019benchmarking}.
Many feature attribution methods are also susceptible to adversarial attacks~\cite{slack2021counterfactual,ivankay2022fooling}.
As a negative result, \cite{bilodeau2022impossibility} prove that for sufficiently rich model classes, many feature attribution methods can provably fail to do better than random guessing.





==> old/introduction_3.tex <==
\section{Introduction}
\label{sec:introduction}

Modern machine learning models are notoriously black-box, yet incredibly powerful at challenging classification tasks.
For effective adoption in critical settings like medical diagnosis~\cite{reyes2020interpretability,tjoa2020survey}, the presence of accurate and  insightful explanations of model behavior is especially important for making a well-informed decision.
One popular family of explanation methods for classification tasks are \emph{feature attributions}~\cite{simonyan2013deep,ribeiro2016should,lundberg2017unified,sundararajan2017axiomatic}.
Given a model and input, a feature attribution method generates a score for each input feature that denotes its importance to the overall prediction.
This form of explanation is popular due to its simplistic interpretation and applicability to diverse problem domains in vision~\cite{smilkov2017smoothgrad,buhrmester2021analysis}, language~\cite{zhang2014explicit,danilevsky2020survey}, and reinforcement learning~\cite{puri2019explain,he2021explainable}.



In this paper we consider the task of jointly classifying and explaining.
We call this \emph{classifying with feature attributions} (CFA): given an input, we would like to simultaneously generate both a classification and a feature attribution.
We focus on \emph{binary feature attributions} --- also known as feature selection --- wherein each feature is either marked as important (1), or not important (0).
The utility of this pairing is clear, but realizing CFA in a principled manner is highly non-trivial.
This is because many feature attribution methods \textbf{lack formal guarantees} with respect to the underlying model.
In particular, many feature attribution methods do not have \emph{robustness} guarantees, which we demonstrate in Figure~\ref{fig:non-robust}: slightly changing the feature attribution induces a classification flip, meaning that the altered attribution now explains some other very different class.
This lack of robustness is undesirable for users, since it implies that a barely perceptible perturbation can drastically alter the explanatory implications.


% Slightly changing the feature attribution should not so drastically alter the prediction.
% A lack of robustness in the feature attribution means that a minimally perturbed example may now instead explain some other very different class --- an undesirable property that may easily erode user trust.

% Moreover, robustness in the explanation is also a desirable property, and we show in Section~\ref{sec:overview} that a number of properties over explanations may be encoded as robustness properties, i.e. sufficiency and necessity.

Robustness in classification, in particular neural networks, is a major area of research~\cite{wong2018provable,gehr2018ai2}.
For binary feature attributions in particular, robustness is an attractive property, and we show in Section~\ref{sec:robustness-formulations} that it may naturally express a number of other useful properties.
Robustifying classifiers is well-studied, most notably through the use of randomized smoothing~\cite{cohen2019certified,yang2020randomized}.
However, most of the relevant results for smoothing and robustness in general are concerned with the input, rather than with respect to feature attributions.
This is an important distinction, as the primary technical challenge in a first-step towards realizing principled CFA is in generating explanations with certified robustness properties: the generated feature attributions should not be brittle, and its minor perturbations should all explain the same class.
We show in Section~\ref{sec:attribution-input-consistency} that naively applying common classes of smoothing techniques violates an important property that we call \emph{attribution-input consistency}, which ensures that robustness with respect to feature attributions meaningfully translates to robustness in the classification.
To the best of our knowledge, there is no existing literature that investigates feature attribution robustness in the context of rigorously provable guarantees.


\input{figures/non-robust}

In this work we study the task of jointly classifying and explaining an input with certifiable robustness guarantees.
We show that for classifiers with appropriate smoothness conditions, one can formally derive robustness guarantees with respect to feature attributions.
To achieve this smoothness condition, we introduce a novel smoothing method that we call Multiplicative Smoothing (\dname{}).
This technique is related to randomized smoothing~\cite{cohen2019certified,yang2020randomized}, is applicable to any classifier, and yields non-trivial robustness guarantees at only a slight penalty to accuracy.
Moreover, we incorporate derandomization techniques~\cite{levine2021improved} to overcome the high sample complexity traditionally associated with randomized smoothing~\cite{kumar2020curse}: our robustness guarantees are exact and not subject to probabilistic uncertainty.

The advantage of our approach is that we may apply \dname{} to \emph{any} off-the-shelf model, and then pair it with \emph{any} feature attribution method, such that they are jointly capable of CFA with robustness guarantees.
We show in Section~\ref{sec:smoothing} how to smooth any model with \dname{}, and we show in Section~\ref{sec:provable-guarantees} how to combine this smoothed model with any feature attribution method.
In summary, our contributions are as follows:

\begin{itemize}
    \item We consider the task of classifying with feature attributions (CFA) subject to certifiable robustness guarantees.
    We show that a number of desirable properties over binary feature attributions are naturally expressible in the language of robustness, and give a precise formalization of such properties.
    Particularly, if the classification model is sufficiently smooth, then one can enforce such robustness guarantees.

    \item We introduce a novel smoothing method applicable to any classifier that we call Multiplicative Smoothing (\dname{}).
    By applying derandomization technique, we overcome high sample complexity issues traditionally associated with randomized smoothing.
    Moreover, the derandomized nature of \dname{} means that our robustness guarantees are exact, and not subject to probabilistic uncertainty.
    

    \item We present numerical experiments on vision and lanugage models that demonstrate the effectiveness of \dname{} in yielding non-trivial robustness guarantees with only a slight accuracy penalty.
    Moreover, our experiments hint at strong practical potential for our method, as we observe empirical results far better than what may be conservatively provable.

\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Related Works}

For extensive surveys on explainability methods in machine learning, see~\cite{burkart2021survey,zhou2021evaluating,nauta2022anecdotal,lyu2022towards,li2022interpretable,bommasani2021opportunities}.
% Below we list a sample of some works relevant to us.

A number of feature attribution methods have been proposed in the past decade.
Notable among these include Vanilla Gradients~\cite{simonyan2013deep}, SmoothGrad~\cite{smilkov2017smoothgrad}, Integrated Gradients~\cite{sundararajan2017axiomatic}, Grad-CAM~\cite{selvaraju2017grad},
Occlusion~\cite{zeiler2014visualizing},
LIME~\cite{ribeiro2016should},
SHAP~\cite{lundberg2017unified},
and their variants.
Of these, SHAP and Integrated Gradients are notable because they are rooted in axiomatic principles.
Variants of SHAP are proposed in~\cite{sundararajan2020many,kwon2022weightedshap}, and Integrated Gradients are studied in detail in~\cite{lundstrom2022rigorous}.
The work of \cite{slack2021reliable} uses Bayesian inference to give confidence intervals over feature attribution scores, as many current methods are sampling-based.
The work of \cite{chattopadhyay2019neural} proposes viewing neural networks as causal models.
A systematic study of many common feature attribution methods is done in~\cite{han2022explanation}.
Perhaps most similar to our approach is~\cite{blanc2021provably}, which studies classifiers of form \(f : \{0,1\}^n \to \{0,1\}\) and presents an algorithm for feature selection with succinctness and probabilistic precision guarantees.

In the absence of formal guarantees, empirical metrics are a common way to heuristically test the quality of feature attributions.
Many such metrics are discussed in~\cite{adebayo2018sanity,hooker2019benchmark,deyoung2019eraser,bastings2021will,rong2022consistent,zhou2022solvability,nauta2022anecdotal}.
The works of~\cite{adebayo2022post,zhou2022feature} propose augmentations to the dataset for sanity-checking the quality of feature attributions.
Feature attribution methods are not without their flaws.
Whether an attribution correctly identifies the relevant features is a well-known issue~\cite{yang2019benchmarking}.
Many feature attribution methods are also susceptible to adversarial attacks~\cite{slack2021counterfactual,ivankay2022fooling}.
As a negative result, \cite{bilodeau2022impossibility} prove that for sufficiently rich model classes, many feature attribution methods can provably fail to do better than random guessing.

Related to feature attributions are \emph{data attributions}~\cite{koh2017understanding,ilyas2022datamodels,park2023trak}, which seek to assign importance values to different points of training data.



==> old/introduction_4.tex <==
\section{Introduction}
\label{sec:introduction}

Modern machine learning models are incredibly powerful at challenging prediction tasks, but notoriously black-box in their decision-making.
One can therefore achieve impressive performance without fully understanding \emph{why}.
In settings where accurate and well-justified decisions are important, however, such power without proof is not sufficient --- particularly in contexts like medical diagnosis~\cite{reyes2020interpretability,tjoa2020survey} and legal analysis~\cite{wachter2017counterfactual,bibal2021legal}.
In order to fully wield the power of such models while ensuring reliability and trust, a user needs accurate and insightful \emph{explanations} of model behavior.
At its core, explanations aim to accurately and informatively describe why a decision was made, often with human comprehension as the objective~\cite{adadi2018peeking}.
What constitutes the form and content of a \emph{good} explanation is highly context-dependent, as it varies by the problem domain (e.g. vision vs language), the objective function (e.g. classification vs regression), and the intended audience (e.g. beginners vs experts).
For surveys on the myriad of explanation methods proposed over the past decade, see~\cite{burkart2021survey,zhou2021evaluating,nauta2022anecdotal,lyu2022towards,li2022interpretable,bommasani2021opportunities}.


Importantly, an explanation should satisfy formal guarantees~\cite{nauta2022anecdotal}.
Such guarantees provide mathematical certainty to the relationship between the explanation, input, and model --- allowing the user the accurately abstract, interpret, and manipulate the explainer outputs.
An absence of formal guarantees means that such explanations are not necessarily \emph{faithful}~\cite{nauta2022anecdotal,lyu2022towards} to the underlying model.
That is, such explanations may not truly reflect model behavior, and are therefore at best plausible heuristics and at worst completely misleading.
Unfortunately, many proposed explanation methods in literature lack such formal guarantees and so fall into this category.
The primary challenge is that an effective explanation method must contend with often conflicting requirements: it must be sufficiently useful to a human user, satisfy formal guarantees, and also simultaneously be model-agnostic.
% The latter two are especially challenging, 
% These simultaneous demands are often conflicting for all but the simplest settings, and for complex neural networks especially, achieving all three is especially challenging.



In this paper we focus on the problem of jointly constructing a classifier-explainer pair subject to formal guarantees.
Given an input, we simultaneously generate both a classification and a feature attribution, such that the feature attribution satisfies formal mathematical properties with respect to the underlying model behavior.
We introduce this problem in generality in Section~\ref{sec:overview}, and for this work we focus on \emph{binary feature attributions} --- also known as feature selection~\cite{li2017feature} --- wherein each feature is either marked as important (1), or not important (0).
Feature attributions~\cite{simonyan2013deep,ribeiro2016should,lundberg2017unified,sundararajan2017axiomatic} are especially popular due to their simplistic interpretation and applicability to diverse problem domains in vision~\cite{smilkov2017smoothgrad,buhrmester2021analysis}, language~\cite{zhang2014explicit,danilevsky2020survey}, and reinforcement learning~\cite{puri2019explain,he2021explainable}.
However, many feature attribution methods lack formal guarantees: one can assign an importance score based on a number of criteria~\cite{simonyan2013deep,lundberg2017unified,selvaraju2017grad}, but it is often unclear how such choices are in fact semantically meaningful (i.e. useful to humans) 
~\cite{adebayo2018sanity,zhou2022solvability} or truly indicative of model behavior (i.e. formal guarantees).
% The focus of our work is on the latter, and we show how to construct a classifier-explainer pair with formal guarantees given \emph{any} existing classifier and feature attribution method.


Our key insight is that if the model satisfies certain robustness conditions, then one can guarantee notions of explanation \emph{stability}, which we expand on in Section~\ref{sec:overview}.
Robustness in classification, in particular neural networks, has been a major area of research over the past decade~\cite{carlini2017towards,wong2018provable,gehr2018ai2,wang2021beta}.
Works in randomized smoothing~\cite{cohen2019certified,yang2020randomized} demonstrate that it is possible to robustify \emph{any} classifier, and at present remains one of the only techniques scalable to very large classifiers without much compromise to performance.
However, naive applications of randomized smoothing to our setting is not sufficient, as the naively smoothed model may not satisfy an important property that we call \emph{attribution-input consistency} --- which we detail in Section~\ref{sec:attribution-input-consistency}.
For this, we introduce a new smoothing method that we call Multiplicative Smoothing (\dname{}), which preserves this property and achieves non-trivial robustness guarantees at only a slight penalty to accuracy.
Moreover, we apply derandomization techniques~\cite{levine2021improved} to ensure that \dname{} avoids a high sample complexity that plagues many common smoothing methods~\cite{kumar2020curse}.
As such, the formal guarantees we can obtain with \dname{} are in fact deterministic and not subject to probabilistic uncertainty.

The advantage of our approach is that we may apply \dname{} to \emph{any} off-the-shelf model, and then appropriately pair it with \emph{any} existing feature attribution method, such that this pair now satisfies formal guarantees.
We show in Section~\ref{sec:smoothing} how to smooth any model with \dname{}, and we show in Section~\ref{sec:provable-guarantees} how to combine this smoothed model with any feature attribution method, subject to explanation stability guarantees.
In summary, our contributions are as follows:

\begin{itemize}
    \item We consider the task of jointly classifying and explaining subject to formal guarantees.
    We focus on binary feature attributions, and show that if the classifier satisfies certain robustness properties, then one can ensure notions of stability in the explanation.

    % \item We consider the task of classifying with feature attributions (CFA) subject to certifiable robustness guarantees.
    % We show that a number of desirable properties over binary feature attributions are naturally expressible in the language of robustness, and give a precise formalization of such properties.
    % Particularly, if the classification model is sufficiently smooth, then one can enforce such robustness guarantees.

    \item We introduce a novel smoothing method applicable to any classifier that we call Multiplicative Smoothing (\dname{}).
    By applying derandomization technique, we overcome high sample complexity issues traditionally associated with randomized smoothing.
    Moreover, the derandomized nature of \dname{} means that our robustness guarantees are exact, and not subject to probabilistic uncertainty.
    
    \item We present numerical experiments on vision and language models that demonstrate the effectiveness of \dname{} in yielding non-trivial robustness guarantees with only a slight accuracy penalty.
    Moreover, our experiments hint at strong practical potential for our method, as we observe empirical results far better than what may be conservatively provable.

\end{itemize}



==> old/introduction_5.tex <==
\section{Introduction}
\label{sec:introduction}

Modern machine learning models are incredibly powerful at challenging prediction tasks, but notoriously black-box in their decision-making.
One can therefore achieve impressive performance without fully understanding \emph{why}.
In settings like like medical diagnosis~\cite{reyes2020interpretability,tjoa2020survey} and legal analysis~\cite{wachter2017counterfactual,bibal2021legal}, where accurate and well-justified decisions are important, such power without proof is insufficient.
In order to fully wield the power of such models while ensuring reliability and trust, a user needs accurate and insightful \emph{explanations} of model behavior.
At their core, explanations aim to accurately and informatively describe why a decision was made, often with human comprehension as the objective~\cite{adadi2018peeking}.
What constitutes the form and content of a \emph{good} explanation is highly context-dependent, as it varies by the problem domain (e.g. vision vs language), the objective function (e.g. classification vs regression), and the intended audience (e.g. beginners vs experts).
For surveys on the many explanation methods proposed over the past decade, see~\cite{burkart2021survey,zhou2021evaluating,nauta2022anecdotal,lyu2022towards,li2022interpretable,bommasani2021opportunities}.




One popular family of explanation methods is \emph{feature attributions}~\cite{simonyan2013deep,ribeiro2016should,lundberg2017unified,sundararajan2017axiomatic}.
Given a model and input, a feature attribution method generates a score for each input feature that denotes its importance to the overall prediction.
To measure feature importance, a host of metrics are explored in the literature, including saliency sensitivity~\cite{simonyan2013deep,smilkov2017smoothgrad,sundararajan2017axiomatic}, surrogate models that are ``interpretable'' by construction~\cite{ribeiro2016should,agarwal2021towards}, Shapley values~\cite{lundberg2017unified,sundararajan2020many,kwon2022weightedshap}, and many others~\cite{selvaraju2017grad,han2022explanation,nauta2022anecdotal}.
Feature attributions are popular in diverse problem domains like vision~\cite{smilkov2017smoothgrad,buhrmester2021analysis}, language~\cite{zhang2014explicit,danilevsky2020survey}, and reinforcement learning~\cite{puri2019explain,he2021explainable}.
For instance consider Figure~\ref{fig:non-stable}, in which the Vision Transformer~\cite{dosovitskiy2020image} classifier predicts the full image (left) as ``Goldfish''.
We then use a feature attribution method like LIME~\cite{ribeiro2016should} to get a ranking of each feature by importance and select the top-25\%, for which the masked image (middle) is consistently predicted as ``Goldfish''.
However, additionally including a single patch of features (right) alters the prediction confidence so much that it now yields ``Axolotl''.
This suggests that the explanation is brittle~\cite{ghorbani2019interpretation}, as small changes easily cause it to now induce some other class.
In this paper we study how to overcome such behavior by analyzing the \emph{stability} of an explanation: we consider an explanation to be stable if once the explanatory features are included, the addition of more features does not change the prediction.

\input{figures/non-stable}

Stability implies that the selected features are enough to explain the prediction~\cite{brown2009new,chen2018learning,li2020survey}, and that this selection maintains strong explanatory power even in the presence of additional information~\cite{ghorbani2019interpretation,boopathy2020proper}.
Similar properties are studied in literature and identified as useful for interpretability~\cite{nauta2022anecdotal}, and we emphasize that our main focus is on analyzing and achieving provable guarantees.
Stability guarantees in particular are useful as they allow one to accurately predict how model behavior varies with the explanation.
Given a stable explanation, one can include more features, e.g. adding context, while maintaining confidence in the consistency of the underlying explanatory power.
Crucially, we observe that such guarantees only make sense when jointly considering the model and explanation method: the explanation method necessarily depends on the model to yield an explanation, and stability is then evaluated with respect to the model.


% We remark that similar notions to our definition of stability are studied in literature, and we refer to~\cite{nauta2022anecdotal} for extensive surveys.

% Thus far, there has been little work on obtaining feature attributions with formal guarantees in a way that is computationally tractable and meaningfully explanatory.

Thus far, existing work on feature attributions with formal guarantees face challenges with computational tractability and explanatory utility.
Such methods tend to take an axiomatic approach: some desirable properties (axioms) are specified, and the attribution satisfies these by construction.
Computing Shapley values~\cite{shapley1953value} is one popular approach and was explored in SHAP~\cite{lundberg2017unified} for explainable machine learning --- however computing these values is expensive, and this has motivated works for fast approximations~\cite{jethani2021fastshap,pelegrina2022k}.
Another well-known method is Integrated Gradients~\cite{sundararajan2017axiomatic}, which uses path integrals to aggregate gradient sensitivity information with respect to some axioms --- however it is not clear that these axioms are relevant to meaningful explanations, and the meaningfulness of gradient saliency-based approaches in general has 
 long been called into question~\cite{kindermans2019reliability}.
Beyond axiomatic approaches, many feature attribution methods use metrics that appear reasonable but may not reliably reflect useful model behavior, a common and known limitation~\cite{zhou2022feature}.
Instead, a popular approach is to evaluate the quality of an attribution with respect to some heuristics of quality~\cite{adebayo2018sanity,hooker2019benchmark,deyoung2019eraser,bastings2021will,rong2022consistent,zhou2022solvability}, such as the leave-one-out error~\cite{weston2000feature,lin2018convolutional}.
However, such evaluations are not substitutes for formal guarantees: an absence of which means that the explanation is at best a plausible guess, and at worst completely misleading~\cite{jacovi2020towards} about model behvaior.

% This is especially a problem, as an explanation method not faithful to the underlying model will at best hallucinate plausible-seeming guesses of behavior, and at worst be completely misleading~\cite{jacovi2020towards}.


In this paper we study how to construct explainable models with provable stability guarantees.
We jointly consider the classification model and explanation method, and present a formalization for studying such properties that we call \emph{explainable models}.
We focus on \emph{binary feature attributions}~\cite{li2017feature} wherein each feature is either marked as explanatory (1) or not explanatory (0).
We present a method to solve this problem, which is inspired by techniques from adversarial robustness, in particular randomized smoothing~\cite{cohen2019certified,yang2020randomized}.
Our method can take \emph{any} off-the-shelf classifier and feature attribution method to efficiently yield an explainable model that satisfies provable stability guarantees.
In summary, our contributions are as follows:

\begin{itemize}

    \item We formalize stability as a key property for binary feature attributions and study this in the framework of explainable models.
    We prove that relaxed variants of stability are guaranteed if the model is sufficiently Lipschitz with respect to the masking of features.

    % present explainable models as a framework for jointly analyzing the model and explanation.

    \item To achieve the sufficient Lipschitz conditions, we develop a smoothing method called Multiplicative Smoothing (\mus{}).
    We show that \mus{} achieves strong smoothness conditions, overcomes key theoretical and practical limitations of standard smoothing techniques, and can be integrated with any classifier and feature attribution method.

    \item We evaluate \mus{} on vision and language models along with different feature attribution methods.
    We demonstrate that \mus{}-smoothed explainable models achieve strong stability guarantees at a small cost to accuracy.
    
    % \item We evaluate \mus{} on the Vision Transformer and ResNet50 vision and RoBERTa language models over the ImageNet1K and TweetEval datasets along with feature attribution methods in vanilla gradient saliency, LIME, SHAP, and Integrated Gradients.
    % We demonstrate that \mus{}-smoothed models achieve strong stability guarantees at a small cost to accuracy.
    

\end{itemize}



==> old/overview_1.tex <==
\section{Overview}
\label{sec:overview}

In this section we present an overview of our smoothing mehtod, \dname{}.
Let \(f : \mcal{X} \to [0,1]^K\) be a model that maps inputs in \(\mcal{X} = \mbb{R}^{n}\) to \(K\) logits, where the class of an input \(x \in \mcal{X}\) is taken to be the largest coordinate of \(y = f(x)\).
We take feature attributions of \(x\) with respect to \(f\) to be binary
\footnote{
    Binary feature attribution is also known as \emph{feature selection}~\cite{li2017feature}.
    In general one may take \(\alpha \in \mbb{R}^{n}\).
    % and remark that in general feature attributions may take on continuous values in \(\mbb{R}^{n}\).
}
vectors \(\alpha \in \{0,1\}^n\), and we say that \(\alpha\) \emph{explains} \(x\) if \(f(x)\) and \(f(x \odot \alpha)\) have the same class, where \(\odot : \mbb{R}^n \times \mbb{R}^n \to \mbb{R}^n\) is the element-wise vector product.
This format lends itself to a simple interpretation:
if \(\alpha_i = 1\), we say that \(x_i\) is \emph{explanatory} of the prediction; if \(\alpha_i = 0\), we say that \(x_i\) is \emph{non-explanatory}.
Directly evaluating \(\alpha\) on \(f\) avoids the challenge of constructing faithful surrogate explanation models and is particularly appealing in domains like image classification, since one intuitively expects that a modified image with only the important (explanatory) portions shown and everything else black (zero) should cause the classifier to confidently yield the intended prediction.
Indeed, modern architectures like Vision Transformer~\cite{dosovitskiy2020image} can perform accurate image classification with only a fraction of the original image present.



A rich family of explanation properties is naturally expressible over binary \(\alpha\).
Of these, our primary focus is on \emph{robustness}, and we show that this can encode certain notions of \emph{sufficiency} and \emph{necessity}: are the explanatory \(x_i\) enough to explain the prediction (sufficient), and is this collection in some sense minimal (necessary).
However, \textbf{existing feature attribution methods are not robust}, which in turn makes it challenging to certify other explanation properties.
To motivate the importance of robustness, consider Figure~\ref{fig:non-robust}, in which we use \(\alpha\) generated by SHAP~\cite{lundberg2017unified} and take \(f\) to be the Vision Transformer~\cite{dosovitskiy2020image}.
Although \(\alpha\) explains \(x\), a small perturbation of \(\alpha + \delta\) causes misclassification to a very different class.
The lack of robust explanations is a problem for interpretability because it means that such \(\alpha\) are only a small perturbation away from explaining some other class, thereby making it harder for users to trust the results.

\red{AAAAA}

\input{figures/durt-overview}

In this section we present an overview of our \dname{} smoothing method.
Our approach is to derive a smoothed classifier \(\tilde{f} : \mcal{X} \to [0,1]^K\) from \(f\) that is robust yet accurate, such that binary attributions then satisfy robustness conditions with respect to \(\tilde{f}\).
An overview of \dname{} is shown in Figure~\ref{fig:durt-overview}, with a detailed presentation found in Section~\ref{sec:smoothing}.
In short, evaluating \(\tilde{f}(x)\) amounts to generating \(N\) ablated copies of \(x\) and taking their average evaluation on \(f\):
\begin{align*}
    \tilde{f}(x) = \frac{1}{N} \sum_{i = 1}^{N} f(x \odot \tilde{\alpha}^{(i)}),
    \qquad \tilde{\alpha}^{(i)} \sim \mcal{D}
\end{align*}
where \(\mcal{D}\) is some distribution on \(\{0,1\}^n\).
If we assume \(f\) outputs a one-hot vector denoting its classification, then the class of \(\tilde{f}(x)\) amounts to majority voting over the \(f(x \odot \tilde{\alpha}^{(i)})\).
By appropriately choosing \(\mcal{D}\), we control the Lipschitz constant of \(\tilde{f}\) to be small enough to enforce the robustness (i.e. sufficiency and necessity) of an explanation \(\alpha\).


Importantly, \dname{} is a non-additive smoothing method, and is therefore different from classical works like~\cite{cohen2019certified,yang2020randomized}.
This distinction is necessary because additive smoothing methods suffer from information leakage in our context, which we demonstrate in Section~\ref{sec:additive-info-leak}.
Our experiments in Section~\ref{sec:experiments} gives evidence that \dname{} allows us to achieve non-trivial robustness with minimal accuracy degradation.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Robustness Formulations of Sufficiency and Necessity}
\label{sec:robustness-formulations}

We now consider how to express the sufficiency and necessity of binary feature attributions in the language of robustness.
Our key insight is to phrase these as robustness with respect to the non-explanatory features.
First, we first define a partial ordering on binary vectors, writing \(\alpha \preceq \beta\) iff \(\alpha_i = 1\) implies \(\beta_i = 1\).
This notation lets us compare different attributions by feature inclusion.
In what follows we take \(f\) to be a classifier and \(x\) to be an input.

It is common to think of sufficiency as having enough information for an explanation.
We therefore propose to think of \(\alpha\) as sufficient explanation for \(x\) if (1) \(\alpha\) explains \(x\), and (2) \(\alpha\) is so explanatory of \(x\) that adding any (small) combination of other (i.e. non-explanatory) features will not change the classification.
This we formalize in the following.

\begin{definition}[Sufficiency]
    We say that \(\alpha \in \{0,1\}^n\) is \emph{sufficient with radius \(r\)} with respect to input \(x\) and classifier \(f\) if:
    \(\alpha\) and \(\alpha + \delta\) both explain \(x\), for all \(\delta \preceq \mbf{1} - \alpha\) with \(\norm{\delta}_1 \leq r\).
    We equivalently write \(P_{\mrm{suff}}(f, x, \alpha, r)\) to mean this property.
\end{definition}

Note that the ones vector \(\mbf{1} \in \{0,1\}^n\) is always a trivial and sufficient explanation of \(x\).
We prefer sparse \(\alpha\), however, with the intuition that typically only a small fraction of an input suffices to explain its classification.

Colloquially, an explanation is necessary if any other explanation is a superset.
That is, \(\alpha\) is necessary if \(\alpha \preceq \alpha'\) for all other explanations \(\alpha'\).
If \(\alpha\) is a necessary explanation, the non-explanatory features of \(\alpha\) may therefore be excluded from \(x\) in some amount while maintaining the prediction.
We formulate this in the following definition.

\begin{definition}[Necessity]
    We say that \(\alpha \in \{0,1\}^n\) is \emph{necessary with radius \(r\)} with respect to input \(x\) and classifier \(f\) if:
    \(\alpha\) and \(\mbf{1} - \delta\) both explain \(x\), for all \(\delta \preceq \mbf{1} - \alpha\) such that \(\norm{\delta}_1 \leq r\).
    We equivalently write \(P_{\mrm{necc}}(f, x, \alpha, r)\) to mean this property.
\end{definition}

Note that our formulation of sufficiency and necessity are both to do with perturbing the non-explanatory features of \(\alpha\).
As such, for large enough high radius of \(r = n - \norm{\alpha}_1\) the two definitions will in fact coincide.
We observe, however, that this rarely occurs in practice, since the radius of perturbation to which we can certify without sacrificing accuracy is much smaller than \(n - \norm{\alpha}_1\), as we usually consider sparse \(\alpha\) (e.g. SHAP-top25\%).



==> old/overview_2.tex <==
\section{Overview}
\label{sec:overview}

In this section we present an overview of our approach.
We first describe the classifying with feature attributions (CFA) task, and formalize the notation of classifier-attribution method pairings.
Crucially, if the classifier satisfies sufficient smoothness conditions, then it has certifiable robustness with respect to the feature attributions.
To do this, we next describe the general idea behind our smoothing method, \dname{}.
Finally, we show that two important properties over binary feature attributions, in particular notions of sufficiency and necessity, may be naturally expressed in the language of robustness.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Classifying with Feature Attributions}
\label{sec:cfa}

Let \(f : \mcal{X} \to [0,1]^K\) be a classification model that maps inputs in \(\mcal{X} = \mbb{R}^{n}\) to \(K\) logits (class probabilities), and take the class of \(x \in \mcal{X}\) is the largest coordinate of \(f(x) \in [0,1]^K\).
A binary feature attribution method \(\varphi : \mcal{X} \to \{0,1\}^n\) maps inputs \(x \in \mcal{X}\) to attributions of form \(\alpha \in \{0,1\}^n\).
We say that \(\alpha\) \emph{explains} \(x\) with respect to \(f\) if \(f(x)\) and \(f(x \odot \alpha)\) have the same class, where \(x \odot \alpha\) is a masking of \(x\) by \(\alpha\) via element-wise vector product.
Note that the ones vector \(\mbf{1} \in \{0,1\}^n\) trivially explains any \(x\).


% If \(\alpha_i = 1\) we say that \(x_i\) is \emph{explanatory} of the classification; otherwise if \(\alpha_i = 0\) we say that \(x_i\) is \emph{non-explanatory}.


When classifying with feature attributions (CFA), it is natural to pair the classification model \(f\) with the feature attribution method \(\varphi\).
We therefore the define a CFA pairing as \(\angles{f, \varphi}\) whose evaluation yields another pairing \(\angles{y, \alpha} = \angles{f, \varphi}(x)\) with logits \(y = f(x)\) and an attribution \(\alpha = \varphi(x)\) that explains \(x\).
We assume that \(\varphi\) has access to \(f\), and one may choose \(\varphi\) to be any feature attribution method~\cite{simonyan2013deep,ribeiro2016should,lundberg2017unified,sundararajan2017axiomatic,smilkov2017smoothgrad,sundararajan2020many,kwon2022weightedshap,selvaraju2017grad,zeiler2014visualizing}.
We more formally describe in Section~\ref{sec:provable-guarantees} a simple idea for transforming any off-the-shelf feature attribution method to be suitable for a CFA pairing. 


We now clarify the notion of robustness with respect to feature attributions.
Consider a CFA pairing \(\angles{f, \varphi}\) and some input \(x \in \mcal{X}\).
For robustness to hold, not only should the attribution \(\varphi(x)\) explain \(x\), but so should any other \(\alpha' \in \{0,1\}^n\) sufficiently close to \(\varphi(x)\).
More formally, this can be understood as robustness of the mapping \(g_x (\alpha) = f(x \odot \alpha)\), where we would like for \(g_x (\varphi(x))\) and \(g_x (\alpha')\) to yield the same class provided \(\varphi(x) \approx \alpha'\).
Note that because \(g_x\) is parametrized by \(x\), robustness is a local property: how much \(\alpha'\) and \(\varphi(x)\) may deviate is depenent on the choice of \(x\).
Crucially, however, the ability to formally guarantee any non-trivial robustness is dependent on the known properties of \(f\).
We show in Section~\ref{sec:ourname-smoothing} that any \(f\) smoothed by \dname{} has the sufficient properties.



% Given some input \(x\) and explanation \(\alpha\):
% if \(\alpha_i = 1\), we say that \(x_i\) is \emph{explanatory} of the prediction; otherwise if \(\alpha_i = 0\), we say that \(x_i\) is \emph{non-explanatory}.


\input{figures/durt-overview}

\subsection{Overview of MuS}

We now describe an overview of our smoothing method, \dname{}, which is able to transform any classifier \(f : \mcal{X} \to [0,1]^K\) into a smoothed classifier \(h : \mcal{X} \to [0,1]^K\) suitable for CFA with robustness guarantees in the feature attribution.
An overview of this method is shown in Figure~\ref{fig:durt-overview}.
Our key insight is that for a CFA pairing \(\angles{h, \varphi}\) to be robust in this sense, classification by \(h\) must be robust with respect to including or excluding features.
Given some \(x\) and let \(\tilde{x}\) be its noised variant where some features are dropped uniformly at random with probability \(1 - \lambda\), the evaluation \(h(x)\) is then taken to be:
\begin{align*}
    h(x) = \frac{1}{N} \sum_{i = 1}^{N} f (\tilde{x}^{(i)}),
    \qquad
    \tilde{x}^{(i)}_j
        = \begin{dcases}
            x_j, &\enskip \text{with probability \(\lambda\)} \\
            0, &\enskip \text{with probability \(1 - \lambda\)}
        \end{dcases},
    \qquad j = 1, \ldots, N
\end{align*}
where \(N\) random maskings of \(x\) are taken and \(\lambda \in [0,1]\) is the keep-probability of each feature.
In expectation, the mapping \(g_x (\alpha) = h(x \odot \alpha)\) is in fact \(\lambda\)-Lipschitz in the \(\ell^1\) norm (Theorem~\ref{thm:basic-smoothing}), and this process can in fact be derandomized (Theorem~\ref{thm:derand-smoothing}) with an appropriate choice of \(x^{(1)}, \ldots, x^{(N)}\).
Let \(g_A > g_B\) be the first and second largest logits of \(g_x (\alpha)\), then for any \(\alpha'\) such that \(\norm{\alpha' - \alpha}_1 \leq (g_A - g_B) / (2 \lambda)\), both \(\alpha\) and \(\alpha'\) explain \(x\), i.e. \(g_x (\alpha)\) and \(g_x (\alpha')\) yield the same class.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Robustness Formulations of Sufficiency and Necessity}
\label{sec:robustness-formulations}

We first present some notation for binary feature attributions.
Let \(\alpha, \beta \in \{0,1\}^n\), we define a partial order, writing \(\alpha \preceq \beta\) iff \(\alpha_i = 1\) implies \(\beta_i = 1\).
With respect to a given \(\alpha\), we say that \(i\) is \emph{explanatory} if \(\alpha_i = 1\), and otherwise that \(i\) is \emph{non-explanatory} if \(\alpha_i = 0\).
Moreover, let us write \(\mbf{0}, \mbf{1} \in \{0,1\}^n\) to mean the zeros and ones vectors, respectively.


The use of binary feature attributions means that a number of properties, in particular sufficiency and necessity, may be naturally expressed in the language of robustness.
We choose to frame these as robustness with respect to non-explanatory features of an attribution \(\alpha\), as it allows one to view sufficiency and necessity in terms of the \emph{inclusionary} and \emph{exclusionary} power of the explanation.


It is common to think of sufficiency as having enough information for an explanation.
That is, one can think of a sufficient \(\alpha\) as one which \emph{includes} enough relevant features, such that adding \emph{any} small enough combination does not change the classification.
We therefore formulate sufficiency as an additive robustness property in the following.

% We therefore think of \(\alpha\) as \emph{sufficient} for \(x\) if (1) \(\alpha\) explains \(x\), and (2) \(\alpha\) is so explanatory of \(x\) that adding any (small) combination of other (i.e. non-explanatory) features will not change the classification.
% Similarly, one can think of a sufficient \(\alpha\) as one which \emph{includes} enough relevant features to explain the classification.
% As such, we formulate sufficiency as an additive-robustness property
% This we formalize in the following.

\begin{definition}[Sufficiency] \label{def:sufficiency}
    Suppose \(\alpha \in \{0,1\}^n\) explains \(x\) with respect to \(f\).
    We say that \(\alpha\) is \emph{sufficient with radius \(r\)} when:
    for all \(\alpha' \succeq \alpha\), if \(\norm{\alpha' - \alpha}_1 \leq r\) then \(\alpha'\) also explains \(x\).
\end{definition}

Write \(P_{\mrm{suff}}(f, x, \alpha, r)\) to equivalently mean the property described above.
In particular, the example in Figure~\ref{fig:non-robust} violates sufficiency with radius \(1\).
Note also that the ones vector \(\mbf{1}\) is always a trivial and sufficient explanation of \(x\).
We prefer sparse \(\alpha\), however, with the intuition that typically only a small fraction of an input suffices to explain its classification.


Next, it is common to think of an explanation as necessary if it is in some sense minimal.
That is, one can judge necessity by how many features \(\alpha\) \emph{excludes}; any (small enough) combination of non-explanatory features removed from the whole input should not alter the prediction.
We therefore present necessity as a subtractive robustness property in the following.

\begin{definition}[Necessity] \label{def:necessity}
    Suppose \(\alpha \in \{0,1\}^n\) explains \(x\) with respect to \(f\).
    We say that \(\alpha\) is \emph{necessary with radius \(r\)} when:
    for all \(\alpha' \succeq \alpha\), if \(\norm{\mbf{1} - \alpha'}_1 \leq r\) then \(\alpha'\) also explains \(x\).
\end{definition}

We write \(P_{\mrm{necc}}(f, x, \alpha, r)\) to equivalently mean to property described above.
We remark that sufficiency and necessity are related in the sense that for a high enough radius of \(r = n - \norm{\alpha}_1\), the two definitions coincide --- though this rarely occurs in practice.
The key distinction is that in sufficiency, the perturbed \(\alpha'\) is close to \(\alpha\), whereas in necessity it is closed to \(\mbf{1}\).




% Note that our formulation of sufficiency and necessity are both to do with perturbing the non-explanatory features of \(\alpha\).
% As such, for large enough high radius of \(r = n - \norm{\alpha}_1\) the two definitions will in fact coincide.
% We observe, however, that this rarely occurs in practice, since the radius of perturbation to which we can certify without sacrificing accuracy is much smaller than \(n - \norm{\alpha}_1\), as we usually consider sparse \(\alpha\) (e.g. SHAP-top-25\%).
% \red{(Remark why focus on local properties?)}



==> old/overview_3.tex <==
\section{Overview}
\label{sec:overview}

In this section we provide an overview of our approach.
We first introduce the task of jointly classifying and explaining subject to guarantees in its full generality, before specializing to the case of binary feature attributions.
We then motivate and formalize the notion of explanation stability, and show that for binary attributions especially, this has natural analogues to the inclusion or exclusion of information.
Finally, we give an overview of our core computational technique in \dname{}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Jointly Classifying and Explaining with Formal Guarantees}

An \emph{explainable model} \(\angles{f, \varphi}\) is a pairing of a classifier \(f : \mcal{X} \to [0,1]^m\) and an explanation method \(\varphi : \mcal{X} \to \mcal{E}\), where \(\mcal{X}\) is the input space and \(\mcal{E}\) is the explanation space.
Given an input \(x \in \mcal{X}\), the evaluation \(f(x) \in [0,1]^m\) is a vector of \(m\) logits (class probabilities), with the class of \(f(x)\) taken to be the largest coordinate.
Given a predicate \(P\), we say that \(\angles{f, \varphi}\) satisfies \(P\) at \(x \in \mcal{X}\) if \(P(f, \varphi, x)\) holds.
If \(P(f, \varphi, x)\) holds for all \(x \in \mcal{X}\), then we say that \(\angles{f, \varphi}\) satisfies \(P\) globally.
The conceptual framework above is is presented in its full generality, and we remark that it captures many of the formulations studied in the literature~\cite{nauta2022anecdotal}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Formal Properties for Binary Feature Attributions}

We now specialize to the case of binary feature attributions, and subsequently focus on the input space \(\mcal{X} = \mbb{R}^n\) and the explanation space \(\mcal{E} = \{0,1\}^n\).
We will flexibly refer to binary vectors \(\alpha \in \{0,1\}^n\) as \emph{explanations} and \emph{feature attributions}.
If \(\alpha_i = 1\) we say that feature \(i\) is \emph{explanatory}, and otherwise if \(\alpha_i = 0\) we say that feature \(i\) is \emph{non-explanatory}.
For a classifier \(f\) and input \(x \in \mcal{X}\), we study \(\alpha\) through the evaluation of \(f(x \odot \alpha\)).
This approach has technical and semantic benefits.
First, directly evaluating \(\alpha\) on \(f\) avoids the challenge of constructing faithful surrogate models.
Second, in domains like image classification one intuitively expects that a masked image with only the important (explanatory) portions shown and everything else black (zero) should cause the classifier to yield the intended prediction.
Indeed, architectures like Vision Transformer~\cite{dosovitskiy2020image} can perform accurate image classification with only a fraction of the original image present.

For two inputs \(x, x' \in \mcal{X}\), we will write \(f(x) \cong f(x')\) to mean that \(f(x)\) and \(f(x')\) yield the same class.
This notion of classification consistency under masking leads to our first formal property.
\begin{definition}
We say that \(\angles{f, \varphi}\) is \emph{consistent} at \(x\) if \(f(x) \cong f(x \odot \varphi(x))\).
\end{definition}
We equivalently write \(P_{\mrm{cons}}(f, \varphi, x)\) to denote this property.
Also write \(\mbf{0}, \mbf{1} \in \{0,1\}^n\) to mean the zeros and ones vectors, respectively, and note that \(\mbf{1}\) is the trivially consistent explanation.



We say that an explanation to be \emph{stable} if it contains so many explanatory features, such that including any more features will not change the classification.
To motivate why stability is desirable, consider Figure~\ref{fig:non-robust}: adding a new feature to the explanation causes a classification change.
A lack of stability is undesirable, as it suggests that the present explanation is not sufficiently convincing --- adding new information may now cause it to explain some other very different class.
To formalize stability, we first introduce a partial ordering: for \(\alpha, \alpha' \in \{0,1\}^n\), we write \(\alpha \preceq \alpha'\) iff \(\alpha_i = 1\) implies \(\alpha_i ' = 1\).
That is, \(\alpha' \succeq \alpha\) iff \(\alpha'\) contains more information than \(\alpha\).


\begin{definition}
We say that \(\angles{f, \varphi}\) is \emph{stable} at \(x\) if \(f(x \odot \varphi(x)) \cong f(x \odot \alpha)\) for all \(\alpha \succeq \varphi(x)\).
\end{definition}

We equivalently write \(P_{\mrm{stab}}(f, \varphi, x)\) to denote this property, and note that \(\mbf{1}\) is a trivially stable explanation.
Moreover, stability at \(x\) also implies consistency at \(x\).
Observe that stability is closely tied to the notion of robustness, albeit the perturbation is additive.
Unfortunately, stability is a difficult property to enforce, as it requires the underlying model to satisfy a monotonicity-like behavior with respect to feature inclusion --- which is especially challenging for neural networks.
Checking stability without additional assumptions on \(f\) is also hard, as there are \(2^{n - \norm{\varphi(x)}_1}\) possible choices for \(\alpha \succeq \varphi(x)\), where \(\norm{\cdot}_1\) is the \(\ell^1\) norm.
\footnote{
On binary vectors \(\beta \in \{0,1\}^n\) we have \(\norm{\beta}_1 = \#\{i : \beta = 1\}\).
}
Instead, we focus on lower and upper-approximations to stability that we introduce next.

\begin{definition}
We say that \(\angles{f, \varphi}\) is \emph{\(r\)-incrementally stable} at \(x\) if \(f(x \odot \varphi(x)) \cong f(x \odot \alpha)\) for all \(\alpha \succeq \varphi(x)\) where \(\norm{\alpha - \varphi(x)}_1 \leq r\).
\end{definition}

We equivalently write \(P_{\mrm{stab}+} ^{r} (f, \varphi, x)\) to denote this form of additive stability, and note that this is a lower-approximation to \(P_{\mrm{stab}} (f, \varphi, x)\).
We also define the upper-approximation variant.

\begin{definition}
We say that \(\angles{f, \varphi}\) is \emph{\(r\)-decrementally stable} at \(x\) if \(f(x \odot \varphi(x)) \cong f(x \odot \alpha)\) for all \(\alpha \succeq \varphi(x)\) where \(\norm{\mbf{1} - \alpha}_1 \leq r\).
\end{definition}

We equivalently write \(P_{\mrm{stab}-} ^{r} (f, \varphi, x)\) to denote this form of subtractive stability.
Note that our definition means that decremental stability entails consistency, but this is not the case for incremental stability.
For a sufficiently large radius of \(r = \ceil{(n - \norm{\varphi(x)}_1) / 2}\), incremental and decremental stability together imply stability.



\input{figures/durt-overview}

\subsection{Overview of MuS}
\label{sec:dname-overview}

We now describe an overview of our smoothing method, \dname{}, which is able to transform any classifier \(f : \mcal{X} \to [0,1]^m\) into a smoothed classifier \(h : \mcal{X} \to [0,1]^m\) suitable for an explainable model with formal guarantees of stability-like properties.
We observe that robustness conditions on \(h\) suffice to ensure incremental and decremental stability.
To achieve robustness, we introduce a smoothing method, \dname{}, which we present in detail in Section~\ref{sec:ourname-smoothing}.
An overview of our smoothing method is shown in Figure~\ref{fig:durt-overview}.
Our key insight is that for an explainable model \(\angles{h, \varphi}\) to be robust in this sense, it suffices that \(h\) is robust with respect to the inclusion and exclusion of features.
Given some \(x\) and let \(\tilde{x}\) be its noised variant where some features are dropped uniformly at random with probability \(1 - \lambda\), the evaluation \(h(x)\) is then taken to be:
\begin{align}
\label{eq:dname-sketch}
    h(x) = \frac{1}{N} \sum_{i = 1}^{N} f (\tilde{x}^{(i)}),
    \qquad
    \tilde{x}^{(i)}_j
        = \begin{dcases}
            x_j, &\enskip \text{with probability \(\lambda\)} \\
            0, &\enskip \text{with probability \(1 - \lambda\)}
        \end{dcases},
    \qquad j = 1, \ldots, n
\end{align}
where \(N\) random maskings of \(x\) are taken and \(\lambda \in [0,1]\) is the keep-probability of each feature.
For all \(x \in \mcal{X}\), the mapping \(g(x, \alpha) = h(x \odot \alpha)\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm with respect to \(\alpha\) in expectation (Theorem~\ref{thm:basic-smoothing}), and this process can be derandomized (Theorem~\ref{thm:derand-smoothing}) with an appropriate choice of \(\tilde{x}^{(1)}, \ldots, \tilde{x}^{(N)} \in \mcal{X}\).
Let \(g_A > g_B\) be the first and second largest logits of \(g(x, \alpha)\), then for any \(\alpha'\) such that \(\norm{\alpha - \alpha'}_1 \leq (g_A - g_B) / (2 \lambda)\), we will have \(g (x, \alpha) \cong g(x, \alpha')\).





==> old/overview_4.tex <==
\section{Overview}
\label{sec:overview}

In this section we provide an overview of our approach.
We observe that formal guarantees for explanations must take into account both the model and explanation method, and for this we present in Section~\ref{sec:explainable-models} a pairing that we call \emph{explainable models}.
This formulation allows us to then describe the desired stability properties in Section~\ref{sec:stability-properties}.
We show in Section~\ref{sec:lipschitz-for-stability} that classifiers with sufficient Lipschitz smoothness with respect to the feature attribution allows us to provide provable guarantees of stability.
We then show in Section~\ref{sec:constructing-stable} that this can be coupled with any feature attribution method in order to generate an explainable model with stability guarantees.
Finally in Section~\ref{sec:ensuring-lipschitz} we give a high-level description of how our smoothing method \dname{} achieves the Lipschitz constants that enables these stability guarantees.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Explainable models}
\label{sec:explainable-models}

We first present explainable models as a formalism for rigorously studying explanations.
Let \(\mcal{X} = \mbb{R}^n\) be the space of inputs, a classifier \(f : \mcal{X} \to [0,1]^m\) maps inputs \(x \in \mcal{X}\) to \(m\) logits (class probabilities) that sum to \(1\), where the class of \(f(x) \in [0,1]^m\) is taken to be the largest coordinate.
Similarly, an explanation method \(\varphi : \mcal{X} \to \{0,1\}^n\) maps an input \(x \in \mcal{X}\) to an explanation \(\varphi(x) \in \{0,1\}^n\) that indicates which features are considered explanatory for the prediction \(f(x)\).
In particular, we may pick and adapt \(\varphi\) from among a selection of existing feature attribution methods like LIME~\cite{ribeiro2016should}, SHAP~\cite{lundberg2017unified}, and many others \cite{simonyan2013deep,sundararajan2017axiomatic,smilkov2017smoothgrad,sundararajan2020many,kwon2022weightedshap}, wherein \(\varphi\) may be thought of as a top-\(k\) feature selector.
Note that the selection of input features necessarily depends on the explanation method executing or analyzing the model, and so it makes sense to jointly study the model and explanation method: given a classifier \(f\) and explanation method \(\varphi\), we call the pairing \(\angles{f, \varphi}\) an \emph{explainable model}.
Given some \(x \in \mcal{X}\), the explainable model \(\angles{f, \varphi}\) maps \(x\) to both a prediction  and explanation.
We illustrate this idea in Figure~\ref{fig:explainable-model}, where \(\angles{f, \varphi}(x) \in [0,1]^m \times \{0,1\}^n\) couples the class probabilities and the feature attribution.

\input{figures/explainable-model}

For an input \(x \in \mcal{X}\), we will evaluate the quality of the binary feature attribution \(\varphi(x)\) through its masking on \(x\).
That is, we will study the behavior of the masked input \(x \odot \varphi(x) \in \mcal{X}\) with respect to \(f\), where \(\odot\) is the element-wise vector product.
To do this, we define a notion of \emph{prediction equivalence}: for two \(x, x' \in \mcal{X}\), we write \(f(x) \cong f(x')\) to mean that \(f(x)\) and \(f(x')\) yield the same class.
This now allows us to formalize the intuition that an explanation \(\varphi(x)\) should suffice to recover the prediction of \(x\) under \(f\).

\begin{definition}
The explainable model \(\angles{f, \varphi}\) is \emph{consistent} at \(x\) if \(f(x) \cong f(x \odot \varphi(x))\).
\end{definition}

Evaluating \(f\) on \(x \odot \varphi(x)\) this way lets us apply the model as-is and therefore avoids the challenge of constructing a surrogate model that is accurate to the original~\cite{alizadeh2020managing}.
Moreover, this approach is reasonable, especially in domains like vision --- where one intuitively expects that a masked image retaining only the important features should induce the intended prediction.
Indeed, architectures like Vision Transformer~\cite{dosovitskiy2020image} can maintain high accuracy with only a fraction of the image present~\cite{salman2022certified}.



Particularly, we would like for \(\angles{f, \varphi}\) to generate explanations that are stable and concise (i.e. sparse).
The former is our central guarantee, and is ensured through smoothing.
The latter implies that \(\varphi(x)\) has few ones entries, and is a desirable property since a good explanation should not contain too much redundant information.
However, sparsity is a difficulty property to enforce,
as this is contingent on the model having high accuracy with respect to heavily masked inputs.
For sparsity we present a simple heuristic in Section~\ref{sec:constructing-stable} and evaluate its effectiveness in Section~\ref{sec:experiments}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Stability properties of explainable models}
\label{sec:stability-properties}

Given an explainable model \(\angles{f, \varphi}\) and some \(x \in \mcal{X}\), stability means that the prediction does not change even if one adds more explanatory features to \(\varphi(x)\).
For instance, the model-explanation pair in Figure~\ref{fig:non-stable} is \emph{not} stable, as the inclusion of a single feature group (patch) changes the prediction.
To formalize this notion of stability, we first introduce a partial ordering: for \(\alpha, \alpha' \in \{0,1\}^n\), we write \(\alpha \succeq \alpha'\) iff \(\alpha_i \geq \alpha_i '\) for all \(i = 1, \ldots, n\).
That is, \(\alpha \succeq \alpha'\) iff \(\alpha\) includes all the features selected by \(\alpha'\).

\begin{definition} \label{def:stable}
The explainable model \(\angles{f, \varphi}\) is stable at \(x\) if \(f(x \odot \alpha) \cong f(x \odot \varphi(x))\) for all \(\alpha \succeq \varphi(x)\).
\end{definition}

Note that the constant explanation \(\varphi(x) = \mbf{1}\), the vector of ones, makes \(\angles{f, \varphi}\) trivially stable at every \(x \in \mcal{X}\), though this is not a concise explanation.
Additionally, stability at \(x\) implies consistency at \(x\).

Unfortunately, stability is a difficult property to enforce in general, as it requires that \(f\) satisfy a monotone-like behavior with respect to feature inclusion --- which is especially challenging for complex models like neural networks.
Checking stability without additional assumptions on \(f\) is also hard: if \(k = \norm{\varphi(x)}_1\) is the number of ones in \(\varphi(x)\), then there are \(2^{n-k}\) possible \(\alpha \succeq \varphi(x)\) to check for consistency.
This large space of possible \(\alpha \succeq \varphi(x)\) motivates us to instead examine \emph{relaxations} of stability.
We introduce lower and upper-relaxations of stability below.

\begin{definition} \label{def:inc-stable}
The explainable model \(\angles{f, \varphi}\) is incrementally stable at \(x\) with radius \(r\) if \(f(x \odot \alpha) \cong f(x \odot \varphi(x))\) for all \(\alpha \succeq \varphi(x)\) where \(\norm{\alpha - \varphi(x)}_1 \leq r\).
\end{definition}

Incremental stability is a lower-relaxation, since we are considering the addition of only a few features.
We also define the upper-relaxation variant, where we consider the inclusion of most features.

% ~\cite{wu2020towards}


\begin{definition} \label{def:dec-stable}
The explainable model \(\angles{f, \varphi}\) is decrementally stable at \(x\) with radius \(r\) if \(f(x \odot \alpha) \cong f(x \odot \varphi(x))\) for all \(\alpha \succeq \varphi(x)\) where \(\norm{\mbf{1} - \alpha}_1 \leq r\).
\end{definition}

Decremental stability is a subtractive form of stability, in contrast to the additive nature of incremental stability.
Note that our definition means that decremental stability entails consistency, but this is not the case for incremental stability.
% Moreover, this notion is related to \emph{incremental deletion}~\cite{nauta2022anecdotal}.
Furthermore, observe that for a sufficiently large radius of \(r = \ceil{(n - \norm{\varphi(x)}_1) / 2}\), incremental and decremental stability together imply stability.


\begin{remark}
Similar notions to the above have been proposed in literature, and we refer to~\cite{nauta2022anecdotal} for an extensive survey.
In particular, consistency is akin to \emph{preservation} and stability is similar to \emph{continuity}, except we are concerned with adding features.
In this regard, incremental stability is most similar to \emph{incremental addition} and decremental stability to \emph{incremental deletion}.
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Lipschitz smoothness entails stability guarantees}
\label{sec:lipschitz-for-stability}
% We now consider how to guarantee the aforementioned properties using Lipschitz smoothness.
For an explainable model \(\angles{f, \varphi}\) we introduce the mapping \(g(x, \alpha) = f(x \odot \alpha)\).
This reparametrizes our stability conditions as ensuring \(g(x, \alpha) \cong g(x, \varphi(x))\) when \(\alpha \succeq \varphi(x)\).
Taking inspiration from adversarial robustness literature, we will leverage smoothness properties of \(g\) to achieve such stability.
We aim to adapt a standard argument encapsulated in the following remark.

\begin{remark} \label{rem:g-lipschitz}
Let \(g_1, \ldots, g_m\) denote the coordinates of \(g : \mcal{X} \times \{0,1\}^n \to [0,1]^m\), and suppose for a given \(x \in \mcal{X}\) that each \(g_k\) satisfies:
\begin{align} \label{eq:lipschitz-in-alpha}
    \norm{g_k (x, \alpha) - g_k (x, \alpha')}_1
    \leq \lambda \norm{\alpha - \alpha'}_1,
    \quad \text{for all \(\alpha \in \{0,1\}^n\)},
\end{align}
for some given \(\lambda > 0\), then \(g(x, \alpha) \cong g(x, \alpha')\)
if \(\norm{\alpha - \alpha'}_1 \leq (g_A (x, \alpha) - g_B (x, \alpha)) / (2 \lambda)\).
Here \(g_A - g_B\) is referred to as the logit gap, where \(g_A, g_B\) denote the first and second largest logits:
\begin{align} \label{eq:logit-gap}
    k^\star = \underset{1 \leq k \leq m}{\mrm{argmax}}\, g_k (x, \alpha),
    \qquad g_A (x, \alpha) = g_{k^\star} (x, \alpha),
    \qquad g_B (x, \alpha) = \max_{i \neq k^\star} g_i (x, \alpha)
\end{align}
Equivalently, \eqref{eq:lipschitz-in-alpha} means that each \(g_k\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm with respect to \(\alpha\) for all \(x \in \mcal{X}\).
\end{remark}

In fact, Lipschitz smoothness is stronger assumption than necessary, as besides \(\alpha \succeq \varphi(x)\) it also imposes guarantees on \(\alpha \preceq \varphi(x)\).
Nevertheless, Lipschitz smoothness is useful as it is at present one of the only properties achievable and scalable to arbitrary models~\cite{yang2020randomized}.


\begin{remark}[Sketch of main result]
Consider an explainable model \(\angles{f, \varphi}\) where the mapping \(g(x, \alpha) = f(x \odot \alpha)\) satisfies the Lipschitz properties as described in Remark~\ref{rem:g-lipschitz}.
Then at any \(x \in \mcal{X}\), the radius of incremental stability \(r_{\mrm{inc}}\) and radius of decremental stability \(r_{\mrm{dec}}\) are respectively:
\begin{align*}
    r_{\mrm{inc}} = \frac{g_A (x, \varphi(x)) - g_B (x, \varphi(x))}{2 \lambda},
    \qquad
    r_{\mrm{dec}} = \frac{g_A (x, \mbf{1}) - g_B (x, \mbf{1})}{2 \lambda}.
\end{align*}
\end{remark}


% \red{(TWO-SIDED REMARK)} Importantly, this Lipschitz condition readily translates into stability guarantees.
% Suppose \(\angles{f, \varphi}\) is consistent at \(x\) and each \(g_k\) satisfies the Lipschitz conditions~\eqref{eq:lipschitz-in-alpha}, then \(\angles{f, \varphi}\) is incrementally stable at \(x\) with radius \(d(x,\alpha)/(2\lambda)\), and decrementally stable at \(x\) with radius \(d(x, \mbf{1}) / (2 \lambda)\).
% As such, if one can enforce a \(\lambda\)-Lipschitz condition on each coordinate of \(g\), then one can provably demonstrate that \(\angles{f, \varphi}\) satisfies stability properties.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Stable explainable models from Lipschitz classifiers}
\label{sec:constructing-stable}

Let \(f : \mcal{X} \to [0,1]^m\) be any classifier with Lipschitz properties previously described in~\eqref{eq:lipschitz-in-alpha}.
We now show how to take any feature attribution method \(\varphi_0 : \mcal{X} \to \mbb{R}^n\) to derive a binary feature attribution method \(\varphi\) that when coupled into \(\angles{f, \varphi}\) satisfies the desired stablity properties.
Note that the range of \(\varphi_0\) is \(\mbb{R}^n\) for full generality, where higher values will denote greater feature importance.

We begin with some desired incremental stability radius \(r_{\mrm{inc}}\) and decremental stability radius \(r_{\mrm{dec}}\), and an ordering on \([n]\) as given by \(\varphi_0 (x)\) (i.e. the highest logit is ordered first).
The construction of the valuation \(\varphi(x)\) is then a simple iterative algorithm:
we begin with \(\alpha = \mbf{0}\), and iteratively assign new entries \(\alpha_i \leftarrow 1\) where the index \(i\) is derived from the ordering of \(\varphi_0 (x)\).
When \(\angles{f, \varphi : x \mapsto \alpha}\) is checked to be consistent, incrementally stable with radius \(r_{\mrm{inc}}\), and decrementally stable with radius \(r_{\mrm{dec}}\) at \(x\), we terminate with the output \(\varphi(x) = \alpha\).
Note that one can use binary search to speed up this procedure.
We take \(\varphi_0\) as an existing feature attribution method like LIME~\cite{ribeiro2016should} or SHAP~\cite{lundberg2017unified}.

Note that the above method of constructing \(\varphi(x)\) does not impose guarantees of conciseness, in the way that we may guarantee stability through Lipschitz smoothness.
Instead, the ordering proposed by an existing feature attribution method serves as a heuristic about the order in which we may greedily construct \(\varphi(x)\).
We show in Section~\ref{sec:experiments} that some feature attributions (e.g. SHAP~\cite{lundberg2017unified}) tend to yield sparser selections on average compared to others (e.g. vanilla gradient saliency~\cite{simonyan2013deep}).


\red{(PREVIEW OF RESULTS HERE?)}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Ensuring Lipschitz smoothness with randomized smoothing}
\label{sec:ensuring-lipschitz}

We now give an overview of our core technical contribution in developing a smoothing method to ensure the Lipschitz properties of Section~\ref{sec:lipschitz-for-stability} --- thereby allowing for explainable models with provable stability guarantees.
We observe that the desired smoothness is with respect to the masking of features.
This means, however, that classical smoothing methods techniques~\cite{cohen2019certified,yang2020randomized} are not well-suited for our purpose, as they are primarily concerned with perturbing features rather than complete maskings.
This therefore motivates us to develop a novel smoothing method suitable for maskings.
We call our smoothing method Multiplicative Smoothing (\dname{}), where the goal is to begin with any \emph{base classifier} \(h : \mcal{X} \to [0,1]^m\) and then apply \dname{}-smoothing to derive a \emph{smoothed classifier} \(f : \mcal{X} \to [0,1]^m\) that satisfies the sufficient Lipschitz conditions.


\input{figures/durt-overview}

The main idea in \dname{} is to begin with an existing classifier \(h : \mcal{X} \to [0,1]^m\), and given \(x \in \mcal{X}\), we evaluate \(h\) on random maskings of \(x\).
This is illustrated in Figure~\ref{fig:durt-overview}.
More formally, given some \(x \in \mcal{X}\) we sample \(N\) random maskings \(\tilde{x}^{(1)}, \ldots, \tilde{x}^{(N)} \in \mcal{X}\), where each \(x^{(i)}\) is generated by dropping features from \(x\) uniformly at random with probability \(1 - \lambda\).
We refer to this fixed \(\lambda \in [0,1]\) as the \emph{smoothing parameter}, and the evaluation of the \dname{}-smoothed classifier \(f\) is then taken to be:
\begin{align}
\label{eq:dname-sketch-f}
    f(x) = \frac{1}{N} \sum_{i = 1}^{N} h (\tilde{x}^{(i)}),
    \qquad
    \tilde{x}^{(i)}_j
        = \begin{dcases}
            x_j &\text{with probability \(\lambda\)} \\
            0 &\text{with probability \(1 - \lambda\)}
        \end{dcases},
    \qquad j = 1, \ldots, n
\end{align}
We show that in expectation, for all \(x \in \mcal{X}\) each coordinate of the mapping \(g(x, \alpha) = f(x \odot \alpha)\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm with respect to the \(\alpha\) parameter (Theorem~\ref{thm:simple-smoothing}), i.e., each \(g_1, \ldots, g_m\) is Lipschitz in \(\alpha\).
Moreover, this process can be made deterministic, i.e. derandomized, with appropriate choice of noise (Theorem~\ref{thm:derand-smoothing}).
Thus, we can guarantee for all \(x\) that \(g(x, \alpha) \cong g(x, \alpha')\) provided \(\norm{\alpha - \alpha'}_1 \leq d(x, \alpha) / (2 \lambda)\).
Additionally, note that \(\lambda = 1\) recovers the original classifier, as feature dropping will happen with probability zero.
We will flexibly refer to \(\lambda\) as the smoothing parameter, the Lipschitz constant, or the feature keep-probability depending on the appropriate context.




==> old/overview_5.tex <==
\section{Overview}
\label{sec:overview}

We observe that formal guarantees for explanations must take into account both the model and explanation method, and for this we present in Section~\ref{sec:explainable-models} a pairing that we call \emph{explainable models}.
This formulation allows us to then describe the desired stability properties in Section~\ref{sec:stability-properties}.
We show in Section~\ref{sec:lipschitz-for-stability} that classifiers with sufficient Lipschitz smoothness with respect to the feature attribution allows us to provide provable guarantees of stability.
Finally in Section~\ref{sec:adapting-methods} we show how to adapt existing feature attribution methods into our explainable model framework.

% We then show in Section~\ref{sec:constructing-stable} that this can be coupled with any feature attribution method in order to generate an explainable model with stability guarantees.
% Finally in Section~\ref{sec:ensuring-lipschitz} we give a high-level description of how our smoothing method \dname{} achieves the Lipschitz constants that enables these stability guarantees.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Explainable models}
\label{sec:explainable-models}

We first present explainable models as a formalism for rigorously studying explanations.
Let \(\mcal{X} = \mbb{R}^n\) be the space of inputs, a classifier \(f : \mcal{X} \to [0,1]^m\) maps inputs \(x \in \mcal{X}\) to \(m\) logits (class probabilities) that sum to \(1\), where the class of \(f(x) \in [0,1]^m\) is taken to be the largest coordinate.
Similarly, an explanation method \(\varphi : \mcal{X} \to \{0,1\}^n\) maps an input \(x \in \mcal{X}\) to an explanation \(\varphi(x) \in \{0,1\}^n\) that indicates which features are considered explanatory for the prediction \(f(x)\).
In particular, we may pick and adapt \(\varphi\) from among a selection of existing feature attribution methods like LIME~\cite{ribeiro2016should}, SHAP~\cite{lundberg2017unified}, and many others \cite{simonyan2013deep,sundararajan2017axiomatic,smilkov2017smoothgrad,sundararajan2020many,kwon2022weightedshap}, wherein \(\varphi\) may be thought of as a top-\(k\) feature selector.
Note that the selection of input features necessarily depends on the explanation method executing or analyzing the model, and so it makes sense to jointly study the model and explanation method: given a classifier \(f\) and explanation method \(\varphi\), we call the pairing \(\angles{f, \varphi}\) an \emph{explainable model}.
Given some \(x \in \mcal{X}\), the explainable model \(\angles{f, \varphi}\) maps \(x\) to both a prediction  and explanation.
We illustrate this idea in Figure~\ref{fig:explainable-model}, where \(\angles{f, \varphi}(x) \in [0,1]^m \times \{0,1\}^n\) couples the class probabilities and the feature attribution.

\input{figures/explainable-model}

For an input \(x \in \mcal{X}\), we will evaluate the quality of the binary feature attribution \(\varphi(x)\) through its masking on \(x\).
That is, we will study the behavior of the masked input \(x \odot \varphi(x) \in \mcal{X}\) with respect to \(f\), where \(\odot\) is the element-wise vector product.
To do this, we define a notion of \emph{prediction equivalence}: for two \(x, x' \in \mcal{X}\), we write \(f(x) \cong f(x')\) to mean that \(f(x)\) and \(f(x')\) yield the same class.
This now allows us to formalize the intuition that an explanation \(\varphi(x)\) should suffice to recover the prediction of \(x\) under \(f\).

\begin{definition}
The explainable model \(\angles{f, \varphi}\) is \emph{consistent} at \(x\) if \(f(x) \cong f(x \odot \varphi(x))\).
\end{definition}

Evaluating \(f\) on \(x \odot \varphi(x)\) this way lets us apply the model as-is and therefore avoids the challenge of constructing a surrogate model that is accurate to the original~\cite{alizadeh2020managing}.
Moreover, this approach is reasonable, especially in domains like vision --- where one intuitively expects that a masked image retaining only the important features should induce the intended prediction.
Indeed, architectures like Vision Transformer~\cite{dosovitskiy2020image} can maintain high accuracy with only a fraction of the image present~\cite{salman2022certified}.



Particularly, we would like for \(\angles{f, \varphi}\) to generate explanations that are stable and concise (i.e. sparse).
The former is our central guarantee, and is ensured through smoothing.
The latter implies that \(\varphi(x)\) has few ones entries, and is a desirable property since a good explanation should not contain too much redundant information.
However, sparsity is a difficulty property to enforce,
as this is contingent on the model having high accuracy with respect to heavily masked inputs.
For sparsity we present a simple heuristic in Section~\ref{sec:adapting-methods} and evaluate its effectiveness in Section~\ref{sec:experiments}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Stability properties of explainable models}
\label{sec:stability-properties}

Given an explainable model \(\angles{f, \varphi}\) and some \(x \in \mcal{X}\), stability means that the prediction does not change even if one adds more explanatory features to \(\varphi(x)\).
For instance, the model-explanation pair in Figure~\ref{fig:non-stable} is \emph{not} stable, as the inclusion of a single feature group (patch) changes the prediction.
To formalize this notion of stability, we first introduce a partial ordering: for \(\alpha, \alpha' \in \{0,1\}^n\), we write \(\alpha \succeq \alpha'\) iff \(\alpha_i \geq \alpha_i '\) for all \(i = 1, \ldots, n\).
That is, \(\alpha \succeq \alpha'\) iff \(\alpha\) includes all the features selected by \(\alpha'\).

\begin{definition} \label{def:stable}
The explainable model \(\angles{f, \varphi}\) is stable at \(x\) if \(f(x \odot \alpha) \cong f(x \odot \varphi(x))\) for all \(\alpha \succeq \varphi(x)\).
\end{definition}

Note that the constant explanation \(\varphi(x) = \mbf{1}\), the vector of ones, makes \(\angles{f, \varphi}\) trivially stable at every \(x \in \mcal{X}\), though this is not a concise explanation.
Additionally, stability at \(x\) implies consistency at \(x\).

Unfortunately, stability is a difficult property to enforce in general, as it requires that \(f\) satisfy a monotone-like behavior with respect to feature inclusion --- which is especially challenging for complex models like neural networks.
Checking stability without additional assumptions on \(f\) is also hard: if \(k = \norm{\varphi(x)}_1\) is the number of ones in \(\varphi(x)\), then there are \(2^{n-k}\) possible \(\alpha \succeq \varphi(x)\) to check for consistency.
This large space of possible \(\alpha \succeq \varphi(x)\) motivates us to instead examine \emph{relaxations} of stability.
We introduce lower and upper-relaxations of stability below.

\begin{definition} \label{def:inc-stable}
The explainable model \(\angles{f, \varphi}\) is incrementally stable at \(x\) with radius \(r\) if \(f(x \odot \alpha) \cong f(x \odot \varphi(x))\) for all \(\alpha \succeq \varphi(x)\) where \(\norm{\alpha - \varphi(x)}_1 \leq r\).
\end{definition}

Incremental stability is a lower-relaxation, since we are considering the addition of only a few features.
We also define the upper-relaxation variant, where we consider the inclusion of most features.

% ~\cite{wu2020towards}


\begin{definition} \label{def:dec-stable}
The explainable model \(\angles{f, \varphi}\) is decrementally stable at \(x\) with radius \(r\) if \(f(x \odot \alpha) \cong f(x \odot \varphi(x))\) for all \(\alpha \succeq \varphi(x)\) where \(\norm{\mbf{1} - \alpha}_1 \leq r\).
\end{definition}

Decremental stability is a subtractive form of stability, in contrast to the additive nature of incremental stability.
Note that our definition means that decremental stability entails consistency, but this is not the case for incremental stability.
% Moreover, this notion is related to \emph{incremental deletion}~\cite{nauta2022anecdotal}.
Furthermore, observe that for a sufficiently large radius of \(r = \ceil{(n - \norm{\varphi(x)}_1) / 2}\), incremental and decremental stability together imply stability.


\begin{remark}
Similar notions to the above have been proposed in literature, and we refer to~\cite{nauta2022anecdotal} for an extensive survey.
In particular for~\cite{nauta2022anecdotal}, consistency is akin to \emph{preservation} and stability is similar to \emph{continuity}, except we are concerned with adding features.
In this regard, incremental stability is most similar to \emph{incremental addition} and decremental stability to \emph{incremental deletion}.
\end{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Lipschitz smoothness entails stability guarantees}
\label{sec:lipschitz-for-stability}
% We now consider how to guarantee the aforementioned properties using Lipschitz smoothness.

If \(f : \mcal{X} \to [0,1]^m\) is Lipschitz with respect to the masking of features, then we can guarantee relaxed stability properties for the explainable model \(\angles{f, \varphi}\).
Because Lipschitz smoothness is a property of functions, we introduce the mapping \(g(x, \alpha) = f(x \odot \alpha)\) to separate the input \(x \in \mcal{X}\) and binary mask \(\alpha \in \{0,1\}^n\).
This then reparametrizes our stability conditions as ensuring \(g(x, \alpha) \cong g(x, \varphi(x))\) when \(\alpha \succeq \varphi(x)\).
We will then study the Lipschitz smoothness of \(g(x, \alpha)\) with respect to the mask \(\alpha\), where we aim to adapt a standard argument outlined in the following remark.

% In particular, we study the Lipschitz smoothness of \(g(x, \alpha)\) with respect to its \(\alpha\) argument.
% Taking inspiration from adversarial robustness literature, we will leverage smoothness properties of \(g\) to achieve such stability.
% We aim to adapt a standard argument encapsulated in the following remark.

\begin{remark} \label{rem:g-lipschitz}
Let \(g_1, \ldots, g_m\) denote the coordinates of \(g : \mcal{X} \times \{0,1\}^n \to [0,1]^m\), and suppose for a given \(x \in \mcal{X}\) that each \(g_k\) satisfies:
\begin{align} \label{eq:lipschitz-in-alpha}
    \norm{g_k (x, \alpha) - g_k (x, \alpha')}_1
    \leq \lambda \norm{\alpha - \alpha'}_1,
    \quad \text{for all \(\alpha \in \{0,1\}^n\)},
\end{align}
for some given \(\lambda > 0\), then \(g(x, \alpha) \cong g(x, \alpha')\)
if \(\norm{\alpha - \alpha'}_1 \leq (g_A (x, \alpha) - g_B (x, \alpha)) / (2 \lambda)\).
Here \(g_A - g_B\) is referred to as the logit gap, where \(g_A, g_B\) denote the first and second largest logits:
\begin{align} \label{eq:logit-gap}
    k^\star = \underset{1 \leq k \leq m}{\mrm{argmax}}\, g_k (x, \alpha),
    \qquad g_A (x, \alpha) = g_{k^\star} (x, \alpha),
    \qquad g_B (x, \alpha) = \max_{i \neq k^\star} g_i (x, \alpha)
\end{align}
Equivalently, \eqref{eq:lipschitz-in-alpha} means that each \(g_k\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm with respect to \(\alpha\) for all \(x \in \mcal{X}\).
\end{remark}

Observe that Lipschitz smoothness is in fact a stronger assumption than necessary, as besides \(\alpha \succeq \varphi(x)\) it also imposes guarantees on \(\alpha \preceq \varphi(x)\).
Nevertheless, Lipschitz smoothness is one of the few classes of properties that can be guaranteed and analyzed at scale on arbitrary models~\cite{yang2020randomized,levine2021improved}.
Crucially, such Lipschitz smoothness can provably certify incremental and decremental stability.
We give a sketch of our main result (Theorem~\ref{thm:stability}) in the following.

\begin{remark}[Sketch of main result] \label{rem:main-result-sketch}
Consider an explainable model \(\angles{f, \varphi}\) where the mapping \(g(x, \alpha) = f(x \odot \alpha)\) satisfies the Lipschitz properties as in Remark~\ref{rem:g-lipschitz}.
Then at any \(x \in \mcal{X}\), the radius of incremental stability \(r_{\mrm{inc}}\) and radius of decremental stability \(r_{\mrm{dec}}\) are respectively:
\begin{align*}
    r_{\mrm{inc}} = \frac{g_A (x, \varphi(x)) - g_B (x, \varphi(x))}{2 \lambda},
    \qquad
    r_{\mrm{dec}} = \frac{g_A (x, \mbf{1}) - g_B (x, \mbf{1})}{2 \lambda}.
\end{align*}
\end{remark}


% \red{(TWO-SIDED REMARK)} Importantly, this Lipschitz condition readily translates into stability guarantees.
% Suppose \(\angles{f, \varphi}\) is consistent at \(x\) and each \(g_k\) satisfies the Lipschitz conditions~\eqref{eq:lipschitz-in-alpha}, then \(\angles{f, \varphi}\) is incrementally stable at \(x\) with radius \(d(x,\alpha)/(2\lambda)\), and decrementally stable at \(x\) with radius \(d(x, \mbf{1}) / (2 \lambda)\).
% As such, if one can enforce a \(\lambda\)-Lipschitz condition on each coordinate of \(g\), then one can provably demonstrate that \(\angles{f, \varphi}\) satisfies stability properties.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Adapting existing feature attribution methods}
\label{sec:adapting-methods}

Most existing feature attribution methods assign a real-valued score to feature importance, rather than a binary value.
We therefore need to convert this to a binary-valued method for use with a stable explainable model.
Let \(\psi : \mcal{X} \to \mbb{R}^n\) be such a continuous-valued method like LIME~\cite{ribeiro2016should} or SHAP~\cite{lundberg2017unified}, and fix some desired incremental stability radius \(r_{\mrm{inc}}\) and decremental stability radius \(r_{\mrm{dec}}\).
Given some \(x \in \mcal{X}\) a simple construction for binary \(\varphi(x) \in \{0,1\}^n\) is described next.

\begin{remark}[Iterative construction of \(\varphi(x)\)]
Consider any \(x \in \mcal{X}\) and let \(\rho\) be an index ordering on \(\psi(x)\) from high-to-low (i.e. largest logit first).
Initialize \(\alpha = \mbf{0}\), and for each \(i \in \rho\):
assign \(\alpha_i \leftarrow 1\) then check whether \(\angles{f, \varphi : x \mapsto \alpha}\) is now consistent, incrementally stable with radius \(r_{\mrm{inc}}\), and decrementally stable with radius \(r_{\mrm{dec}}\).
If so then terminate with \(\varphi(x) = \alpha\); otherwise continue.

\end{remark}

Note that the above method of constructing \(\varphi(x)\) does not impose guarantees of conciseness in the way that we may guarantee stability through Lipschitz smoothness.
Instead, the ordering proposed by an existing feature attribution method serves as a heuristic about the order in which we may greedily construct \(\varphi(x)\).
We show in Section~\ref{sec:experiments} that some feature attributions (e.g. SHAP~\cite{lundberg2017unified}) tend to yield sparser selections on average compared to others (e.g. vanilla gradient saliency~\cite{simonyan2013deep}).




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Ensuring Lipschitz smoothness with randomized smoothing}
% \label{sec:ensuring-lipschitz}

% We now give an overview of our core technical contribution in developing a smoothing method to ensure the Lipschitz properties of Section~\ref{sec:lipschitz-for-stability} --- thereby allowing for explainable models with provable stability guarantees.
% We observe that the desired smoothness is with respect to the masking of features.
% This means, however, that classical smoothing methods techniques~\cite{cohen2019certified,yang2020randomized} are not well-suited for our purpose, as they are primarily concerned with perturbing features rather than complete maskings.
% This therefore motivates us to develop a novel smoothing method suitable for maskings.
% We call our smoothing method Multiplicative Smoothing (\dname{}), where the goal is to begin with any \emph{base classifier} \(h : \mcal{X} \to [0,1]^m\) and then apply \dname{}-smoothing to derive a \emph{smoothed classifier} \(f : \mcal{X} \to [0,1]^m\) that satisfies the sufficient Lipschitz conditions.


% \input{figures/durt-overview}

% The main idea in \dname{} is to begin with an existing classifier \(h : \mcal{X} \to [0,1]^m\), and given \(x \in \mcal{X}\), we evaluate \(h\) on random maskings of \(x\).
% This is illustrated in Figure~\ref{fig:durt-overview}.
% More formally, given some \(x \in \mcal{X}\) we sample \(N\) random maskings \(\tilde{x}^{(1)}, \ldots, \tilde{x}^{(N)} \in \mcal{X}\), where each \(x^{(i)}\) is generated by dropping features from \(x\) uniformly at random with probability \(1 - \lambda\).
% We refer to this fixed \(\lambda \in [0,1]\) as the \emph{smoothing parameter}, and the evaluation of the \dname{}-smoothed classifier \(f\) is then taken to be:
% \begin{align}
% \label{eq:dname-sketch-f}
%     f(x) = \frac{1}{N} \sum_{i = 1}^{N} h (\tilde{x}^{(i)}),
%     \qquad
%     \tilde{x}^{(i)}_j
%         = \begin{dcases}
%             x_j &\text{with probability \(\lambda\)} \\
%             0 &\text{with probability \(1 - \lambda\)}
%         \end{dcases},
%     \qquad j = 1, \ldots, n
% \end{align}
% We show that in expectation, for all \(x \in \mcal{X}\) each coordinate of the mapping \(g(x, \alpha) = f(x \odot \alpha)\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm with respect to the \(\alpha\) parameter (Theorem~\ref{thm:simple-smoothing}), i.e., each \(g_1, \ldots, g_m\) is Lipschitz in \(\alpha\).
% Moreover, this process can be made deterministic, i.e. derandomized, with appropriate choice of noise (Theorem~\ref{thm:derand-smoothing}).
% Thus, we can guarantee for all \(x\) that \(g(x, \alpha) \cong g(x, \alpha')\) provided \(\norm{\alpha - \alpha'}_1 \leq d(x, \alpha) / (2 \lambda)\).
% Additionally, note that \(\lambda = 1\) recovers the original classifier, as feature dropping will happen with probability zero.
% We will flexibly refer to \(\lambda\) as the smoothing parameter, the Lipschitz constant, or the feature keep-probability depending on the appropriate context.




==> old/provable_guarantees_1.tex <==
\section{Constructing Explainable Models with Provable Guarnatees}
\label{sec:provable-guarantees}

We now discuss how to construct an explainable model from any classifier \(f\) and explanation method \(\varphi_0\).
Specifically, we will apply \dname{} on \(f\) to yield \(h\), and then adapt \(\varphi_0\) into \(\varphi\), such that the explainable model \(\angles{h, \varphi}\) satisfies consistency, incremental stability, and decremental stability.
We first begin with an overview of how to prove incremental and decremental stability using the robustness of \(h\).
We then show how to adapt \(\varphi_0\) into \(\varphi\).



% We now present how to verify sufficiency and necessity with respect to a \dname{}-smoothed classifier.
% Additionally, we present a simple algorithm for yielding robust feature attributions by construction.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Analysis of Incremental and Decremental}
\label{sec:robustness-analysis}
We take the \dname{}-smoothed classifier as in Theorem~\ref{thm:masking}:
\begin{align*}
    g(x, \alpha; \lambda, \mu) = \expval{s \sim \mcal{D}}\, h(x \odot \tilde{\alpha}),
    \qquad
    \tilde{\alpha} = (\mbf{1} - \mu) + \mu \mbb{I}[\lambda \alpha \geq s],
\end{align*}
except we have now made the \(\lambda, \mu\) parameters now explicitly, and recall that we can recover convert between \(f\) and \(g\) via \(f(x; \lambda, \mu) = g(x, \mbf{1}; \lambda, \mu)\).
Our task is to find the radius to which \(\angles{f, \varphi}\) is incrementally stable and decrementally stable.
Let us suppose that \(\angles{f, \varphi}\) is consistent, and consider some \(x \in \mcal{X}\) for which \(\alpha = \varphi(x)\) such that \(f(x) \cong f(x \odot \alpha)\).


\paragraph{Incremental Stability}
We apply the noise mask \(\mu = \mbf{1}\) and evaluate:
\begin{align}
    r_{\mrm{inc}} =
    \frac{g_A (x, \alpha; \lambda, \mbf{1}) -
          g_B (x, \alpha; \lambda, \mbf{1})}{2\lambda}
    = \frac{f_A (x \odot \alpha; \lambda, \mbf{1}) - f_B (x \odot \alpha; \lambda, \mbf{1})}{2 \lambda}
\end{align}

\paragraph{Decremental Stability}
We apply the noise mask \(\mu = \mbf{1} - \alpha\) and evaluate:
\begin{align}
    r_{\mrm{dec}} =
    \frac{g_A (x, \mbf{1}; \lambda, \mbf{1} - \alpha) -
          g_B (x, \mbf{1}; \lambda, \mbf{1} - \alpha)}{2\lambda}
    = \frac{f_A (x; \lambda, \mbf{1} - \alpha) - f_B (x; \lambda, \mbf{1} - \alpha)}{2 \lambda}
\end{align}
Consequently, we have that \(\angles{f, \varphi}\) is incrementally stable with radius \(r_{\mrm{inc}}\) and decrementally stable with radius \(r_{\mrm{dec}}\) at \(x\).
Note that we require a small Lipschitz constant (\(\lambda \leq 1/2\)) in order to get non-trivial radii (\(r_{\mrm{inc}}, r_{\mrm{dec}} \geq 1\)).
Since the logit gap is \(\leq 1\), this demonstrates a fundamental trade-off in how much radii one can achieve at the expense of more noise.
However, there are techniques for boosting the coverage of an input \(x\), in particular using feature grouping as discussed in Section~\ref{sec:basic-extensions} --- and demonstrate an example of which in Figure~\ref{fig:non-robust}.


\subsection{Constructing Robust Feature Attributions}
\label{sec:constructing-stable}

We now show how to derive from any feature attribution method \(\varphi_0 : \mcal{X} \to \mbb{R}^n\) a binary feature attribution method \(\varphi\) with the desired formal properties.
Note that the domain of \(\varphi_0\) is \(\mbb{R}^n\) for full generality, where higher values will denote greater feature importance.

We begin with some desired incremental stability radius \(r_{\mrm{inc}}\) and decremental stability radius \(r_{\mrm{dec}}\), and an ordering on \([n]\) as given by \(\varphi_0 (x)\).
We then construct the valuation \(\varphi(x)\) in a simple iterative algorithm as follows:
we begin with \(\alpha = \mbf{0}\), and iteratively assign new entries \(\alpha_i \leftarrow 1\) where the index \(i\) is derived from the ordering of \(\varphi_0 (x)\).
When \(\angles{f, \varphi : x \mapsto \alpha}\) is consistent, \(r_{\mrm{inc}}\)-incrementally stable, and \(r_{\mrm{dec}}\)-decrementally stable at \(x\), we terminate with the output \(\varphi(x) = \alpha\).
We remark that one can use binary search to speed up this search process.
We have found it helpful to use \(\varphi_0\) based on an existing continuous-valued feature attribution method (e.g. LIME~\cite{ribeiro2016should}, SHAP~\cite{lundberg2017unified}).




==> old/smoothing_1.tex <==
\section{Randomized Smoothing}
\label{sec:smoothing}

Randomized smoothing is a collection of techniques for robustness guarantees against adversarial attacks, and are the only known methods known to scale to very large models.
In this section we present \dname{}, a derandomized smoothing method that gives strong robustness guarantees with minimal accuracy loss, all while maintaining a low sample complexity.
We first give an overview of randomized smoothing in Section~\ref{sec:smoothing-primer}.
We then show in Section~\ref{sec:attribution-input-consistency} that the commonly used additive smoothing methods are not suitable in our setting due to violating attribution-input consistency.
In Section~\ref{sec:ourname-smoothing} we formally define and construct \dname{}.
Finally in Section~\ref{sec:basic-extensions} we present some basic extensions of noise masking and feature grouping that improve the versatility of \dname{}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{A Primer on Randomized Smoothing}
\label{sec:smoothing-primer}

An important early work in randomized smoothing for classification models is~\cite{cohen2019certified}, which proposed additive Gaussian smoothing to achieve robustness.
Later works soon showed that additive Gaussian smoothing in fact leads to tight Lipschitz constants in the \(\ell^2\) norm~\cite{levine2019certifiably,salman2019provably}.
Additive smoothing for general \(\ell^p\) norms is studied in~\cite{yang2020randomized}, which introduces a relevant result for \(\ell^1\) norm smoothing that we state below:
given any classifier \(f\), and consider the smooth classifier \(h\) defined by
\begin{align} \label{eq:additive-l1}
    h(x) = \expval{\varepsilon \sim \mcal{U}^n(-1/(2\lambda), 1/(2\lambda))} f(x + \varepsilon),
\end{align}
then its components \(h_1, \ldots, h_K\) are \(\lambda\)-Lipschitz in the \(\ell^1\) norm, where \(\mcal{U}^{n}\) is the \(n\)-dimensional uniform distribution and \(\lambda > 0\) is a tunable noise parameter.
Intuitively, a smaller \(\lambda\) implies more noise in the smoothing procedure, and so achieves smaller Lipschitz constants at the expense of accuracy.
Smaller Lipschitz constants are desirable in robustness analysis: let \(h_A (x) \geq h_B(x) \geq \cdots\) be an ordering of the logits of \(h(x)\), where let \(d = h_A (x) - h_B (x)\) be the gap between the two largest logits.
Then for any \(x'\) such that \(\norm{x' - x}_1 \leq d / (2\lambda)\) we have the same class for \(h(x)\) and \(h(x')\).
In other words, \(h(x)\) is locally robust around a \(\ell^1\) radius of \(d / (2\lambda)\), and we remark that this also generalizes to other \(\ell^p\) norms.
As a practical concern, the \(\lambda\) cannot be too small, because doing so is equivalent to injecting a lot of noise and thereby hurting the smoothed model accuracy.

\paragraph{Robustness to Feature Inclusion and Exclusion}
In the above we have described the general approach of additive smoothing methods, and we now turn our attention to robustness with respect to the feature attribution.
In order to derive a smoothed classifier \(h\) that is robust to the inclusion and exclusion of features, we construct a mapping \(g(x, \alpha) = h(x \odot \alpha)\) that is robust in \(\alpha\).
As alluded to in Section~\ref{sec:dname-overview}, we will use random noise for dropping features, rather than for additive perturbations.
We therefore define the mapping \(g : \mcal{X} \times \{0,1\}^n \to [0,1]^K\) as:
\begin{align}
\label{eq:dname-sketch-g}
    g(x, \alpha) = \expval{\tilde{\alpha} \sim \mcal{D}(\alpha, \lambda)} f(x \odot \tilde{\alpha}),
    \qquad
    \tilde{\alpha}_j
    = \begin{dcases}
        1, &\enskip \text{with probability \(\lambda\)} \\
        0, &\enskip \text{with probability \(1 - \lambda\)}
    \end{dcases},
    \qquad j = 1, \ldots, n
\end{align}
where \(\mcal{D}\) is a distribution on \(\{0,1\}^n\) parametrized by \(\alpha \in \{0,1\}^n\) and \(\lambda \in [0,1]\).
Observe that one can recover the smoothed classifier as \(h(x) = g(x, \mbf{1})\), is similar to the presentation in~\eqref{eq:dname-sketch}.
We will formalize this presentation of \(g\) in Theorem~\ref{thm:basic-smoothing}, where we show that for all \(x \in \mcal{X}\), the mapping \(g(x, \alpha)\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm with respect to \(\alpha\) --- thereby establishing a robustness guarantee that allows us to provably guarantee incremental and decremental stability of an explainable model \(\angles{h, \varphi}\).
% Moreover, we will also show that this construction preserves the identity \(g(x, \alpha) = g(x \odot \alpha, \mbf{1})\), which we call \emph{attribution-input consistency}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Additive Smoothing Violates Attribution-Input Consistency}
\label{sec:attribution-input-consistency}

We now show that naive application of additive smoothing methods like~\eqref{eq:additive-l1} violates attribution-input consistency.
A required condition for our robustness properties to hold is that perturbations on \(\alpha\) must imply perturbations on \(x\).
This we express as the identity \(g(x, \alpha) = g(x \odot \alpha, \mbf{1})\), which must hold for all classifiers \(f\), inputs \(x \in \mcal{X}\) and attributions \(\alpha \in \{0,1\}^n\).
That is, any changes in \(\alpha\) on the LHS are directly evaluated in the RHS evaluation on \(x \odot \alpha\).
Importantly, this condition is not always satisfied by additive smoothing methods.


\begin{theorem}
There exists \(f : \mcal{X} \to [0,1]\) and distribution \(\mcal{D}\) such that \(g\) defined as
\begin{align*}
    g(x, \alpha) = \expval{\varepsilon \sim \mcal{D}} f(x \odot (\alpha + \varepsilon)),
\end{align*}
satisfies the inequation \(g(x, \alpha) \neq g(x \odot \alpha, \mbf{1})\) for some \(x \in \mcal{X}\) and \(\alpha \in \{0,1\}^n\).
\end{theorem}
\begin{proof}
Consider some \(f\) such that \(f(\mbf{0}) = 0\), and \(f(x) = 1\) for all other \(x \in \mcal{X}\).
Suppose that \(\mcal{D}\) is a non-constant distribution on \(\mbb{R}^n\), and consider \(\alpha = \mbf{0}\).
Then we have the strict inequality
\begin{align*}
    g(x, \alpha) = \expval{\varepsilon \sim \mcal{D}} f(x \odot (\alpha + \varepsilon))
    > \expval{\varepsilon \sim \mcal{D}} f((x \odot \alpha) \odot (\mbf{1} + \varepsilon))
    = g(x \odot \alpha, \mbf{1})
    = 0
\end{align*}
\end{proof}

Intuitively, this violation occurs because the additive noising process may turn non-explanatory bits of \(\alpha\) into values \(> 0\).
This causes the \(f\) within the \(g(x, \alpha)\) term to observe more features of \(x\) than it would have been able to, had the input been pre-ablated as with the RHS \(g(x \odot \alpha, \mbf{1})\).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multiplicative Smoothing}
\label{sec:ourname-smoothing}

We first formalize the intuition of~\eqref{eq:dname-sketch-g} in a smoothing method that we call \sname{} (Theorem~\ref{thm:basic-smoothing}), and we leverage the analysis techniques developed in~\cite{levine2021improved} to establish its smoothness properties.
Crucially, \sname{} preserves attribution-input consistency (Proposition~\ref{prop:sname-consistency}).
We then present a \emph{derandomized} variant of this smoothing, which we call \dname{} (Theorem~\ref{thm:derand-smoothing}), and also show that it also preserves this consistency (Proposition~\ref{prop:dname-consistency}).
We examine in detail how to couple the components of the random noise vector, such that the expected value can be computed at a low sample complexity.

\begin{theorem}[\sname{}] \label{thm:basic-smoothing}
    Let \(f : \mcal{X} \to [0,1]\) be measurable and define \(g : \mcal{X} \times \mbb{R}^{n} \to [0,1]\) as
    \begin{align} \label{eq:thm:basic-smoothing}
        g(x, \alpha) = \expval{s \sim \mcal{U}^{n} (0,1)} f(x \odot \tilde{\alpha}),
        \qquad \tilde{\alpha} = \mbb{I}[\lambda \alpha \geq s],
        \qquad \lambda \in [0,1] \enskip \text{fixed}.
    \end{align}
    Then \(g(x, \cdot) : \mbb{R}^{n} \to [0,1]\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm for all \(x \in \mcal{X}\).
\end{theorem}

Our first result shows that using the same uniform distribution as additive smoothing can also yield similar \(\ell^1\) norm Lipschitz bounds in the multiplicative case.
We have first presented this result for \(\mbb{R}^n\) rather than \(\{0,1\}^n\) for generality, but this does not hinder theoretical applications.
This type of smoothing can be viewed as probabilistically dropping features: when \(\alpha \in \{0,1\}^n\), we have \(\mrm{Pr}[\tilde{\alpha}_i = 1] = \lambda \alpha_i\).
Importantly, an advantage is that \sname{} preserves attribution-input consistency.

\begin{proposition}\label{prop:sname-consistency}
    Take \(g\) as in Theorem~\ref{thm:basic-smoothing}, then \(g(x, \alpha) = g(x \odot \alpha, \mbf{1})\) for all \(x \in \mcal{X}\) and \(\alpha \in \{0,1\}^n\).
\end{proposition}
\begin{proof}
Fix some \(x \in \mcal{X}\) and \(\alpha \in \{0,1\}^n\), then
\begin{align*}
    g(x, \alpha)
    = \expval{}\, f(x \odot \mbb{I}[\lambda \alpha \geq s])
    = \expval{}\, f(x \odot \alpha \odot \mbb{I}[\lambda \mbf{1} \geq s])
    = g(x \odot \alpha, \mbf{1}),
\end{align*}
\end{proof}


Our next aim is to make this process derandomized, which is useful in that it allows for the exact computation of the expected value --- and thus the Lipschitz constant --- rather than relying on high probability bounds and high sample complexity.
We acquire inspiration from~\cite{levine2021improved}, and the main idea is to draw random noise from discretizations of the unit interval.
Specifically, we fix an integer \(q > 1\) to denote the granularity of this discretization.
We then require \(\lambda \in \{1/q, 2/q, \ldots, 1\}\), and that \(s\) follows a similar (but shifted) discretization.
This is formalized in the following result.


\begin{theorem}[\dname{}] \label{thm:derand-smoothing}
    Fix an integer \(q > 0\) and let \(s \sim \mcal{D}\) be a \(n\)-dimensional random vector with each coordinate uniformly distributed as
    \begin{align} \label{eq:thm:derand-smoothing-1}
        s_i \sim \mcal{U}(\{1/q, 2/q, \ldots, 1\}) - 1/(2q),
        \quad i = 1, \ldots, n,
    \end{align}
    where \(\mcal{D}\) is any finite discrete distribution on \([0,1]^n\) such that \(s_i\) need not be independent.
    Let \(f : \mcal{X} \to [0,1]\) be measurable and define \(g : \mcal{X} \times \{0,1\} ^{n} \to [0,1]\) as
    \begin{align} \label{eq:thm:derand-smoothing-2}
        g(x, \alpha) = \expval{s \sim \mcal{D}} f(x \odot \tilde{\alpha}),
        \qquad \tilde{\alpha} = \mbb{I}[\lambda \alpha \geq s],
        \qquad \lambda \in \{1/q, 2/q, \ldots, 1\} \enskip \text{fixed}.
    \end{align}
    Then \(g(x, \cdot) : \{0,1\}^n \to [0,1]\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm for all \(x \in \mcal{X}\).
\end{theorem}

This form of smoothing also preserves attribution-input consistency.

\begin{proposition}\label{prop:dname-consistency}
    Take \(g, \mcal{D}\) as in Theorem~\ref{thm:derand-smoothing}, then \(g(x, \alpha) = g(x \odot \alpha, \mbf{1})\) for all \(x \in \mcal{X}\) and \(\alpha \in \{0,1\}^n\).
\end{proposition}
\begin{proof}
Identical to that of Proposition~\ref{prop:sname-consistency}.
\end{proof}


We say that \dname{} is a \emph{derandomized} smoothing method because we can construct \(\mcal{D}\) such that the expected value in~\eqref{eq:thm:derand-smoothing-2} can be exactly evaluated with a small number of samples (\(q\) samples, in fact).
This is in contrast to \sname{}, where the nature of the continuous uniform noise means that we can only approximate the expected value through randomized sampling.

\paragraph{Sampling from \(\mcal{D}\)}
Let us now consider the distribution \(\mcal{D}\) of Theorem~\ref{thm:derand-smoothing}.
For some \(s \sim \mcal{D}\), each component \(s_i\) need not be independent; we require only that its marginal distribution is uniform over \(q\) distinct values.
This is an important simplifying assumption: had we drawn \(s\) from a coordinate-wise independent distribution like \(\mcal{U}^{n}(S)\) with \(S \subseteq [0,1]\) a finite set, then we would need \(\abs{S}^n\) samples to exactly compute the expected value.
Below we demonstrate a construction of \(\mcal{D}\) that satisfies the conditions of the theorem, and allows for exact computation of the expected value in \(q\) samples.


% \paragraph{Sampling from \(\mcal{D}\)}

The primary insight in the construction of \(\mcal{D}\) is to reduce the \(n\)-dimensional source of randomness to a one-dimensional noise.
We first fix some \(v \in \{0, 1/q, \ldots, (q-1)/q\}^n\) when the model is initialized, and at test time we take a single random scalar uniformly at random
\begin{align*}
    s_{\mrm{base}} \sim \mcal{U}(\{1/q, 2/q, \ldots, 1\}) - 1/(2q),
\end{align*}
and define each component of \(s\) to be
\begin{align*}
    s_i = (v_i + s_{\mrm{base}}) \enskip\mrm{mod}\enskip 1,
    \quad \text{for all \(i = 1, \ldots, n\).}
\end{align*}
In effect, \(v\) acts as the initial \(n\)-dimensional seed, while \(s_{\mrm{base}}\) is the one-dimensional noise.
Notably, there are only \(q\) possible values of \(s_{\mrm{base}}\), and so there are only \(q\) different possible values for \(s\) (once \(v\) is fixed).
This allows us to exactly compute the expected value in \eqref{eq:thm:derand-smoothing-2} using only \(q\) samples of \(f\).
% Experimentally for image classification over ImageNet1K, we have found \(q \leq 64\) to be sufficient, with even \(q = 16\) achieving good results.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsubsection{Basic Extensions}

\subsection{Basic Extensions}
\label{sec:basic-extensions}

We now present two basic extensions to \dname{} in noise masking and feature grouping.
Noise masking allows us to selectively choose where to apply noise, while feature grouping reduces the effective feature dimension of an input.
Combined, these extensions allow us to achieve stronger robustness guarantees over the explanations.

\paragraph{Noise Masking}
It may be desirable to selectively apply noise to some features and not others.
We introduce Theorem~\ref{thm:masking} below as a more fine-grained approach for boosting the possibly conservative Lipschitz constants that we may otherwise get from the Theorem~\ref{thm:derand-smoothing}.
Our idea is to use a binary vector \(\mu \in \{0, 1\}^n\) called the \emph{noise mask}, where \(\mu_i = 1\) denotes that feature \(x_i\) should be noised, while if \(\mu_i = 0\), then feature \(x_i\) should not be noised, and is retained.

\begin{theorem} \label{thm:masking}
    Take \(\mcal{D}, f, \lambda\) be as in Theorem~\ref{thm:derand-smoothing} and define \(g : \mcal{X} \times \{0,1\}^n \to [0,1]\) as
    \begin{align} \label{eq:thm:masking-1}
        g(x, \alpha)
            = \expval{s \sim \mcal{U}^n (0,1)} f(x \odot \tilde{\alpha}),
        \qquad
        \tilde{\alpha}
            = (\mbf{1} - \mu) + \mu \odot \mbb{I}[\lambda \alpha \geq s],
        \qquad \mu \in \{0,1\}^n \enskip \text{fixed}.
    \end{align}
    Then \(g(x, \cdot) : \{0,1\}^n \to [0,1]\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm for all \(x \in \mcal{X}\).
\end{theorem}

When \(\mu = \mbf{1}\), this reduces to the case of Theorem~\ref{thm:derand-smoothing}.
Importantly, under mild assumptions on \(\mu\), the noise masking process also preserves attribution-input consistency.

\begin{proposition}
\label{prop:mask-consistency}
    Take \(\mcal{D}, g, \mu\) as in Theorem~\ref{thm:masking}, then
    \(g(x, \alpha) = g(x \odot \alpha, \mbf{1})\)
    for all \(x \in \mcal{X}\) and \(\alpha \preceq \mu\).
\end{proposition}

% When \(\mu = \mbf{1}\), we always have \(\alpha \preceq \mu\).



\paragraph{Grouping Features}
We have so far assumed that \(\mcal{X} = \mbb{R}^{n}\), but sometimes it may be desirable to group features together, e.g. color channels of the same pixel.
Our results also hold for more general \(\mcal{X} = \mbb{R}^{d_1} \times \cdots \times \mbb{R}^{d_n}\), where for such \(x \in \mcal{X}\) and \(\alpha \in \mbb{R}^{n}\) we lift \(\odot\) as
\begin{align*}
    (x \odot \alpha)_i = x_i \cdot \mbb{I}[\alpha_i = 1] \in \mbb{R}^{d_i}.
\end{align*}
All of our proofs are identical under this construction, with the exception of the dimensionalities of terms like \((x \odot \alpha)\).
An example of feature grouping is given in Figure~\ref{fig:non-robust}.







==> old/smoothing_2.tex <==
\section{Multiplicative smoothing for Lipschitz constants}
\label{sec:smoothing}
In this section we present our main technical contribution in Multiplicative Smoothing (\dname{}).
The goal is to transform an arbitrary base classifier \(h : \mcal{X} \to [0,1]^m\) into a smoothed classifier \(f : \mcal{X} \to [0,1]^m\) that satisfies the appropriate Lipschitz conditions~\eqref{eq:lipschitz-in-alpha}.
This then allows one to appropriately couple an explanation method \(\varphi\) with \(f\) in order to form an explainable model \(\angles{f, \varphi}\) with provable stability guarantees.

We first give an extended overview in Section~\ref{sec:extended-overview}, and illustrate that a principal motivation for developing \dname{} is because classical smoothing techniques may fail to satisfy a property that we call \emph{masking equivalence}.
We then formally introduce \dname{} in two parts: first a simple approach in Section~\ref{sec:dname-rand} and then a derandomized approach in Section~\ref{sec:dname-derand}.
Both forms of smoothing achieve the desired Lipschitz smoothness, but the key distinction is in the choice of noise distribution.
In particular, we show that each coordinate of the noise vector need not be statistically independent, and this allows us to exactly evaluate the smoothed model with \(N \ll 2^n\) samples.
We finally combine all the details in Section~\ref{sec:certifying-stability} and present how to provably certify the stability of an \dname{}-smoothed explainable model \(\angles{f, \varphi}\).



\subsection{Extended overview}
\label{sec:extended-overview}

We expand on the overview given in Section~\ref{sec:ensuring-lipschitz}, and describe the procedure in detail.
Again, it will be useful to study \(g : \mcal{X} \times \{0,1\}^n \to [0,1]^m\), the two-parameter form of \(f\).
Unlike earlier, however, we first introduce \(g\) and then use it to define \(f\), since doing so allows us to more conveniently study Lipschitz smoothness to maskings.
We therefore present the smoothing process as follows:
\begin{align} \label{eq:dname-sketch-g}
    g(x, \alpha)
        = \expval{s \sim \mcal{D}}
            h(x \odot \tilde{\alpha}),
    \qquad \tilde{\alpha}_i = \alpha_i \odot s_i,
    \qquad s_i \sim \mrm{Bernoulli}(\lambda),
    \qquad i = 1, \ldots, n
\end{align}
where \(\mcal{D}\) is a distribution on \(\{0,1\}^n\) where each coordinate is Bernoulli with parameter \(\lambda \in [0,1]\).
The same intuition in Figure~\ref{fig:durt-overview} carries over and note the similarity to~\eqref{eq:dname-sketch-f}, where now each \(\tilde{\alpha} \sim \mcal{A}\) is a random masking of \(\alpha\) with features dropped uniformly with probability \(1 - \lambda\).
We then define the smoothed classifier via the mapping \(f(x) = g(x, \mbf{1})\).

Observe that for \(g\) the noise is with respect to \(\alpha\) rather than \(x\).
In order to preserve equivalence between \(f\) and \(g\), it is therefore necessary that we satisfy the identity \(f(x \odot \alpha) = g(x \odot \alpha, \mbf{1}) = g(x, \alpha)\) for all \(x \in \mcal{X}\) and \(\alpha \in \{0,1\}^n\).
This is especially relevant for translating between Lipschitz smoothness of \(g\) into stability guarantees with \(f\).

\begin{definition}
    The function \(g : \mcal{X} \times \{0,1\}^n \to [0,1]^m\) satisfies masking equivalence if \(g(x, \alpha) = g(x \odot \alpha, \mbf{1})\) for all \(x \in \mcal{X}\) and \(\alpha \in \{0,1\}^n\).
\end{definition}

Then for \(g\) that take the above form~\eqref{eq:dname-sketch-g}, masking equivalence is easy to show.

\begin{lemma}\label{lem:masking-equivalence}
    Fix \(\lambda \in [0,1]\) and let \(\mcal{A}\) be any distribution on \(\{0,1\}^n\) with the properties listed in \eqref{eq:dname-sketch-g}, then \(g : \mcal{X} \times \{0,1\}^n \to [0,1]^m\) satisfies masking equivalence.
\end{lemma}
\begin{proof}
Note that any \(\alpha \in \{0,1\}^n\) satisfies the identity \(\alpha = \mbf{1} \odot \alpha\).
We may therefore write:
\begin{align*}
    g(x, \alpha)
        = \expval{s \sim \mcal{D}} h(x \odot (\alpha \odot s))
        = \expval{s \sim \mcal{D}} h(x \odot \alpha \odot (\mbf{1} \odot s))
        = g(x \odot \alpha, \mbf{1})
\end{align*}
\end{proof}



% Importantly, our principal motivation for developing \dname{} is because classical smoothing techniques~\cite{cohen2019certified,yang2020randomized} might fail to satisfy masking equivalence.
% This then adds a layer of inconvenience when translating between \(g\) and \(f\), and we elaborate on this phenomenon in Section~\ref{sec:masking-equivalence}.
% We then formally introduce \dname{} in two parts: first a simple approach in Section~\ref{sec:dname-rand} and then a derandomized approach in Section~\ref{sec:dname-derand}.
% The key distinction is in the choice of \(\mcal{D}\), where importantly each coordinate of \(\tilde{\alpha}\) need not be statistically independent to achieve the desired Lipschitz constant.
% The practicality of this is that the derandomization introduced in Section~\ref{sec:dname-derand} allows us to exactly evaluate the expected value~\eqref{eq:dname-sketch-g} using \(N \ll 2^n\) samples, thereby avoiding the exponential sample complexity of a simple implementation.
% We finally combine all the details in Section~\ref{sec:certifying-stability} and present how to provably certify the stability of an \dname{}-smoothed explainable model \(\angles{f, \varphi}\).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Classical smoothing violates masking equivalence}
% \label{sec:masking-equivalence}

Crucially, many classical smoothing techniques fail to satisfy masking equivalence.
We will focus on \emph{additive smoothing}~\cite{cohen2019certified,yang2020randomized}, which is by far the most common style of randomized smoothing.
The key distinction between additive smoothing and our proposed approach in~\eqref{eq:dname-sketch-g} is in how noise is applied,
where let \(\mcal{D}_{\mrm{mult}}\) and \(\mcal{D}_{\mrm{add}}\) be any two distributions on (subsets of) \(\mbb{R}^n\):
\begin{align*}
    g(x, \alpha)
    = \begin{dcases}
        \expval{s \sim \mathcal{D}_{\mrm{mult}}} h(x \odot (\alpha \odot s))
            &\text{multiplicative noise injection} \\
        \expval{s \sim \mcal{D}_{\mrm{add}}} h(x \odot (\alpha + s))
            &\text{additive noise injection}
    \end{dcases}
\end{align*}
We next show that additive smoothing has counterexamples to masking equivalence.

% As alluded to earlier, additive smoothing may violate masking equivalence.

\begin{proposition} \label{prop:additive-smoothing-fails}
There exists \(h : \mcal{X} \to [0,1]\) and distribution \(\mcal{D}\) such that \(g\) defined as
\begin{align*}
    g(x, \alpha) = \expval{s \sim \mcal{D}} h(x \odot (\alpha + s)),
\end{align*}
satisfies the inequation \(g(x, \alpha) \neq g(x \odot \alpha, \mbf{1})\) for some \(x \in \mcal{X}\) and \(\alpha \in \{0,1\}^n\).
\end{proposition}
\begin{proof}
Consider some \(h\) such that \(h(\mbf{0}) = 0\), and \(h(x) = 1\) for all other \(x \in \mcal{X}\).
Suppose that \(\mcal{D}\) is a non-constant distribution on \(\mbb{R}^n\), and consider \(\alpha = \mbf{0}\).
Then we have the strict inequality
\begin{align*}
    g(x, \alpha) = \expval{s \sim \mcal{D}} h(x \odot (\alpha + s))
    > \expval{s \sim \mcal{D}} h((x \odot \alpha) \odot (\mbf{1} + s))
    = g(x \odot \alpha, \mbf{1})
    = 0
\end{align*}
\end{proof}

Intuitively, this occurs because additive smoothing primarily applies noise by perturbing feature values, rather than completely masking them.
As such, there might be ``information leakage'' when non-explanatory bits of \(\alpha\) are changed into non-zero values.
This then causes each sample of \(h(x \odot \tilde{\alpha})\) within \(g(x, \alpha)\) to observe more features of \(x\) than it would have been able to otherwise.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multiplicative smoothing with simple noise}
\label{sec:dname-rand}

It suffices to use \(\mcal{U}^n (0,1)\), the uniform distribution on \([0,1]^n\), to achieve the sufficient Lipschitz constants for stability.
This we illustrate in the following result.

\begin{theorem}[Simple \dname{}] \label{thm:simple-smoothing}
    Consider any \(h : \mcal{X} \to [0,1]\) and define \(g : \mcal{X} \times \{0,1\}^n \to [0,1]\) as
    \begin{align} \label{eq:thm:simple-smoothing}
        g(x, \alpha) = \expval{s \sim \mcal{U}^{n} (0,1)} h(x \odot \tilde{\alpha}),
        \qquad \tilde{\alpha} = \mbb{I}[\lambda \alpha \geq s],
        \qquad \lambda \in [0,1] \enskip \text{fixed}.
    \end{align}
    Then \(g(x, \cdot) : \{0,1\}^{n} \to [0,1]\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm for all \(x \in \mcal{X}\).
\end{theorem}

We emphasize that the formulation of Theorem~\ref{thm:simple-smoothing} is just that of~\eqref{eq:dname-sketch-g} using the uniform distribution, and this choice will satisfy zeroing coordinates of \(\alpha\) with probability \(1 - \lambda\).
A limitation of using a uniform distribution, however, is that one needs an exponential number of samples to exactly compute the expected value.
This is a barrier to tractable implementation, and approximating the expected value with fewer samples would require probabilistic bounds on the Lipschitz constant.
We remark that this need for approximation arises in many randomized smoothing methods~\cite{cohen2019certified}, and high sample complexity is a known issue for randomized smoothing~\cite{kumar2020curse}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multiplicative smoothing with derandomization}
\label{sec:dname-derand}

Importantly, each noise coordinate from \(\mcal{D}\) need only be uniform and \emph{not} statistically independent to attain the desired Lipschitz conditions (Theorem~\ref{thm:derand-smoothing}).
We construct \(\mcal{D}\) with structured dependence and exploit it to significantly reduce the sample complexity of evaluating the smoothed model.
We call this process process \emph{derandomization}, and achieve it using two key ideas from~\cite{levine2021improved}: first, by fixing an integer \(q > 0\) to discretize the values of \(\lambda \in \{1/q, \ldots, q/q\}\); second, by a construction of \(\mcal{D}\) (Remark~\ref{rem:constructing-D}).
One then needs only \(q\) samples to \emph{exactly} evaluate the smoothed model --- an exponential reduction from the simple noise case in Theorem~\ref{thm:simple-smoothing}.
% In the following we first present the smoothness results of using such a discretized and non-independent \(\mcal{D}\) in Theorem~\ref{thm:derand-smoothing}.
% We then present an explicit construction of \(\mcal{D}\).

\begin{theorem}[Derandomized \dname{}] \label{thm:derand-smoothing}
    Fix an integer \(q > 0\) and let \(s \sim \mcal{D}\) be a \(n\)-dimensional random vector with each coordinate uniformly distributed as
    \begin{align} \label{eq:thm:derand-smoothing-1}
        s_i \sim \mcal{U}(\{1/q, \ldots, q/q\}) - 1/(2q),
        \quad i = 1, \ldots, n,
    \end{align}
    where \(\mcal{D}\) is any finite discrete distribution on \([0,1]^n\) such that \(s_i\) need not be independent.
    Consider any \(h : \mcal{X} \to [0,1]\) and define \(g : \mcal{X} \times \{0,1\} ^{n} \to [0,1]\) as
    \begin{align} \label{eq:thm:derand-smoothing-2}
        g(x, \alpha) = \expval{s \sim \mcal{D}} h(x \odot \tilde{\alpha}),
        \qquad \tilde{\alpha} = \mbb{I}[\lambda \alpha \geq s],
        \qquad \lambda \in \{1/q, \ldots, q/q\} \enskip \text{fixed}.
    \end{align}
    Then \(g(x, \cdot) : \{0,1\}^n \to [0,1]\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm for all \(x \in \mcal{X}\).
\end{theorem}

We emphasize that the main difference between the earlier simple variant in Theorem~\ref{thm:simple-smoothing} and the result here are: the discretization of the smoothing parameter \(\lambda\) and noise \(s \sim \mcal{D}\), and the lack of coordinate-wise independence.
Under a sufficiently fine discretization as \(q \to \infty\), one may thus view Theorem~\ref{thm:derand-smoothing} as a generalization of Theorem~\ref{thm:simple-smoothing}.
The non-independence assumption in Theorem~\ref{thm:derand-smoothing} is crucial for reducing sample complexity, as it allows us to impose structure on \(\mcal{D}\) and compress an \(n\)-dimensional source of randomness down to a single dimension.
We use results from~\cite{levine2021improved} to achieve this, which we expand upon in the following remark.

% \subsubsection{Constructing and sampling for derandomization}
\begin{remark} \label{rem:constructing-D}
% We now consider a construction of \(\mcal{D}\) suitable for Theorem~\ref{thm:derand-smoothing}, i.e. that it is discretized and coordinate-wise \emph{dependent}.
% The non-independence assumption in Theorem~\ref{thm:derand-smoothing} is crucial for reducing sample complexity, as it allows us to impose structure on \(\mcal{D}\) and compress an \(n\)-dimensional source of randomness down to a single dimension.
% We achieve this with the results from~\cite{levine2021improved}: on model initialization fix a random seed \(v \in \{0, 1/q, \ldots, (q-1)/q\}^n\) and at test time sample a random scalar \(s_{\mrm{base}}\) to generate the \(n\)-dimensional noise \(s\) as:
We can exactly compute the expected value of \(g\) in Theorem~\ref{thm:derand-smoothing} by constructing \(s \sim \mcal{D}\) as follows: on model initialization fix a random seed \(v \in \{0, 1/q, \ldots, (q-1)/q\}^n\) and at test time sample a random scalar \(s_{\mrm{base}}\) to generate the \(n\)-dimensional noise \(s\) as:
\begin{align*}
    s_{\mrm{base}} \sim \mcal{U}(\{1/q, \ldots, q/q\}) - 1/(2q),
    \qquad
    s_i = (v_i + s_{\mrm{base}}) \enskip\mrm{mod}\enskip 1
    \quad \text{for all \(i = 1, \ldots, n\).}
\end{align*}
% and define each component of \(s\) to be
% \(s_i = (v_i + s_{\mrm{base}}) \enskip\mrm{mod}\enskip 1\) for all \(i = 1, \ldots, n\).
% \begin{align*}
%     s_i = (v_i + s_{\mrm{base}}) \enskip\mrm{mod}\enskip 1,
%     \quad \text{for all \(i = 1, \ldots, n\).}
% \end{align*}
% In effect, \(v\) acts as the initial \(n\)-dimensional seed, while \(s_{\mrm{base}}\) is the one-dimensional noise.
Observe that each coordinate of noise \(s_i\) is uniform and so satisfies the condition for Theorem~\ref{thm:derand-smoothing}.
There here are only \(q\) distinct values of \(s_{\mrm{base}}\), meaning there are only \(q\) distinct values for \(s\) (for fixed \(v\)).
We can therefore exactly compute the expected value with only \(q\) samples from \(\mcal{D}\).
\end{remark}


% Importantly, this choice of \(\mcal{D}\) preserves masking equivalence, where the proof is identical to that of Proposition~\ref{prop:simple-equivalence}.

% \begin{proposition}\label{prop:derand-equivalence}
%     Take \(g\) as in Theorem~\ref{thm:derand-smoothing}, then \(g\) satisfies masking equivalence.
% \end{proposition}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Certifying stability properties with Lipschitz classifiers}
\label{sec:certifying-stability}

Two variants of \dname{} are presented above --- the simple noise case (Theorem~\ref{thm:simple-smoothing}) and the derandomized noise case (Theorem~\ref{thm:derand-smoothing}) --- and both achieve the sufficient Lipschitz smoothness for certifying stability.
In the following we use ``smoothing'' to flexibly refer to either the simple or derandomized variant of \dname{}, as the procedure is identical to both.


The idea is to begin with any base classifier \(h : \mcal{X} \to [0,1]^m\) and then smooth each coordinate function \(h_1, \ldots, h_m\) into \(g_1, \ldots, g_m\), using which we construct \(g : \mcal{X} \times \{0,1\}^n \to [0,1]^m\).
Like earlier, we define \(f(x) = g(x, \mbf{1})\) to be the \dname{}-smoothed classifier.
Note that each coordinate of \(g\) is Lipschitz in its second argument, which means that each coordinate of \(f\) is Lipschitz to the masking of features.
This then allows us to guarantee stability when \(f\) is the classifier part of an explainable model.
We formalize this in the following result.

% By masking equivalence we have the identity
% \begin{align*}
%     f(x \odot \alpha)
%     = g(x \odot \alpha, \mbf{1})
%     = g(x, \alpha)
% \end{align*}

\begin{theorem}[Stability] \label{thm:stability}
    Consider any \(h : \mcal{X} \to [0,1]^m\) with coordinates \(h_1, \ldots, h_m\).
    Fix an appropriate \(\lambda > 0\) and let \(g_1, \ldots, g_m\) be the respectively smoothed coordinates as in either Theorem~\ref{thm:simple-smoothing} (or Theorem~\ref{thm:derand-smoothing}), using which we analogously define \(g : \mcal{X} \times \{0,1\}^n \to [0,1]^m\).
    Also define \(f(x) = g(x, \mbf{1})\).
    Then for any explanation method \(\varphi\), the explainable model \(\angles{f, \varphi}\) at any \(x \in \mcal{X}\) is incrementally stable with radius \(r_{\mrm{inc}}\) and decrementally stable with radius \(r_{\mrm{dec}}\):
    \begin{align*}
        r_{\mrm{inc}} = \frac{g_A (x, \varphi(x)) - g_B (x, \varphi(x))}{2 \lambda},
        \qquad
        r_{\mrm{dec}} = \frac{g_A (x, \mbf{1}) - g_B (x, \mbf{1})}{2 \lambda},
    \end{align*}
    where \(g_A, g_B\) are the first and second largest logits of \(g\) as in~\eqref{eq:logit-gap}.
\end{theorem}


Note that it is only in the case where the radius \(\geq 1\) do non-trivial stability guarantees exist.
Because each \(g_k\) has range in \([0,1]\), this means that a Lipschitz constant of \(\lambda \geq 1/2\) is necessary to attain at least one radius of stability.
We present in Appendix~\ref{sec:basic-extensions} some extensions to \dname{} that allows one to achieve higher coverage of features.



==> old/smoothing_3.tex <==
\section{Multiplicative smoothing for Lipschitz constants}
\label{sec:smoothing}
In this section we present our main technical contribution in Multiplicative Smoothing (\dname{}).
The goal is to transform an arbitrary base classifier \(h : \mcal{X} \to [0,1]^m\) into a smoothed classifier \(f : \mcal{X} \to [0,1]^m\) that satisfies the appropriate Lipschitz conditions.
This then allows one to appropriately couple an explanation method \(\varphi\) with \(f\) in order to form an explainable model \(\angles{f, \varphi}\) with provable stability guarantees.

We first motivate and give an overview of \dname{} in Section~\ref{sec:dname-overview}, where we illustrate that a principal motivation for developing \dname{} is because classical smoothing techniques may fail to satisfy a property that we call \emph{masking equivalence}.
We then formally introduce \dname{} in two parts: first a simple approach in Section~\ref{sec:dname-rand}, and then a more efficient method in Section~\ref{sec:dname-derand} that we call the derandomized approach.
Both forms of smoothing achieve the desired Lipschitz smoothness, but the key distinction is in the choice of noise distribution.
In particular, we show that each coordinate of the noise vector need not be statistically independent, and this allows us to exactly evaluate the smoothed model with \(N \ll 2^n\) samples.
We finally combine all the details in Section~\ref{sec:certifying-stability} and present how to provably certify the stability of an \dname{}-smoothed explainable model \(\angles{f, \varphi}\).




\subsection{Overview of MuS}
\label{sec:dname-overview}

Our key insight is that Lipschitz smoothness to the masking of features can be achieved if one randomly masks features during classification.
We therefore define \(f\) as follows:
\begin{align} \label{eq:dname-sketch-f}
    f(x) = \expval{s \sim \mcal{D}} h(x \odot s),
    \qquad s_i \sim \mcal{B}(\lambda),
    \qquad i = 1, \ldots, n
\end{align}



\begin{align} \label{eq:dname-sketch-g}
    g(x, \alpha)
        = \expval{s \sim \mcal{D}}
            h(x \odot \tilde{\alpha}),
    \qquad \tilde{\alpha}_i = \alpha_i \odot s_i,
    \qquad s_i \sim \mcal{B}(\lambda),
    \qquad i = 1, \ldots, n
\end{align}

\red{AAAAAAAAAAAAAAAAAAA}


We therefore construct \(f\) in two steps: first we use \(h\) to define a function \(g(x, \alpha) \in [0,1]^m\) such that \(g\) is Lipschitz in \(\alpha \in \{0,1\}^n\) for all \(x \in \mcal{X}\); then we defined the smoothed classifier by \(f(x) = g(x, \mbf{1})\) and show that it satisfies the desired properties.
This \(g\) is the essence of \dname{} and is defined as follows:
where \(s \sim \mcal{D}\) is a random vector on \(\{0,1\}^n\) with each coordinate Bernoulli.
We treat the input \(x\) and mask \(\alpha\) as separate parameters for \(g\) because Lipschitz smoothness is a property over functions, and we show that such \(g\) are \(\lambda\)-Lipschitz in its \(\alpha\) parameter.
The evaluation of \(g(x, \alpha)\) is illustrated in Figure~\ref{fig:durt-overview} and is decomposed into three stages: first, we randomly drop bits from \(\alpha\) with probability \(1-\lambda\), for which we sample \(N\) new masks \(\tilde{\alpha}^{(1)}, \ldots, \tilde{\alpha}^{(N)} \preceq \alpha\); second, we apply these new masks on the original input to yield \(x \odot \tilde{\alpha}^{(i)}\) for \(i = 1, \ldots, N\); third, we evaluate each \(h(x \odot \tilde{\alpha}^{(i)})\) for \(i = 1, \ldots, N\) and average the results --- the class of \(g(x, \alpha)\) being a majority vote.


\input{figures/durt-overview}


The relevance  to stability is this: \(g\) defined as in~\eqref{eq:dname-sketch-g} satisfies \emph{masking equivalence} (Definition~\ref{def:masking-equivalence}):
\begin{align}
    g(x, \alpha)
    = g(x \odot \alpha, \mbf{1})
    = f(x \odot \alpha),
    \tag{by Lemma~\ref{lem:masking-equivalence}}
\end{align}
which lets us rewrite stability properties with \(f\) in terms of \(g\):
\begin{align}
    f(x \odot \alpha)
    = g(x, \alpha)
    \cong g(x, \varphi(x))
    = f(x \odot \varphi(x))
    \quad \text{for all \(\alpha \succeq \varphi(x)\)},
    \tag{c.f. Definition~\ref{def:stable})}
\end{align}
where incremental and decremental stability may be analogously defined.
This translation is useful, as \(g\) is \(\lambda\)-Lipschitz in its \(\alpha\) parameter (Theorem~\ref{thm:simple-smoothing}, Theorem~\ref{thm:derand-smoothing}), and so allows us to establish the desired stability properties (Theorem~\ref{thm:stability}).

We now fo

We now show that \(g\) as defined in~\eqref{eq:dname-sketch-g} satisfies masking equivalence.
\begin{definition} \label{def:masking-equivalence}
    The function \(g : \mcal{X} \times \{0,1\}^n \to [0,1]^m\) satisfies masking equivalence if \(g(x, \alpha) = g(x \odot \alpha, \mbf{1})\) for all \(x \in \mcal{X}\) and \(\alpha \in \{0,1\}^n\).
\end{definition}

\begin{lemma}\label{lem:masking-equivalence}
    Fix \(\lambda \in [0,1]\) and let \(\mcal{D}\) be any distribution on \(\{0,1\}^n\) with the properties listed in \eqref{eq:dname-sketch-g}, then \(g : \mcal{X} \times \{0,1\}^n \to [0,1]^m\) satisfies masking equivalence.
\end{lemma}
\begin{proof}
Note that any \(\alpha \in \{0,1\}^n\) satisfies the identity \(\alpha = \mbf{1} \odot \alpha\).
We may therefore write:
\begin{align*}
    g(x, \alpha)
        = \expval{s \sim \mcal{D}} h(x \odot (\alpha \odot s))
        = \expval{s \sim \mcal{D}} h(x \odot \alpha \odot (\mbf{1} \odot s))
        = g(x \odot \alpha, \mbf{1})
\end{align*}
\end{proof}

Masking equivalence is algebraically useful for converting between between \(f\) and \(g\) when manipulating stability guarantees.
Importantly, we were motivated to develop \dname{} because classical smoothing techniques, namely additive smoothing~\cite{cohen2019certified,yang2020randomized}, may fail to satisfy masking equivalence.
Additive smoothing is by far the most popular smoothing technique, and differs from \dname{} in how noise is applied, where let \(\mcal{D}_{\mrm{mult}}\) and \(\mcal{D}_{\mrm{add}}\) be any two distributions on (subsets of) \(\mbb{R}^n\):
\begin{align*}
    g(x, \alpha)
    = \begin{dcases}
        \expval{s \sim \mathcal{D}_{\mrm{mult}}} h(x \odot (\alpha \odot s))
            &\text{multiplicative noise injection} \\
        \expval{s \sim \mcal{D}_{\mrm{add}}} h(x \odot (\alpha + s))
            &\text{additive noise injection}
    \end{dcases}
\end{align*}

Particularly, additive smoothing has counterexamples to masking equivalence.

% As alluded to earlier, additive smoothing may violate masking equivalence.

\begin{proposition} \label{prop:additive-smoothing-fails}
There exists \(h : \mcal{X} \to [0,1]\) and distribution \(\mcal{D}\) such that \(g\) defined as
\begin{align*}
    g(x, \alpha) = \expval{s \sim \mcal{D}} h(x \odot (\alpha + s)),
\end{align*}
satisfies the inequation \(g(x, \alpha) \neq g(x \odot \alpha, \mbf{1})\) for some \(x \in \mcal{X}\) and \(\alpha \in \{0,1\}^n\).
\end{proposition}
\begin{proof}
Consider some \(h\) such that \(h(\mbf{0}) = 0\), and \(h(x) = 1\) for all other \(x \in \mcal{X}\).
Suppose that \(\mcal{D}\) is a non-constant distribution on \(\mbb{R}^n\), and consider \(\alpha = \mbf{0}\).
Then we have the strict inequality
\begin{align*}
    g(x, \alpha) = \expval{s \sim \mcal{D}} h(x \odot (\alpha + s))
    > \expval{s \sim \mcal{D}} h((x \odot \alpha) \odot (\mbf{1} + s))
    = g(x \odot \alpha, \mbf{1})
    = 0
\end{align*}
\end{proof}

Intuitively, this occurs because additive smoothing primarily applies noise by perturbing feature values, rather than completely masking them.
As such, there might be ``information leakage'' when non-explanatory bits of \(\alpha\) are changed into non-zero values.
This then causes each sample of \(h(x \odot \tilde{\alpha})\) within \(g(x, \alpha)\) to observe more features of \(x\) than it would have been able to otherwise.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multiplicative smoothing}
\label{sec:dname}

\begin{theorem}[MuS] \label{thm:mus}
    Consider any \(h : \mcal{X} \to [0,1]\) and define \(g : \mcal{X} \times \{0,1\}^n \to [0,1]\) as
    \begin{align*}
        g(x, \alpha)
            = \expval{s \sim \mcal{D}} h(x \odot \tilde{\alpha}),
            \qquad
            \tilde{\alpha} = \alpha \odot s,
            \qquad s_i \sim \mcal{B} (\lambda)
    \end{align*}
    Then \(g(x, \cdot) : \{0,1\}^n \to [0,1]\) is \(\lambda)\)-Lipschitz in the \(\ell^1\) norm for all \(x \in \mcal{X}\).
\end{theorem}

\red{AAAAAAAAAAAAAAAAAAAAAAAAAAAAAAA}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multiplicative smoothing with simple noise}
\label{sec:dname-rand}

It suffices to use \(\mcal{U}^n (0,1)\), the uniform distribution on \([0,1]^n\), to achieve the sufficient Lipschitz constants for stability.
This we illustrate in the following result.

\begin{theorem}[Simple \dname{}] \label{thm:simple-smoothing}
    Consider any \(h : \mcal{X} \to [0,1]\) and define \(g : \mcal{X} \times \{0,1\}^n \to [0,1]\) as
    \begin{align} \label{eq:thm:simple-smoothing}
        g(x, \alpha) = \expval{s \sim \mcal{B}^{n} (\lambda)} h(x \odot \tilde{\alpha}),
        \qquad \tilde{\alpha} = \alpha \odot s,
        \qquad \lambda \in [0,1] \enskip \text{fixed}.
    \end{align}
    Then \(g(x, \cdot) : \{0,1\}^{n} \to [0,1]\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm for all \(x \in \mcal{X}\).
\end{theorem}

We emphasize that the formulation of Theorem~\ref{thm:simple-smoothing} is just that of~\eqref{eq:dname-sketch-g} using the uniform distribution, and this choice will satisfy zeroing coordinates of \(\alpha\) with probability \(1 - \lambda\).
A limitation of using a uniform distribution, however, is that one needs an exponential number of samples to exactly compute the expected value.
This is a barrier to tractable implementation, and approximating the expected value with fewer samples would require probabilistic bounds on the Lipschitz constant.
We remark that this need for approximation arises in many randomized smoothing methods~\cite{cohen2019certified}, and high sample complexity is a known issue for randomized smoothing~\cite{kumar2020curse}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multiplicative smoothing with derandomization}
\label{sec:dname-derand}

Importantly, each noise coordinate from \(\mcal{D}\) need only be uniform and \emph{not} statistically independent to attain the desired Lipschitz conditions (Theorem~\ref{thm:derand-smoothing}).
We construct \(\mcal{D}\) with structured dependence and exploit it to significantly reduce the sample complexity of evaluating the smoothed model.
We call this process process \emph{derandomization}, and achieve it using two key ideas from~\cite{levine2021improved}: first, by fixing an integer \(q > 0\) to discretize the values of \(\lambda \in \{1/q, \ldots, q/q\}\); second, by a construction of \(\mcal{D}\) (Remark~\ref{rem:constructing-D}).
One then needs only \(q\) samples to \emph{exactly} evaluate the smoothed model --- an exponential reduction from the simple noise case in Theorem~\ref{thm:simple-smoothing}.
% In the following we first present the smoothness results of using such a discretized and non-independent \(\mcal{D}\) in Theorem~\ref{thm:derand-smoothing}.
% We then present an explicit construction of \(\mcal{D}\).

\begin{theorem}[Derandomized \dname{}] \label{thm:derand-smoothing}
    Fix an integer \(q > 0\) and let \(s \sim \mcal{D}\) be a \(n\)-dimensional random vector with each coordinate uniformly distributed as
    \begin{align} \label{eq:thm:derand-smoothing-1}
        s_i \sim \mcal{U}(\{1/q, \ldots, q/q\}) - 1/(2q),
        \quad i = 1, \ldots, n,
    \end{align}
    where \(\mcal{D}\) is any finite discrete distribution on \([0,1]^n\) such that \(s_i\) need not be independent.
    Consider any \(h : \mcal{X} \to [0,1]\) and define \(g : \mcal{X} \times \{0,1\} ^{n} \to [0,1]\) as
    \begin{align} \label{eq:thm:derand-smoothing-2}
        g(x, \alpha) = \expval{s \sim \mcal{D}} h(x \odot \tilde{\alpha}),
        \qquad \tilde{\alpha} = \mbb{I}[\lambda \alpha \geq s],
        \qquad \lambda \in \{1/q, \ldots, q/q\} \enskip \text{fixed}.
    \end{align}
    Then \(g(x, \cdot) : \{0,1\}^n \to [0,1]\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm for all \(x \in \mcal{X}\).
\end{theorem}

We emphasize that the main difference between the earlier simple variant in Theorem~\ref{thm:simple-smoothing} and the result here are: the discretization of the smoothing parameter \(\lambda\) and noise \(s \sim \mcal{D}\), and the lack of coordinate-wise independence.
Under a sufficiently fine discretization as \(q \to \infty\), one may thus view Theorem~\ref{thm:derand-smoothing} as a generalization of Theorem~\ref{thm:simple-smoothing}.
The non-independence assumption in Theorem~\ref{thm:derand-smoothing} is crucial for reducing sample complexity, as it allows us to impose structure on \(\mcal{D}\) and compress an \(n\)-dimensional source of randomness down to a single dimension.
We use results from~\cite{levine2021improved} to achieve this, which we expand upon in the following remark.

% \subsubsection{Constructing and sampling for derandomization}
\begin{remark} \label{rem:constructing-D}
% We now consider a construction of \(\mcal{D}\) suitable for Theorem~\ref{thm:derand-smoothing}, i.e. that it is discretized and coordinate-wise \emph{dependent}.
% The non-independence assumption in Theorem~\ref{thm:derand-smoothing} is crucial for reducing sample complexity, as it allows us to impose structure on \(\mcal{D}\) and compress an \(n\)-dimensional source of randomness down to a single dimension.
% We achieve this with the results from~\cite{levine2021improved}: on model initialization fix a random seed \(v \in \{0, 1/q, \ldots, (q-1)/q\}^n\) and at test time sample a random scalar \(s_{\mrm{base}}\) to generate the \(n\)-dimensional noise \(s\) as:
We can exactly compute the expected value of \(g\) in Theorem~\ref{thm:derand-smoothing} by constructing \(s \sim \mcal{D}\) as follows: on model initialization fix a random seed \(v \in \{0, 1/q, \ldots, (q-1)/q\}^n\) and at test time sample a random scalar \(s_{\mrm{base}}\) to generate the \(n\)-dimensional noise \(s\) as:
\begin{align*}
    s_{\mrm{base}} \sim \mcal{U}(\{1/q, \ldots, q/q\}) - 1/(2q),
    \qquad
    s_i = (v_i + s_{\mrm{base}}) \enskip\mrm{mod}\enskip 1
    \quad \text{for all \(i = 1, \ldots, n\).}
\end{align*}
% and define each component of \(s\) to be
% \(s_i = (v_i + s_{\mrm{base}}) \enskip\mrm{mod}\enskip 1\) for all \(i = 1, \ldots, n\).
% \begin{align*}
%     s_i = (v_i + s_{\mrm{base}}) \enskip\mrm{mod}\enskip 1,
%     \quad \text{for all \(i = 1, \ldots, n\).}
% \end{align*}
% In effect, \(v\) acts as the initial \(n\)-dimensional seed, while \(s_{\mrm{base}}\) is the one-dimensional noise.
Observe that each coordinate of noise \(s_i\) is uniform and so satisfies the condition for Theorem~\ref{thm:derand-smoothing}.
There here are only \(q\) distinct values of \(s_{\mrm{base}}\), meaning there are only \(q\) distinct values for \(s\) (for fixed \(v\)).
We can therefore exactly compute the expected value with only \(q\) samples from \(\mcal{D}\).
\end{remark}


% Importantly, this choice of \(\mcal{D}\) preserves masking equivalence, where the proof is identical to that of Proposition~\ref{prop:simple-equivalence}.

% \begin{proposition}\label{prop:derand-equivalence}
%     Take \(g\) as in Theorem~\ref{thm:derand-smoothing}, then \(g\) satisfies masking equivalence.
% \end{proposition}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Certifying stability properties with Lipschitz classifiers}
\label{sec:certifying-stability}

Two variants of \dname{} are presented above --- the simple noise case (Theorem~\ref{thm:simple-smoothing}) and the derandomized noise case (Theorem~\ref{thm:derand-smoothing}) --- and both achieve the sufficient Lipschitz smoothness for certifying stability.
In the following we use ``smoothing'' to flexibly refer to either the simple or derandomized variant of \dname{}, as the procedure is identical to both.


The idea is to begin with any base classifier \(h : \mcal{X} \to [0,1]^m\) and then smooth each coordinate function \(h_1, \ldots, h_m\) into \(g_1, \ldots, g_m\), using which we construct \(g : \mcal{X} \times \{0,1\}^n \to [0,1]^m\).
Like earlier, we define \(f(x) = g(x, \mbf{1})\) to be the \dname{}-smoothed classifier.
Note that each coordinate of \(g\) is Lipschitz in its second argument, which means that each coordinate of \(f\) is Lipschitz to the masking of features.
This then allows us to guarantee stability when \(f\) is the classifier part of an explainable model.
We formalize this in the following result.

% By masking equivalence we have the identity
% \begin{align*}
%     f(x \odot \alpha)
%     = g(x \odot \alpha, \mbf{1})
%     = g(x, \alpha)
% \end{align*}

\begin{theorem}[Stability] \label{thm:stability}
    Consider any \(h : \mcal{X} \to [0,1]^m\) with coordinates \(h_1, \ldots, h_m\).
    Fix an appropriate \(\lambda > 0\) and let \(g_1, \ldots, g_m\) be the respectively smoothed coordinates as in either Theorem~\ref{thm:simple-smoothing} (or Theorem~\ref{thm:derand-smoothing}), using which we analogously define \(g : \mcal{X} \times \{0,1\}^n \to [0,1]^m\).
    Also define \(f(x) = g(x, \mbf{1})\).
    Then for any explanation method \(\varphi\), the explainable model \(\angles{f, \varphi}\) at any \(x \in \mcal{X}\) is incrementally stable with radius \(r_{\mrm{inc}}\) and decrementally stable with radius \(r_{\mrm{dec}}\):
    \begin{align*}
        r_{\mrm{inc}} = \frac{g_A (x, \varphi(x)) - g_B (x, \varphi(x))}{2 \lambda},
        \qquad
        r_{\mrm{dec}} = \frac{g_A (x, \mbf{1}) - g_B (x, \mbf{1})}{2 \lambda},
    \end{align*}
    where \(g_A, g_B\) are the first and second largest logits of \(g\) as in~\eqref{eq:logit-gap}.
\end{theorem}


Note that it is only in the case where the radius \(\geq 1\) do non-trivial stability guarantees exist.
Because each \(g_k\) has range in \([0,1]\), this means that a Lipschitz constant of \(\lambda \geq 1/2\) is necessary to attain at least one radius of stability.
We present in Appendix~\ref{sec:basic-extensions} some extensions to \dname{} that allows one to achieve higher coverage of features.



==> old/smoothing_proofs_1.tex <==
\section{Proofs for Section~\ref{sec:smoothing}}


\subsection{Proof of Theorem~\ref{thm:simple-smoothing}}
\begin{proof}
Observe that if \(s \sim \mcal{B}^n (\lambda)\), then \(\alpha \odot s\) and \(\mbb{I}[\lambda \alpha \geq r]\) with \(r \sim \mcal{U}^n (0,1)\) are statistically equivalent.
Consider any \(x \in \mcal{X}\) and let \(\mbb{I}_{\geq 0} : \mbb{R}^{n} \to \{0,1\}^n\) be the coordinate-wise indicator function of non-negativity.
Then we may express \(g(x, \alpha)\) as:
\begin{align*}
    g(x, \alpha)
    &= \expval{s \sim \mcal{B}^n (\lambda)}
        \bracks{h(x \odot \alpha \odot s)} \\
    &= \expval{r \sim \mcal{U}^n (0,1)}
        \bracks{h(x \odot \mbb{I} [\lambda \alpha \geq r])} \\
    &= \expval{r \sim \mcal{U}^n (0,1)}
        \bracks{(h \circ (x \odot \cdot) \circ \mbb{I}_{\geq 0}) (\lambda \alpha - r)} \\
    &= \expval{r \sim \mcal{U}^n (0,1)}
        \bracks{\omega (\lambda \alpha - r)}
        \tag{\(\omega = h \circ (x \odot \cdot) \circ \mbb{I}_{\geq 0}\)} \\
    &= \expval{t \sim \mcal{U}^n (-1/(2\lambda), 1/(2\lambda))}
        \bracks{\omega(\lambda\alpha + 
        \lambda t - \mbf{1}/2))} \\
    &= \expval{t \sim \mcal{U}^n (-1/(2\lambda), 1/(2\lambda))}
        \bracks{\zeta (\alpha + t)}
    \tag{\(\zeta (z) = \omega(\lambda z - \mbf{1}/2)\)}
    % &= \red{XXXXX} \\
    % &= \expval{t \sim \mcal{U}^n (-1/(2\lambda), 1/(2\lambda))}
    %     \bracks{\omega (\alpha + t - \mbf{1}/(2\lambda))},
\end{align*}
where we use the relation
\begin{align*}
    \underbrace{- \mcal{U}^n (0,1)}_{\sim - r}
    = \lambda \underbrace{\mcal{U}^n (-1/(2\lambda), 1/(2\lambda))}_{\sim t} - \mbf{1}/2.
\end{align*}
It follows from Theorem 1~\cite{levine2021improved} that \(g(x, \cdot)\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm.
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Theorem~\ref{thm:derand-smoothing}}
\begin{proof}
Fix any \(s \sim \mcal{D}\) and \(x \in \mcal{X}\).
Let \(\alpha, \alpha' \in \{0,1\}^n\) and define \(\delta = \alpha - \alpha'\).
Observe that \(\tilde{\alpha}_i \neq \tilde{\alpha}_i '\) exactly when: \(\abs{\delta_i} = 1\) and \(s_i < \lambda\) (if \(s_i > \lambda\), then \(\tilde{\alpha}_i = \tilde{\alpha}_i ' = 0\); we also cannot have \(\lambda = s_i\) by the values of \(\mcal{D}\)).
Because \(s_i\) is uniformly distributed across \(q\) distinct values and only \(\lambda q\) of them are \(< \lambda\), it follows that \(\mrm{Pr}[\lambda < s_i] = \lambda\).
Consequently, we have \(\mrm{Pr}[\tilde{\alpha}_i \neq \tilde{\alpha}_i '] = \lambda \abs{\delta_i}\).
Applying the union bound:
\begin{align*}
    \prob{s \sim \mcal{D}}
        \bracks{\tilde{\alpha} \neq \tilde{\alpha}'}
    = \prob{s \sim \mcal{D}}
        \bracks{\bigcup_{i=1}^{n} \tilde{\alpha}_i \neq \tilde{\alpha}_i '}
    \leq \sum_{i=1}^{n} \lambda \abs{\delta_i}
    = \lambda \norm{\delta}_1,
\end{align*}
and so:
\begin{align*}
    \abs{g(x, \alpha) - g(x, \alpha')}
    &= \abs*{\expval{s \sim \mcal{D}} h(x \odot \tilde{\alpha})
        - \expval{s \sim \mcal{D}} h(x \odot \tilde{\alpha}')} \\
    &= \abs*{\expval{s \sim \mcal{D}}
            \bracks{h(x \odot \tilde{\alpha}) - h(x \odot \tilde{\alpha}')}} \\
    &= \Big|
            \prob{s \sim \mcal{D}} \bracks{\tilde{\alpha} \neq \tilde{\alpha}'}
            \cdot \expval{s \sim \mcal{D}} \bracks{h(x \odot \tilde{\alpha}) - h(x \odot \tilde{\alpha}') \,|\, \tilde{\alpha} \neq \tilde{\alpha}'} \\
    &\quad - \prob{s \sim \mcal{D}} \bracks{\tilde{\alpha} = \tilde{\alpha}'}
            \cdot \expval{s \sim \mcal{D}} \bracks{h(x \odot \tilde{\alpha}) - h(x \odot \tilde{\alpha}') \,|\, \tilde{\alpha} = \tilde{\alpha}'}
        \Big|.
\end{align*}
Note that \(\mbb{E}\, \bracks{h(x \odot \tilde{\alpha}) - h(x \odot \tilde{\alpha}') \,|\, \tilde{\alpha} = \tilde{\alpha}'} = 0\), and so
\begin{align*}
    \abs{g(x, \alpha) - g(x, \alpha')}
    &= \prob{s \sim \mcal{D}} \bracks{\tilde{\alpha} \neq \tilde{\alpha}'}
            \cdot
            \underbrace{
                \abs*{\expval{s \sim \mcal{D}} \bracks{h(\angles{x, \tilde{\alpha}}) - h(\angles{x, \tilde{\alpha}'}) \,|\, \tilde{\alpha} \neq \tilde{\alpha}'}}
            }_{\leq 1 \enskip \text{because \(h(\cdot) \in [0,1]\)}}
    \\
    & \leq \prob{s \sim \mcal{D}} \bracks{\tilde{\alpha} \neq \tilde{\alpha}'}
    \leq \lambda \norm{\delta}_1.
\end{align*}
% which is \(\leq \lambda \norm{\delta}_1\).
Thus, \(g(x, \cdot)\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Proof of Theorem~\ref{thm:stability}}
\begin{proof}
We show the case for simple smoothing (Theorem~\ref{thm:simple-smoothing}), since the proof for derandomized smoothing (Theorem~\ref{thm:derand-smoothing}) is nearly identical.
We first show incremental stability.
Let \(x \in \mcal{X}\) be arbitrary, then by Lemma~\ref{lem:masking-equivalence} we have
\begin{align*}
    f(x \odot \varphi(x))
    = g(x \odot \varphi(x), \mbf{1})
    = g(x, \varphi(x)),
\end{align*}
and suppose without loss of generality that \(g_1 (x, \varphi(x)) > g_2 (x, \varphi(x))\) are the top two logits of \(g(x, \varphi(x))\) at this \(x\).
By Lipschitz smoothness from Theorem~\ref{thm:simple-smoothing} we have for all \(\alpha \in \{0,1\}^n\) that
\begin{align*}
    \norm{g_1 (x, \varphi(x)) - g_1 (x, \alpha)}_1
    &\leq \lambda \norm{\varphi(x) - \alpha}_1 \\
    \norm{g_2 (x, \varphi(x)) - g_2 (x, \alpha)}_1
    &\leq \lambda \norm{\varphi(x) - \alpha}_1
\end{align*}
Observe that if \(\alpha\) is sufficiently close to \(\varphi(x)\), i.e.
\begin{align*}
    2 \lambda \norm{\varphi(x) - \alpha}_1 \leq g_1 (x, \varphi(x)) - g_2 (x, \varphi(x)),
\end{align*}
then \(g_1 (x, \alpha)\) is also the top logit of \(g(x, \alpha)\).
This means that \(g(x, \varphi(x)) \cong g(x, \alpha)\) and thus \(f(x \odot \varphi(x)) \cong f(x \odot \alpha)\), thereby proving incremental stability with radius \(d(x, \varphi(x)) / (2 \lambda)\).

The decremental stability case is similar, except we replace \(\varphi(x)\) with \(\mbf{1}\).
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Some Basic Extensions}
\label{sec:basic-extensions}
We now discuss some extensions to \dname{} that help with performance, namely \emph{feature grouping} and \emph{selective noising}.

\paragraph{Feature Grouping}
We have so far assumed that \(\mcal{X} = \mbb{R}^{n}\), but sometimes it may be desirable to group features together, e.g. color channels of the same pixel.
Our results also hold for more general \(\mcal{X} = \mbb{R}^{d_1} \times \cdots \times \mbb{R}^{d_n}\), where for such \(x \in \mcal{X}\) and \(\alpha \in \mbb{R}^{n}\) we lift \(\odot\) as
\begin{align*}
    (x \odot \alpha)_i = x_i \cdot \mbb{I}[\alpha_i = 1] \in \mbb{R}^{d_i}.
\end{align*}
All of our proofs are identical under this construction, with the exception of the dimensionalities of terms like \((x \odot \alpha)\).
An example of feature grouping is given in Figure~\ref{fig:non-stable}.


\paragraph{Selective Noising}
It may be desirable to selectively apply noise to some features and not others.
This is particularly the case in settings like decremental stability, where for an explainable model \(\angles{f, \varphi}\) and given input \(x \in \mcal{X}\) we only wish to noise over the non-explanatory features as given by \(\varphi(x)\).
We introduce Theorem~\ref{thm:selective-masking} below as a more fine-grained approach for boosting the possibly conservative Lipschitz constants that we may otherwise get from the Theorem~\ref{thm:derand-smoothing}.
Our idea is to use a binary vector \(\mu \in \{0, 1\}^n\) called the \emph{selective noise mask}, where \(\mu_i = 1\) denotes that feature \(x_i\) should be noised, while if \(\mu_i = 0\), then feature \(x_i\) should not be noised, and is retained.
\begin{theorem} \label{thm:selective-masking}
    Take \(\mcal{D}, h, \lambda\) be as in Theorem~\ref{thm:derand-smoothing} and define \(g : \mcal{X} \times \{0,1\}^n \to [0,1]\) as
    \begin{align} \label{eq:thm:selective-masking-1}
        g(x, \alpha)
            = \expval{s \sim \mcal{U}^n (0,1)} h(x \odot \tilde{\alpha}),
        \qquad
        \tilde{\alpha}
            = (\mbf{1} - \mu) + \mu \odot \mbb{I}[\lambda \alpha \geq s],
        \qquad \mu \in \{0,1\}^n \enskip \text{fixed}.
    \end{align}
    Then \(g(x, \cdot) : \{0,1\}^n \to [0,1]\) is \(\lambda\)-Lipschitz in the \(\ell^1\) norm for all \(x \in \mcal{X}\).
\end{theorem}
\begin{proof}
Let \(\alpha, \alpha' \in \{0,1\}^n\) and define \(\delta = \alpha - \alpha'\), and fix \(s \sim \mcal{D}\) and \(x \in \mcal{D}\) as in the proof of Theorem~\ref{thm:derand-smoothing}.
Observe that if \(\mu_i = 0\), then \(\tilde{\alpha}_i = \tilde{\alpha}_i' = 1\), and so \(\tilde{\alpha}_i \neq \tilde{\alpha}_i '\) exactly when: \(\mu_i = 1\) and \(\abs{\delta_i} = 1\) and \(s_i < \lambda\).
Consequently, \(\mrm{Pr}[\tilde{\alpha}_i \neq \tilde{\alpha}_i '] = \lambda \mu_i \abs{\delta_i}\).
Applying the union bound:
\begin{align*}
    \prob{s \sim \mcal{D}}
        \bracks{\tilde{\alpha} \neq \tilde{\alpha}'}
    =
    \prob{s \sim \mcal{D}}
        \bracks{\bigcup_{i=1}^{n} \tilde{\alpha}_i \neq \tilde{\alpha}_i '}
    \leq \sum_{i=1}^{n} \lambda \mu_i \abs{\delta_i}
    \leq \lambda \norm{\delta}_1,
\end{align*}
where recall each \(\mu_i \in \{0,1\}\).
The rest then follows as in the proof of Theorem~\ref{thm:derand-smoothing}.
\end{proof}


Importantly, selective noising still preserves the masking equivalence property under an ordering assumption that \(\mu \succeq \varphi(x)\).

\begin{proposition}
\label{prop:noise-mask-equivalence}
    Take \(\mcal{D}, g, \mu\) as in Theorem~\ref{thm:selective-masking}, then
    \(g(x, \alpha) = g(x \odot \alpha, \mbf{1})\)
    for all \(x \in \mcal{X}\) and \(\mu \succeq \alpha\).
\end{proposition}
\begin{proof}
Let \(\tilde{x} = x \odot \tilde{\alpha}\), and define \(\tilde{x}_{\mrm{LHS}}\) (resp. \(\tilde{x}_{\mrm{RHS}}\)) to be the corresponding terms of \(g(x, \alpha)\) (resp. \(g(x \odot \alpha, \mbf{1})\)).
It suffices to show that \(\tilde{x}_{\mrm{LHS}} = \tilde{x}_{\mrm{RHS}}\).
Then:
\begin{align*}
    \tilde{x}_{\mrm{LHS}}
    &= x \odot \big((\mbf{1} - \mu) + \mu \odot \mbb{I}[\lambda \alpha \geq s]\big) \\
    &= x \odot \big((\mbf{1} - \mu) + \alpha \odot \mu \odot \mbb{I}[\lambda \mbf{1} \geq s]\big)
\end{align*}
where observe that \(\mbb{I}[\lambda \alpha \geq s] = \alpha \odot \mbb{I}[\lambda \mbf{1} \geq s]\), and also:
\begin{align*}
    \tilde{x}_{\mrm{RHS}}
    &= (x \odot \alpha) \odot \big((\mbf{1} - \mu) + \mu \odot \mbb{I}[\lambda \mbf{1} \geq s]\big).
\end{align*}
Note that \(\tilde{x}_{\mrm{LHS}} = \tilde{x}_{\mrm{RHS}}\) iff
\begin{align*}
    x \odot (1 - \mu) =
    x \odot \alpha \odot (1 - \mu),
\end{align*}
which indeed holds because \(\mu \succeq \alpha\).
\end{proof}



==> old_figures/certified-accuracy.tex <==
\begin{figure}[ht]
\centering

% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=1.0\textwidth]{images/vit-cert-robust.png}
% \end{subfigure}

% \begin{subfigure}[b]{0.48\textwidth}
% \includegraphics[width=1.0\textwidth]{images/resnet-cert-robust.png}
% \end{subfigure}

% \begin{subfigure}[b]{0.48\textwidth}
% \includegraphics[width=1.0\textwidth]{images/roberta-cert-robust.png}
% \end{subfigure}

\includegraphics[width=1.0\textwidth]{images/cert-accs.png}

\caption{
Certified accuracy plots of SHAP-top-\(\lambda\) with \(q = 64\) and \(N = 2000\) samples from ImageNet and TweetEval.
}
\label{fig:certified-accuracy}
\end{figure}



==> old_figures/empirical-robustness.tex <==
\begin{figure}[ht]

\begin{center}
\includegraphics[width=1.0\textwidth]{images/emp-robust.png}
\end{center}

\caption{Empirical robustness.}
\label{fig:empirical-robustness}
\end{figure}



==> old_figures/feature-attributions-eval.tex <==
\begin{figure}[ht]

\begin{subfigure}{1.0\textwidth}
\centering
\includegraphics[width=1.0\textwidth]{images/method-clean-accs.png}
\caption{Clean accuracy scores}
\label{fig:feature-attributions-eval-1}
\end{subfigure}

\vspace{1em}

\begin{subfigure}{1.0\textwidth}
\centering
\includegraphics[width=0.75\textwidth]{images/cert-exp-densities.png}
\caption{Density values}
\label{fig:feature-attributions-eval-2}
\end{subfigure}

\caption{(Top) Clean accuracy of different methods with top-\(k\) fractions of \(k \in \{1/8, 2/8, 3/8, 4/8\}\) and \(\lambda \in \{1/8, 2/8, 3/8, 4/8\}\).
(Bottom) Density values of using different methods to construct a certifiably robust \(\alpha \in \{0,1\}^{196}\) of radius \(1\) with respect to \(P_{\mrm{suff}}\) and \(P_{\mrm{necc}}\).
}
\label{fig:feature-attributions-eval}
\end{figure}



==> old_figures/models-table.tex <==
\begin{figure}[ht]

\begin{center}
\begin{tabular}{ |c|c|c|c|c|c|c| } 
 \hline
 \textbf{Model} & \textbf{Dataset} & \textbf{Optimizer} & \textbf{Learning Rate} & \textbf{Batch Size} \\
 \hline
 Vision Transformer (\texttt{b\_16}) & ImageNet1K & Adam & \(10^{-6}\) & 32 \\
 \hline
 ResNet50 & ImageNet1K & Adam & \(10^{-6}\) & 32 \\
 \hline
 RoBERTa & TweetEval & Adam & \(10^{-6}\) & 1 \\
 \hline
\end{tabular}
\end{center}

\caption{
Default parameters for Adam were used.
For each \(\lambda \in \{1/8, \ldots, 8/8\}\), each model was trained for \(1\) epoch, meaning that a total of \(8 \times 3 = 24\) models are used in the experiments.
}
\label{fig:models-table}
\end{figure}



% odels in Vision Transformer~\cite{dosovitskiy2020image} and ResNet50~\cite{he2016deep}; and one language model in RoBERTa~\cite{liu2019roberta}.
% For the vision dataset we use ImageNet~\cite{russakovsky2015imagenet} and for the language dataset we use TweetEval~\cite{barbieri2020tweeteval}.

==> old_figures/robust-explanation-accuracy.tex <==
\begin{figure}[h]
\centering

\includegraphics[width=1.0\textwidth]{images/robust-exp-accs.png}

\caption{
We plot the radii up to which the fraction of inputs are consistent and incrementally stable (top), and consistent and decrementally stable (bot).
We take \(\varphi\) to be SHAP top-25\% with \(q = 64\) and \(N = 2000\) samples from their respective datasets.
}
\label{fig:robust-explanation-accuracy}
\end{figure}



==> old_figures/search-algorithm.tex <==

% \begin{algorithm}[tb]
\begin{algorithm}[!ht]
    \caption{Using \dname{} to solve Problem~\eqref{prob:search}}
    \label{alg:prob:search}
\begin{algorithmic}
    \STATE {\bfseries Given:} model \(f\), input \(x\), order \(\beta\), radii \(r_{\mrm{suff}}, r_{\mrm{necc}}\)
    \STATE Initialize \(\alpha \leftarrow 0^n\)
    \FOR{\(i \in \beta\)}
        \STATE \(\alpha_i \leftarrow 1\)
        \IF{\(P_{\mrm{suff}}(f, x, \alpha, r_{\mrm{suff}})\) and \(P_{\mrm{necc}}(f, x, \alpha, r_{\mrm{necc}})\)}
            \STATE \textbf{return} \(\alpha\)
        \ENDIF
   \ENDFOR
    \STATE \textbf{return} \(\bot\)
\end{algorithmic}
\end{algorithm}

